Sample and Expand: Discovering Low-rank Submatrices With Quality Guarantees

The problem of approximating a matrix by a low-rank one has been extensively studied. This problem assumes, however, that the whole matrix has a low-rank structure. This assumption is often false for real-world matrices. We consider the problem of discovering submatrices from the given matrix with bounded deviations from their low-rank approximations. We introduce an effective two-phase method for this task: first, we use sampling to discover small nearly low-rank submatrices, and then they are expanded while preserving proximity to a low-rank approximation. An extensive experimental evaluation confirms that the method we introduce compares favorably to existing approaches.

==> arXiv-2506.06456v1/additional_analysis.tex <==
Theorem~\ref{th:expansion} provides approximation guarantees for the near-rank-$1$ sub\-matrices found by \ourmethod. 
In more detail, the approximation guarantees are obtained for an interpretable approximation where each row or column is collinear with a single row or column. 
The approximation given by the \svd of the sub\-matrices output by \ourmethod also incurs bounded error in terms of Frobenius and spectral norm, but not necessarily in terms of max norm. 

For the approximation given by the \svd,  it is of particular interest to study the singular values. % of near-rank-$1$ sub\-matrices. 
More specifically, since the spectral norm of a matrix is also equal to its largest singular value, it is interesting to study the spectral norm of the matrix of differences \outputerror obtained by using the rank-$1$ \svd to approximate a sub\-matrix discovered by \ourmethod. 
%spectral norm of the matrix of errors \outputerror obtained when using the rank-$1$ \svd to approximate a sub\-matrix \outputmat discovered by \ourmethod. 
The following result provides a bound on the spectral norm of such matrix of differences. 


%Intuitively, this bounds how much \outputerror can stretch a vector. 


\begin{theorem}\label{th:expansion_appendix}
Let $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ be a near-rank-$1$ sub\-matrix output by \ourmethod, with anchor row $\anchorrow$, anchor column $\anchorcolumn$ and tolerance $\delta$. 
%be any row and any column of $\outputmat$,
%If, as for the matrices \outputmat output by Algorithm~\ref{alg:rankone}, the maximum absolute deviation between two entries in the matrices of ratios obtained by dividing all rows by $\anchorrow$ and all columns by column $\anchorcolumn$  are
%obtained by dividing all rows (columns) by a single row (column) is 
%bounded by $\delta$,
The matrix $\outputerror = \outputmat - \estimate{\outputmat}$ where $\estimate{\outputmat}$ is the rank-$1$ approximation of \outputmat given by \svd satisfies: 

\begin{align}
\spectralnorm{\outputerror}  \leq  
\min\Bigg\{  
%\sqrt{(\nrows -1) \left(1 - \sqrt{1 - 8  \tol^2 \max_i \| \outputmat_{i,:} \|_2 \omega_r (1 - \omega_r)} \right)} 
\sqrt{
\gamma ( \frac{\nrowssubmatrix-1}{\nrowssubmatrix} )  - (\nrowssubmatrix-1) \sqrt{1 -  8 \max_i \| \outputmat_{i,:} \|^2_2 \tol^2 \omega_r  (1 - \tol^2 \omega_r ) } }, 
, \notag &\\
%\sqrt{(\ncols-1) \left(1 - \sqrt{1 - 8  \tol^2 \max_j \| \outputmat_{:,j} \|_2 \omega_c (1 - \omega_c)} \right)}
\sqrt{
\gamma ( \frac{\ncolssubmatrix-1}{\ncolssubmatrix} )  - (\ncolssubmatrix-1) \sqrt{1 -  8 \max_j \| \outputmat_{:,j} \|^2_2 \tol^2 \omega_c  (1 - \tol^2 \omega_c ) } }
\Bigg\},
\end{align}
where 
$\gamma = \frobeniusnorm{\outputmat}^2$, 
$\omega_r = \frac{\sum_{i < j} {x^r_i}^2 {x^r_j}^2 }{\| \anchorrow \|_2^2 \min_i \| \outputmat_{i,:} \|^2_2}$
and 
$\omega_c = 
\frac{\sum_{i < j} {x^c_i}^2 {x^c_j}^2 }{\| \anchorcolumn \|_2^2 \min_j \| \outputmat_{:,j} \|^2_2 }$. 


\iffalse 
$\gamma^r_{max} = \max_i \| \outputmat_{i,:} \|^2_2$


$\omega_c =  
\frac{\sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\| \anchorcolumn \|_2^2}$,  $\gamma^r_{min} = \min_i \| \outputmat_{i,:} \|^2_2$, $\gamma^r_{max} = \max_i \| \outputmat_{i,:} \|^2_2$, $\gamma^c_{min} = \min_j \| \outputmat_{:,j} \|^2_2$ and $\gamma^c_{max} = \max_j \| \outputmat_{:,j} \|^2_2$.    
\fi 
\end{theorem}

Although the bound given in Theorem~\ref{th:expansion_appendix} is rather  intricate, it could be considerably simplified by normalizing data, and its interpretation is similar to that of the bounds presented in 
Theorem~\ref{th:expansion}. 
Like Theorem~\ref{th:expansion}, Theorem~\ref{th:expansion_appendix} bounds the approximation error (in this case, in terms of spectral norm) based on the tolerance parameter $\tol$. 
%Further, the bound could be considerably simplified by normalizing data. 

\iffalse
However, notice that the bound cannot be used to directly set the value of \tol during the execution of Algorithm~\ref{alg:rankone} to match an input threshold \errorbound. For this purpose, one would preliminarily need to make the bound  looser by replacing \outputmat with \inputmat and $\nrows'$ and $\ncols'$ with \nrows and \ncols. 
\fi

\iffalse 
Although not as easily as for Theorem~\ref{th:expansion}, also Theorem~\ref{th:expansion_appendix} can be used to inform the selection of the value of \tol after computing the ratio matrices based on error requirements in terms of spectral norm, as long as the near-rank-$1$ sub\-matrices output by \ourmethod are approximated via \svd.    
\fi 


%to meet specific error requirements defined in terms of spectral norm, provided that the near-rank-$1$ sub\-matrices output by \ourmethod are approximated via \svd.  




































\iffalse 
\cnote[MC]{We probably do not need this - we currently keep this section in case we want to move part of the analysis (particularly, probabilistic analysis or time-complexity analysis paragraph) here.}
For completeness, here, we also notice that the bound we impose on the ratios also leads to a simply necessary (but not sufficient) condition for a matrix to be \emph{entry-wise} (in infinity norm) close to rank-$1$ at the expansion stage. 
Such condition may e.g. provide insights that are useful for setting the value of the parameter $\delta$. 

\begin{proposition}\label{prop:necessary}
    Given $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$, and its rank-$1$ approximation $\estimate{\outputmat}$, in order for the entry-wise approximation error to be bounded by $\Delta$, the upper bound $\delta$ on the row-wise and column ratios must satisfy: 
    \[
    \delta < \frac{\Delta}{\min_{i,j}(\outputmat_{i,j})}
    \]
    %If the difference between any entry of the ratios of two rows or columns $\yvec$ and $\xvec$ of \outputmat is larger than $\tol$, then at least an entry-wise error incurred by the rank-$1$ approximation $\estimate{\outputmat}$ must be larger than $\Delta \min_{i,j}(\xvec_j, \xvec_i)$. 
\end{proposition}


Future work may take advantage of Proposition~\ref{prop:necessary} to develop a pruning strategy to retrieve a near-rank-$1$ matrix with strong entry-wise guarantees. 
\fi 

==> arXiv-2506.06456v1/additional_experimental_setup.tex <==
\spara{Datasets.}
To generate synthetic data,  we proceed as follows.
\begin{itemize}%\setlength{\itemsep}{0pt} 
    \item First, we generate vectors $\xvec \in \real^{\nrowssubmatrix}$ and $\yvec \in \real^{\ncolssubmatrix}$ according to a given probability distribution $\mathcal{P}$. 
    
    \item We then compute the rank-$1$ matrix $\outputmat = \xvec  \yvec^T \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$, and we inject additive noise generated according to the probability distribution $\mathcal{P}$, rescaled by a factor $\epsilon_{noise}$ and re-centered to have $0$ mean. The larger the parameter $\epsilon_{noise}$, the higher the noise and the more \outputmat deviates from a rank-$1$ matrix. 

    \item We finally generate a larger matrix $\inputmat \in \real^{\nrows \times \ncols}$ by resampling uniformly at random the entries of the sub\-matrix $\outputmat$ and planting the near-rank-$1$ sub\-matrix in randomly-sampled row indices $\rowset'$ and column indices $\colset'$.
\end{itemize}

The above data-generating mechanism is designed to make the task of near-rank-$1$ sub\-matrix recovery as challenging as possible. If the distribution of the entries in the  near-rank-$1$ sub\-matrix  deviates significantly from the remaining entries (or background), then co-clustering algorithms may suffice to discover the sub\-matrix.
We consider different choices for the distribution $\mathcal{P}$, namely standard normal, uniform in $[0,1]$, exponential of rate $1$, Beta with parameters $2$ and $3$, Gamma with shape $2$ and scale $1$ and Poisson of rate $5$. 

We always consider synthetic matrices $\inputmat \in \real^{\nrows \times \ncols}$ with $\nrows = 250$ and $\ncols=250$, and the parameter $\noisescale$ is set to $1^{-5}$, unless stated otherwise. 

In the experiments carried out to evaluate the performance of \ourmethod against the baselines, we first plant near-rank-$1$ square sub\-matrices of increasing size $\nrowssubmatrix \times \nrowssubmatrix$ with $\nrowssubmatrix \in \{  
25,50,75,100, 125 \}$. 

%In addition to the synthetic data with a single planted near-rank-$1$ sub\-matrix, we also consider the general setting where multiple near low-rank sub\-matrices are planted. 
In addition to the synthetic data with a single planted near-rank-$1$ sub\-matrix, we also consider the general setting that involves multiple planted near-rank-$1$ sub\-matrices.
More formally, we generate: 
\begin{equation*}
    \outputmat = \sum_{h = 1}^{N_{patterns}  }  \outputmat^*_h, 
\end{equation*}
where: 
\[
\outputmat^*_h =
\begin{cases}
 \outputmat_{h_{i,j}}, & \text{if } i \in \rowset_h \text{ and } j \in \colset_h \\
 0, & \text{otherwise},
\end{cases}
\]
and $\outputmat_h$ is generated as explained above and planted in row indices $\rowset_h$ and column indices $\colset_h$. 
In the experiments, we consider $N_{patterns} \in \{1,2,3,4,5\}$, and we sample $\nrowssubmatrix$ and $\ncolssubmatrix$ uniformly at random between $20$ and $75$. 
For the purposes of the experimental evaluation, it is assumed that each method is aware of the number of planted sub\-matrices. 
Thus, each method (iteratively) discovers $N_{patterns}$ 
sub\-matrices. In particular, \ourmethod follows the procedure sketched in Algorithm~\ref{alg:iterated}. 
A key point to highlight is that although all the generated matrices $\outputmat^*_h$ are close to rank $1$, they can overlap with each other, yielding intersection sub\-matrices that are close to a low-rank structure, but not necessarily close to rank $1$.  
The overlap between different planted sub\-matrices makes the task of discovering near-low-rank sub\-matrices more challenging than in the case of a single planted near-rank-$1$ sub\-matrix. 
In fact, in the absence of overlap between different planted sub\-matrices, our method can simply iteratively discover each sub\-matrix independently of the others. 

%Therefore, the case of $N_{patterns} > 1$ reflects the general setting of local low-rank-approximation. 



\iffalse 
where $\outputmat^*_i = $, and each $\outputmat_i$ is generated as explained above,
and we plant $\outputmat$ in a larger matrix obtained by resampling uniformly at random the entries of \outputmat. 
In these experiments, we generate $5$ submatrices $\nrowssubmatrix \times \ncolssubmatrix$, with $\nrowssubmatrix$ and $\ncolssubmatrix$ sampled uniformly at random between $20$ and $750$. 
\fi 


As concerns real-world datasets, we consider $15$ heterogeneous matrices coming from different domains. % that are common in the low-rank-approximation literature. 
Summary characteristics and references are provided in Table~\ref{tab:real_world_datasets} in Section~\ref{sec:exp_setup}. 
%Table~\ref{tab:real_world_datasets_appendix} shows the same characteristics for the other $12$ datasets considered in the experiments. 
We choose data matrices from different domains that are common in the low-rank-approximation literature. 
In particular, we consider benchmark  datasets for supervised-learning tasks (\Isolet, \Ozone, \Hearth), image datasets (\Olivetti, \OrlRnSp, \Mandrill and \Cameraman), 
benchmark datasets for recommender systems (\MovieLens, \Google and \MovieTrust), 
gene-expression data (\Golub and  \BRCA), neural-network weights (\Imagenet), and two miscellaneous datasets  (\Hyperspectral and \NPAS). 



%the real-world datasets used in
%our experimental analysis are given in %Table~\ref{tab:real_world_datasets}.

\iffalse 
\begin{table}[t]
\centering
\caption{\label{tab:real_world_datasets_appendix} Summary characteristics for real-world datasets. We report the number of rows, columns,  the low-rankness score, the entry-wise maximum squared deviation from the rank-1 \svd (Max rank-$1$ deviation) and a reference.}
    \label{tab:datasets}
    \begin{tabular}{lrrrrr}  % l = left-aligned, r = right-aligned
    \toprule
    {{{Dataset}}} & 
    {{~\# Rows}} & 
    {{~\# Columns}} & 
    {{~Low-rankness}} & 
    {{~Max rank-${1}$}} & 
    {{~Reference}} \\
    & & & {{score}} & {{deviation}} & \\
    \midrule
    \Isolet & 7797 & 617 & 0.88  & 0.98  & \cite{asuncion2007uci} \\
    \Olivetti & 400  & 4096 & 0.95  & 0.53  & \cite{asuncion2007uci} \\
    \OrlRnSp & 400 & 1024 & 0.95  & 0.55  & \cite{orl_faces} \\
    \Golub & 7129 & 38 & 1.00  & 0.28  & \cite{esposito2021review} \\
    \Mandrill & 512 & 512 & 0.92  & 0.36  & \cite{usc-sipi} \\
    \Ozone & 2536 & 72 & 1.00  & 0.08  & \cite{asuncion2007uci} \\
    \BRCA & 317 & 496 & 0.72  & 0.89  & \cite{tomczak2015review} \\
    \Google & 5456 & 24 & 0.76  & 0.77  & \cite{asuncion2007uci} \\
    \NPAS & 1418 & 78 & 0.85  & 0.15  & \cite{kaggle} \\
    \MovieTrust & 200 & 200 & 0.77  & 1  & \cite{kaggle} \\
    \Hearth & 920 & 15 & 0.94  & 0.08  & \cite{asuncion2007uci} \\
    \Imagenet & 64 & 27 & 0.92  & 0.22  & \cite{deng2009imagenet} \\
    \bottomrule
\end{tabular}
\end{table}
\fi 


\iffalse 
\begin{table}[t]
\centering
\caption{\label{tab:real_world_datasets_appendix} Summary characteristics for the real-world datasets used in the experiments. We report the number of rows, columns, a reference, the low-rankness score and the entry-wise maximum squared deviation from the rank-1 \svd.}
    \label{tab:datasets}
    \begin{tabular}{lrrrrr}  % l = left-aligned, r = right-aligned
        %\toprule
        %\textbf{Dataset} & \textbf{Rows} & \textbf{Columns} & 
        %\textbf{References} & 
        %\textbf{L-R Score} & \textbf{Max Rank-$\mathbf{1}$ Dev} \\
        %\midrule
        \toprule
        {{{Dataset}}} & 
        {{~\# Rows}} & 
        {{~\# Columns}} & 
        {{~Reference}} & 
        {{~Low-rankness}} & 
        {{~Max rank-${1}$}} \\
        & & & & {{score}} & {{deviation}} \\
        \midrule
        %\Hyperspectral & 5554 & 2151 & \cite{leone2022hyperspectral} & 0.89 & 0.23   \\
        \Isolet & 7797 & 617 &  \cite{asuncion2007uci} & 0.88  & 0.98  \\
        %Swamp & 7411 & 522 &  & 0.99  & 0.21  \\
        \Olivetti & 400  & 4096 & \cite{asuncion2007uci} & 0.95  & 0.53  \\
        %\MoiveLens & 943 & 1682 & \cite{kaggle} & 0.30  & 1.00  \\ 
        \OrlRnSp & 400 & 1024 & \cite{orl_faces} &  0.95  & 0.55  \\
        %Credit & 690 & 572 & \cite{asuncion2007uci}  &  1.00  & 0.00  \\
        %\Jester & 3000 & 101 & \cite{goldberg2020jester} &  0.91  & 0.88  \\
        \Golub & 7129 & 38 & \cite{esposito2021review} &  1.00  & 0.28  \\
        \Mandrill & 512 & 512 & \cite{usc-sipi} &  0.92  & 0.36  \\
        \Ozone & 2536 & 72 & \cite{asuncion2007uci} &  1.00  & 0.08  \\
        %\SKCM & 334 & 523 & \cite{tomczak2015review} &  0.76  & 0.85  \\
        \BRCA & 317 & 496 & \cite{tomczak2015review} &  0.72  & 0.89  \\
        % \PRAD & 337 & 457 & \cite{tomczak2015review} &  0.78  & 0.85  \\
        \Google & 5456 & 24 & \cite{asuncion2007uci} &  0.76  & 0.77  \\
        \NPAS & 1418 & 78 & \cite{kaggle} &  0.85  & 0.15  \\
        %\Cameraman & 256 & 256 & \cite{usc-sipi} & 
        %0.86  & 0.56  \\
        \MovieTrust & 200 & 200 & \cite{kaggle} & 
 0.77  & 1  \\
        \Hearth & 920 & 15 & \cite{asuncion2007uci} & 0.94  & 0.08  \\
        %Diabetes & 442 & 11 & \cite{asuncion2007uci} &  1.00  & 0.00  \\
        \Imagenet & 64 & 27 & \cite{deng2009imagenet} &   0.92  & 0.22  \\
        \bottomrule
    \end{tabular}
\end{table}
\fi 

\spara{Metrics.}
Here, we offer more details on the performance metrics adopted to assess the performance of \ourmethod against the baselines, which are briefly discussed in Section~\ref{sec:exp_setup}. 

When the ground truth is available, i.e., in synthetic data, we can assess the performance of a method in recovering the ground truth by the (balanced) $F_1$ score, which is a widely used metric in binary classification and information-retrieval tasks. 
The $F_1$ score corresponds to the the harmonic mean of precision and recall. 
Formally, it is 
defined as
\(
F_1 = \frac{2 \cdot \text{TP}}{2 \cdot \text{TP} + \text{FP} + \text{FN}}, 
\)
where TP, FP, FN are the true positives, false positives and false negatives, respectively. 
A method assigns a nonzero value to all the entries with indices in the discovered sub\-matrices and zero to the remaining entries. 
The nonzero values, in particular, are given by the low-rank approximation of the discovered sub\-matrices. 
A true positive occurs when a method assigns a nonzero value to an entry in a planted near-rank-$1$ sub\-matrix.
Similarly, a false positive occurs when the method assigns a nonzero value to an entry that is not part of a planted near-rank-$1$ sub\-matrix. Finally, false negatives correspond to those entries for which a method predicts a zero value in one of the entries that are part of a planted near-rank-$1$ sub\-matrix.

Given the ground truth, in addition to the $F_1$ score, it is of primary importance to assess the estimate of a planted sub\-matrix that is given by a method. 
For this purpose, we compute the reconstruction error, which is given by: 
\[
\frobeniusnormshort{\outputerror}^2 = 
\frobeniusnormshort{\outputmat - \estimate{\outputmat} }^2, 
\]
where  \outputmat is a ground-truth near-rank-$1$ sub\-matrix and $\estimate{\outputmat}$ its estimate. % given by any of the methods under comparison. 
The choice of the squared Frobenius norm is standard, but any other norm could be considered instead. 
To ensure that the error is comparable across sub\-matrices of varying sizes, we report the reconstruction error averaged over all entries of \outputmat. 

In real-world datasets no ground truth is available. 
In this case, there are two fundamental quantities that should be monitored; a measure of closeness to a low-rank matrix and a measure of size. 
The measure of closeness to a low-rank matrix is the crucial quantity. However, the size of the sub\-matrices is also important. %as larger sub\-matrices are preferable to smaller ones with similar proximity to a low-rank structure. 
%The idea is that sub\-matrices that are as close as possible to a rank-$1$ matrix and as large as possible should be preferred. 
The two quantities are typically inversely related;  it is always possible to obtain a perfectly rank-$1$ sub\-matrix by reducing its size, and vice versa, it is always possible to obtain a sub\-matrix as large as the input matrix by making it deviate more and more from a rank-$1$ sub\-matrix. 
Thus, a method is preferred over another whenever it strikes a more desirable balance between closeness to rank $1$ and size. 


As regards closeness to a rank-$1$ matrix,  we monitor the low-rankness score, introduced in Section~\ref{sec:preliminaries}. 
For a sub\-matrix $\outputmat \in \real^{\nrowssubmatrix \times  \ncolssubmatrix}$ with $i$-th singular value $\sigma_i^2$,   %\dots \sigma^2_{\min(\nrowssubmatrix,\ncolssubmatrix)}$, t
the low-rankness score is defined as 
\( \lowrankness{\outputmat} = 
    \frac{\sigma_1(\outputmat)^2}
         {\sum_{i=1}^{\min(\nrowssubmatrix,\ncolssubmatrix)} \sigma_i(\outputmat)^2} \). 
The low-rankness score has been adopted in previous work to monitor the performance in experiments with real-world datasets~\cite{dang2023generalized}. It mathematically equals the reciprocal of the popular stable-rank measure. 
%and has been adopted in the literature to measure the closeness of a matrix to rank-$1$ and the closer this measure is to $1$, the closer is the matrix to rank $1$. 
The low-rankness scores ranges between $0$ and $1$. The closer the low-rankness score is to $1$, the closer the sub\-matrix is to the ideal scenario of rank exactly $1$. 
It is important to consider the low-rankness of a sub\-matrix in relation to the input matrix it is extracted from. 
A sub\-matrix of size $\nrowssubmatrix \times \ncolssubmatrix$ with a low-rankness score of $0.95$ is extremely desirable if the low-rankness score of the input matrix is $0.3$. However, the same sub\-matrix is not as desirable when the  
low-rankness score of the input matrix is $0.9$. 
Therefore, to facilitate the understanding of the results, in addition to the raw low-rankness scores of the top-$5$ output sub\-matrices, we also report the average relative percentage increase in low-rankness with respect to the input matrix. 
The relative percentage increase in low-rankness is given by: 
\[
\frac{ \lowrankness{\outputmat}  - \lowrankness{\inputmat}    }{\lowrankness{\inputmat}}\cdot 100, 
\]
where $\lowrankness{\outputmat}$ and  $\lowrankness{\inputmat}$ indicate the low-rankness score of an output sub\-matrix $\outputmat$ and of the input matrix \inputmat, respectively. 
An important point to highlight is that, while the rank of a sub\-matrix can never exceed that of the larger matrix it is contained in, the low-rankness score of a sub\-matrix can be smaller than that of the matrix it is contained in.
Therefore, the relative percentage increase in low-rankness can be negative.



%An important point to highlight is that, while the rank of a sub\-matrix can never be larger than the rank of a larger matrix it is contained it, the low-rankness score of a sub\-matrix can. 


Finally, also for the size of an output sub\-matrix, %we simply count the number of entries in it, and 
as for the low-rankness score, it is important to consider the size of the sub\-matrix in relation to the size of the input matrix. 
Therefore, in addition to the raw number $|\outputmat|$ of entries in the top-$5$ output sub\-matrices, we report the percentage $\frac{|\outputmat|}{|\inputmat|} \cdot 100$ of entries in the input matrix that are part of the output sub\-matrix,
averaged over the top-$5$ output sub\-matrices. 

\spara{Parameters settings.}
In this paragraph, we provide more details concerning the parameter settings for the methods considered in the experiments. 

In Section~\ref{sec:exp_setup}, we discuss the values of the parameters $\tol$ and $\toleranceinit$ used in the experiments. 
In addition to $\tol$ and $\toleranceinit$, the other  important parameter to be given in input to \ourmethod is the target rank $\generalrank$. % which  to approximate the output sub\-matrices. 
If $\generalrank=1$, \ourmethod utilizes Algorithm~\ref{alg:rankone} to discover near-rank-$1$ sub\-matrices, otherwise it uses Algorithm~\ref{alg:rankk} to discover near-rank-$\generalrank$ sub\-matrices. 
%In line with previous work, we focus mostly on the case of rank-$1$ sub\-matrices. 
In the experiments with synthetic data, 
when the number of planted patterns is $1$, we consider $\generalrank =1$, when it is between $2$ and $4$, we consider  $\generalrank=1$ and $\generalrank=2$, and finally when there are $5$ patterns, we additionally consider  $\generalrank=3$.  %Algorithm~\ref{alg:rankk} with $\generalrank=3$. 
In all cases, however, the total number of initialization is $\nrep = 25$.  
In the case of real-world data, we always consider~$\generalrank=1$. 

Finally, the parameter $\lambda$ in the objective function $f$ controlling the relative weight of reconstruction error and size is held constant to its default value of $1$. 

As concerns the baselines, for sparse PCA, we set the sparsity-controlling parameter $\alpha$ to $1$.
In the convex-optimization-based approach, we set the parameter $\theta$ controlling the trade-off between nuclear and $L_1$ norm to $10$.
\svp is a parameter-free method. 
Finally, \rpsp samples $10^5$ $2 \times 2$ and $4 \times 4$ sub\-matrices and $10^4$ $8 \times 8$ and $16 \times 16$ sub\-matrices and  the number of score matrices that are computed (and summed up) before finding the final solution is set to $30$. 


\spara{Implementation details.}
We conclude this section by providing details regarding the implementation of \ourmethod and of the baseline approaches. 

An important choice for the implementation of \ourmethod is the approach leveraged to extract 
%a sub\-matrix with as many ones as possible from the the binary matrix \ind, or equivalently, 
a maximum-edge bi\-clique in the bipartite graph $\mathcal{G}_{\ind}$. 
In all the experiments with synthetic data, we 
leverage the algorithm of Lyu et al.~\cite{lyu2020maximum} for mining maximum-edge bicliques and we rely on an implementation in \textsc{C} of the algorithm available online.\footnote{\url{https://github.com/wonghang/pymbc}}

%extract maximum-edge biclique via the algorithm of Lyu et al.~\cite{lyu2020maximum} and we use rely

In the experiments with real-data, to eschew possible scalability issues, we heuristically extract dense submatrices from the indicator matrix \ind via spectral biclustering~\cite{kluger2003spectral}, which, as discussed in Section~\ref{sec:algorithms}, is the heuristic of choice to approximate maximum-edge bicliques. This algorithm is not guaranteed to return   
sub\-matrices of \ind consisting of all ones (i.e., bi\-cliques). 
%Therefore, 
%the dense subgraphs of $\mathcal{G}_{\ind}$ extracted via spectral bi\-clustering may not be cliques, and s
Subsequently, the guarantees reported in Theorem~\ref{th:expansion} may not hold when spectral bi\-clustering is used. 
Despite the lack of theoretical guarantees, the implementation of \ourmethod using spectral biclustering is effective in practice, as demonstrated by our experiments.

To approximate the discovered sub\-matrices, we use the interpretable approximation in terms of the original rows or columns of the data if the target rank is~$1$ and the \svd otherwise. 



%This means that the guarantees~\ref{}
\iffalse 
%except in a few datasets (Jester, SKCM1, BRCA1, PRAD1) where particularly dense indicator matrices occur and biclustering returns too large submatrices so that we prefer the simple greedy heuristic that iteratively removes the row or column from the indicator matrix with the least ones until the density exceeds a threshold that we set to $0.9$. 
\fi 
For spectral biclustering, we use the implementation available in the \textsc{scikit-learn} \textsc{Python} library.\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.cluster.SpectralBiclustering.html}}


To handle sparse datasets, we also implement particular constraints that avoid returning trivial rank-$1$ sub\-matrices consisting of all zeros. 


%Finally, in the experiments investigating the impact of $\tol$ in~\ref{ap:additional_experiments}, to extract dense submatrices from $\ind$, we use the algorithm of Lyu et al.~\cite{lyu2020maximum} for $\tol \leq 0.1$ and biclustering otherwise. 

%\iffalse 
%In the experiments with synthetic data, we rely on an implementation of the maximum-biclique-extraction algorithm of Lyu et al.~\cite{lyu2020maximum} available online~\footnote{\url{https://github.com/wonghang/pymbc}}. 
%Instead, in the experiments with real-data, we heuristically extract an approximation of a maximum-edge biclique using 
%\fi 
As for the baselines, we implement \svp in \textsc{Python}. 
For \rpsp, we instead rely on the implementation provided by the authors.\footnote{\url{https://github.com/ptdang1001/RPSP}}
%Both \rpsp and our method can take advantage of parallel computing to speed up execution; for the purposes of our evaluation, however, we do not rely on it. 
For \sparsePCA and for the convex-optimization approach (\cvx), we use the \textsc{scikit-learn}\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.decomposition.SparsePCA.html}} and \textsc{cvxpy}\footnote{\url{https://www.cvxpy.org}} \textsc{Python} libraries, respectively. 
















%possibly expressing it as percentages of the total number of entries in the input matrices. 



==> arXiv-2506.06456v1/additionalexperiments.tex <==
In this section, we present additional experimental results. 
First, we present preliminary experiments, and then we present additional results of experiments evaluating the performance of the method we introduce in both synthetic and real data. 

\spara{Preliminary experiments.}
%\cnote[MC]{Candidate for removing?}
%In preliminary experiments, we investigate salient characteristics of the synthetic data generated as explained in Section~\ref{sec:exp_setup}. 
The goal of the preliminary experiments is to 
provide valuable insights into the synthetic data used in our experiments, and on the behavior of \ourmethod in such data. 

We first consider a full-rank $250 \times 250$ matrix with all i.i.d. entries generated from a standard normal distribution and no planted near-rank-$1$ sub\-matrix. 
%the distributions listed in~\ref{ap:additional_experimental_setup
For such matrix, in Figure~\ref{fig:prelimary_full_rank},  we show the distribution of the determinants of the initially-sampled $2 \times 2$ matrices as well as the probability of hitting a near-rank-$1$ $2 \times 2$ sub\-matrix with near-zero determinant as a function of the parameter $\toleranceinit$ (with $ \toleranceinit \in \{ 10^{-8}, 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4} \}$). 
%to be expanded in the second phase of \ourmethod
Finally, we show the average reconstruction error $\frobeniusnorm{\outputerror}^2$ of the sub\-matrices retrieved by \ourmethod as a function of the proportion of entries of the input matrix they include. 
As Figure~\ref{fig:prelimary_full_rank} suggests, although the input matrix is generated completely at random and with no planted near-rank-$1$ sub\-matrix, it still contain many $2 \times 2$ sub\-matrices with near-zero determinant, and the probability of \ourmethod hitting a near-rank-$1$ $2 \times 2$ sub\-matrix in the initialization phase quickly grows as the initial tolerance parameter $\toleranceinit$ is increased, 
confirming the intuition gained through the simple probabilistic analysis presented in Section~\ref{sec:analysis}. 
However, no large matrix with small reconstruction error is found at the expansion phase, since, unlike in real-world matrices, it is unlikely that large low-rank sub\-matrices occur in matrices consisting solely of i.i.d. entries. % in m with entries generated i.i.d. according to a given distribution. 

Figure~\ref{fig:prelimary_planted} presents similar results as Figure~\ref{fig:prelimary_full_rank}, but for a synthetic $250 \times 250$ matrix where a near-rank-$1$ sub\-matrix is generated from a standard normal distribution and planted according to the procedure illustrated in~\ref{ap:additional_experimental_setup}. 
In particular, for such matrix, the figure shows the distribution of the values in the planted near-rank-$1$ sub\-matrices and in the background, the probability that \ourmethod samples a near-rank-$1$ $2 \times 2$ sub\-matrix in the initialization phase as a function of the parameter $\toleranceinit$ (with $ \toleranceinit \in \{ 10^{-8}, 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4} \}$) and the average reconstruction error as a function of the $F_1$ score for the sub\-matrices output by our method in different iterations. 
The figure demonstrates that the planted near-rank-$1$ sub\-matrices are drawn from the same distribution as the background, reflecting a scenario where standard co-clustering algorithms are generally not able to identify low-rank sub\-matrices. 
Furthermore, the figure also demonstrates that the probability of hitting a near-rank-$1$ $2 \times 2$ sub\-matrix is generally larger than in the case of Figure~\ref{fig:prelimary_full_rank} since the planted near-rank-$1$ sub\-matrices contain a large number of $2 \times 2$ rank-$1$ sub\-matrices. 
Finally, the figure confirms that \ourmethod expands many initial sub\-matrices into larger matrices with $F_1$ score close to $1$ and reconstruction error close to $0$, suggesting that the ground-truth sub\-matrix is recovered in many iterations. 
%As shown next, this is not necessarily the case for the baseline approaches. 
%, there is significant variability in the results associated with different data-generating distributions. 



\begin{figure}[t]
\begin{center}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_normal_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_normal_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_normal_0_100_0001.pdf} \\
        \iffalse
        & \textsc{Uniform} & \\
         \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_uniform_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_uniform_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_uniform_0_100_0001.pdf} \\

        & \textsc{Exponential} & \\
         \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_exponential_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_exponential_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_exponential_0_100_0001.pdf} \\

        & \textsc{Beta} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_beta_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_beta_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_beta_0_100_0001.pdf} \\

        & \textsc{Gamma} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_gamma_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_gamma_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_gamma_0_100_0001.pdf} \\

        & \textsc{Poisson} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/twobytwo_determinants_poisson_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_poisson_0_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_poisson_0_100_0001.pdf} \\
        \fi 
        \vspace*{-1.1cm}
    \end{tabular}
\end{center}
\caption{
\label{fig:prelimary_full_rank}
Full-rank $250 \times 250$ synthetic matrix with i.i.d entries from a standard normal distribution and without planted near-rank-$1$ sub\-matrices.
We show the distribution of $2 \times 2$-sub\-matrix determinants (left), the probability of observing a $2 \times 2$-sub\-matrix with determinant in absolute value lower than the initial tolerance threshold $\toleranceinit$  as a function of $\toleranceinit$ (center) and the (per-entry) average reconstruction error as a function of the proportion of entries in the sub\-matrix for individual iterations of our method (right). 
}
\end{figure}


\begin{figure}[t]
\begin{center}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_normal_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_normal_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_normal_25_100_0001_v2.pdf} \\
        \iffalse
        & \textsc{Uniform} & \\
         \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_uniform_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_uniform_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_uniform_25_100_0001_v2.pdf} \\

        & \textsc{Exponential} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_exponential_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_exponential_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_exponential_25_100_0001_v2.pdf} \\

        & \textsc{Beta} & \\
         \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_beta_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_beta_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_beta_25_100_0001.pdf} \\

        & \textsc{Gamma} & \\
         \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_gamma_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_gamma_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_gamma_25_100_0001_v2.pdf} \\

        & \textsc{Poisson} & \\
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/histogram_distribution_poisson_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/prob_poisson_25_100_0001.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/preliminaryExperiments/scatterplot_poisson_25_100_0001.pdf} \\
        \fi 
        \vspace*{-1.1cm}
    \end{tabular}
\end{center}
\caption{
\label{fig:prelimary_planted}
Full-rank synthetic $250 \times 250$ matrix generated from a standard normal distribution and with a $25 \times 25$ planted near-rank-$1$ submatrix.
We show the distribution of the values in the entire matrix and sub\-matrix (left), the probability of observing a $2 \times 2$-sub\-matrix with determinant in absolute value lower than the initial tolerance threshold $\toleranceinit$ as a function $\toleranceinit$ (center) and the (per-entry) average reconstruction error as a function of the $F_1$ score for individual iterations of our method (right). 
}
\end{figure}






\begin{figure}[t!]
    \begin{tabular}{cccc}
        \textsc{\Hyperspectral} & 
        \textsc{\OrlRnSp} & \textsc{\Mandrill} & \textsc{Normal} \\
        \includegraphics[width=0.24\textwidth]{images/size_by_lowrankness_v3_leone_h.pdf} & 
        
        \includegraphics[width=0.24\textwidth]{images/size_by_lowrankness_v3_orlRnSp_h.pdf} & 
        \includegraphics[width=0.24\textwidth]{images/size_by_lowrankness_v3_mandrill_h.pdf} & 
        \includegraphics[width=0.24\textwidth]{images/size_by_lowrankness_v3_normal_h.pdf} \\
        \vspace*{-0.7cm}
    \end{tabular}
\caption{\label{fig:impact_of_delta}Experiments on four example datasets (\Hyperspectral, \OrlRnSp, \Google and a $250 \times 250$ synthetic dataset with i.i.d normally-distributed entries)
%entries drawn i.i.d. from a standard normal distribution)
to investigate the impact of $\tol$ on the output of \ourmethod.
Each point indicates the low-rankness score and the percentage of entries of the discovered sub\-matrices  %(averaged over $30$ runs) 
for a given value of $\tol$, with $\tol \in \{10^{-6}, 10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}.$}
%\cnote[MC]{We might need to move this figure to avoid it taking its own page.}
\end{figure}




\spara{Experiments on synthetic and real-world data: impact of tolerance parameter.}
The results provided by \ourmethod vary with $\tol$. 
%depend on an important parameter, $\tol$. 
Intuitively, this parameter indirectly bounds the approximation error and thereby it embodies the trade-off between sub\-matrix size and low-rankness. 
In more detail, a larger value of $\tol$ leads to denser indicator matrices $\ind$ and thus larger output sub\-matrices $\outputmat$. 
On the other hand, a smaller value of $\tol$ leads to generally smaller output sub\-matrices $\outputmat$ which, however, may have higher low-rankness. 
In practice, \ourmethod returns high-quality results across reasonable choices of $\tol$. 
In Figure~\ref{fig:impact_of_delta} we show, for four examples example datasets (\Hyperspectral, \OrlRnSp, \Mandrill and a synthetic $250 \times 250$ matrix with  i.i.d.  entries drawn from a standard normal distribution and no planted near-rank-$1$ sub\-matrices), the low-rankness score against the size of the sub\-matrices output by \ourmethod for different choices of the parameter $\tol$. 
%Specifically, we vary $\tol$ in $\{ [1^{-5}, 1^{-4}, 1^{-3}, 1^{-2}, 1^{-1}, 0.25, 0.5, 0.75, 1\}$. 
Specifically, we vary $\tol$ in $\{ 10^{-5}, 10^{-4}, 10^{-3}, 10^{-2}, 10^{-1} \}$. 
As for all the experiments in real-world datasets, the results in Figure~\ref{fig:impact_of_delta} are obtained by relying on spectral bi\-clustering for approximating maximum-edge bi\-cliques. As a consequence, it is not guaranteed that larger values of $\tol$ lead to larger size and lower low-rankness.   
Nevertheless, the results confirm that, also in the case where maximum-edge bi\-cliques are approximated,  larger values of $\tol$ generally result in sub\-matrices of larger size and lower low-rankness. 
Moreover, \ourmethod outputs high-quality sub\-matrices for any appropriate choice of $\tol$. 





\spara{Experiments on synthetic data: impact of noise.}
To demonstrate the robustness of \ourmethod to noise, Figure~\ref{fig:noise} shows results for the performance of different methods in near-rank-$1$ sub\-matrix recovery as the level of noise increases. 
We use the same experimental setup as for the results shown in Figure~\ref{fig:near_rank_one_recovery}, except that the dimension of the planted ground-truth near-rank-$1$ sub\-matrix is held fixed to $75 \times 75$ and the scale of the noise $\noisescale$ is varied in $\{  10^{-8}, 10^{-7}, 10^{-6}, 10^{-5}, 10^{-4}  \}$. 
The figure highlights that, in this setting, \ourmethod and \rpsp outperform the other baselines. Most importantly, the results resemble those shown in Figure~\ref{fig:near_rank_one_recovery} for planted sub\-matrices of size $75 \times 75$, confirming that \ourmethod is fairly robust to noise.  


\iffalse 
Figure~\ref{fig:near_rank_one_recovery} in Section~\ref{sec:exp_results} reports results in the experiments where the goal is to detect a single planted near-rank-$1$ sub\-matrix for data drawn from a standard normal distribution. 
Figure~\ref{fig:near_rank_one_recovery_appendix} reports analogous results for the other five distributions considered in our experimental evaluation. 
\begin{figure}[t]
\begin{center}
\input{images/tikz/legend_with_svp}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Uniform} & \\
         \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_uniform_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_uniform_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_uniform_125_250_1e05_4.pdf} \\

        & \textsc{Exponential} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_exponential_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_exponential_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_exponential_125_250_1e05_4.pdf} \\


        & \textsc{Beta} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_beta_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_beta_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_beta_125_250_1e05_4.pdf} \\


        & \textsc{Gamma} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_gamma_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_gamma_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_gamma_125_250_1e05_4.pdf} \\


        & \textsc{Poisson} & \\
         \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_poisson_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_poisson_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_poisson_125_250_1e05_4.pdf} \\
    \end{tabular}
\end{center}
\caption{
\label{fig:near_rank_one_recovery_appendix}
Full-rank synthetic $250 \times 250$ matrices generated from different distributions with planted near-rank-$1$ submatrices.
Performance of different methods in the task of near-rank-$1$ submatrix discovery.  
We show the average (per-entry) reconstruction error (left), the $F_1$ score (center) and the runtime (right) of different methods as a function of planted submatrix size.
}
\end{figure}
Similarly, Figure~\ref{fig:local_low_rank_approximation_by_submatrices} in Section~\ref{sec:exp_results} and Figure~\ref{fig:local_low_rank_approximation_by_submatrices_appendix} display the same metrics as in  Figure~\ref{fig:near_rank_one_recovery}, but in the scenario where multiple near-rank-$1$ matrices are planted, for data generated from a standard normal distribution (Figure~\ref{fig:local_low_rank_approximation_by_submatrices}) and for the other five probability distributions we generate synthetic data from (Figure~\ref{fig:local_low_rank_approximation_by_submatrices_appendix}). 
\fi 

\iffalse 
Figure~\ref{fig:local_low_rank_approximation_by_submatrices} in Section~\ref{sec:exp_results} displays the same metrics as Figure~\ref{fig:near_rank_one_recovery}, in the scenario where multiple near-rank-$1$ matrices are planted, for data generated i.i.d. from a standard normal distribution.
displays the same results for the other five probability distributions we generate synthetic data from.
\fi 

\iffalse 
The results shown in Figures~\ref{fig:near_rank_one_recovery_appendix}~and~\ref{fig:local_low_rank_approximation_by_submatrices_appendix} largely confirm those shown in Section~\ref{sec:exp_results} for normally-distributed data. \ourmethod is fast and, unlike the baselines, consistently retrieves the ground-truth planted sub\-matrices. 
\fi 





\iffalse 
\begin{figure}[t]
\begin{center}
\input{images/tikz/legend_with_svp}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Uniform} & \\
         \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_uniform_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_uniform_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_uniform_5_250_1e05_4.pdf} \\

        & \textsc{Exponential} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_exponential_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_exponential_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_exponential_5_250_1e05_4.pdf} \\


        & \textsc{Beta} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_beta_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_beta_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_beta_5_250_1e05_4.pdf} \\


        & \textsc{Gamma} & \\
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_gamma_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_gamma_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_gamma_5_250_1e05_4.pdf} \\


        & \textsc{Poisson} & \\
         \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_poisson_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_poisson_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_poisson_5_250_1e05_4.pdf} \\
    \end{tabular}
\end{center}
\caption{
\label{fig:local_low_rank_approximation_by_submatrices_appendix}
Full-rank synthetic $250 \times 250$ matrices generated from different distributions with planted near-rank-$1$ sub\-matrices.
Performance of different methods in discovering multiple planted near-rank-$1$ sub\-matrices. 
We show the average (per-entry) reconstruction error (left), the $F_1$ score (center) and the runtime (right) of different methods as a function of the number of (possibly overlapping) planted sub\-matrices. 
}
\end{figure}
\fi 

\begin{figure}[p]
\begin{center}
\input{images/tikz/legend_with_svp}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_normal_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_normal_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_normal_75_250_001_4.pdf} \\
        & \textsc{Uniform} & \\
         \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_uniform_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_uniform_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_uniform_75_250_001_4.pdf} \\
        & \textsc{Exponential} & \\
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_exponential_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_exponential_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_exponential_75_250_001_4.pdf} \\
        & \textsc{Beta} & \\
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_beta_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_beta_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_beta_75_250_001_4.pdf} \\
        & \textsc{Gamma} & \\
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_gamma_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_gamma_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_gamma_75_250_001_4.pdf} \\
        & \textsc{Poisson} & \\
         \includegraphics[width=0.3\textwidth]{images/plotsNoise/avg_rec_error_by_noise_with_svp_poisson_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/f1_scores_by_noise_with_svp_poisson_75_250_001_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/plotsNoise/runtimes_by_noise_with_svp_poisson_75_250_001_4.pdf} \\
        \vspace*{-0.65cm}
    \end{tabular}
\end{center}
\caption{
\label{fig:noise}
Full-rank synthetic $250 \times 250$-matrices generated from different distributions with planted near-rank-$1$ submatrices of dimensions $75 \times 75$.
Performance of different methods in the task of near-rank-$1$ submatrix discovery. 
We show the average (per-entry) reconstruction error (left), the $F_1$ score (center) and the runtime (right) of the different methods under comparison as a function of the noise scale \noisescale.
The $x$-axis is on logarithmic scale. 
}
\end{figure}







\begin{figure}[p]
\begin{center}
\input{images/tikz/legend_only_rpsp}
    \begin{tabular}{ccc}
        \textsc{\Hyperspectral} & \textsc{\Isolet} & \textsc{\Olivetti} \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_leone_with_yaxislabs_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_isolet_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_olivetti_h.pdf} \\
        \textsc{\MovieLens} & \textsc{\OrlRnSp} &     \textsc{\Golub} \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_rating_with_yaxislabs_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_orlRnSp_h.pdf} & 
        %\includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_jester.pdf} \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_golub_h.pdf} \\
        \textsc{\Mandrill} & \textsc{\Ozone} & \textsc{\BRCA} \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_mandrill_with_yaxislabs_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_ozone_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_BRCA1_h.pdf} 
        \\
       %\textsc{\SKCM} & \textsc{\BRCA} & \textsc{\PRAD}  \\
       % \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_SKCM1_with_yaxislabs.pdf} & 
       % \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_BRCA1.pdf} & 
       % \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_PRAD1.pdf} \\
         \textsc{\Google} & \textsc{\NPAS} & \textsc{\Cameraman}  \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_google_reviews_with_yaxislabs_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_NPAS_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_cameraman_h.pdf} \\
        \textsc{\MovieTrust} & \textsc{\Hearth} & \textsc{\Imagenet} \\
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_movie_trust_with_yaxislabs_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_hearth_h.pdf} & 
        \includegraphics[width=0.33\textwidth]{images/plotsRealData/barchart_less_text_with_svp_imagenet_h.pdf} \\
        \vspace*{-0.65cm}
    \end{tabular}
\end{center}
\caption{\label{fig:real_data_top_five_patters} Real-world datasets. Low-rankness score and size for each of the top-$5$ sub\-matrices discovered by different methods.}
\end{figure}



\spara{Experiments on real-world data: fine-grained results.}
Table~\ref{tab:results_real_data} shows average low-rankness and size of the top-$5$ low-rank sub\-matrices retrieved by our method, \rpsp and \svp for three datasets. 
%Table~\ref{tab:results_real_data_appendix} shows analogous results for the other datasets considered in our empirical evaluation. 
%The results shown in Table~\ref{tab:results_real_data_appendix} reinforce the findings of the real-data experiments presented in Section~\ref{sec:experiments}. 
%In particular, although the results vary across datasets, they suggest that \ourmethod achieves an unprecedented balance between low-rankness and size. 
%\svp is very fast and returns sub\-matrices of large size. However, the low-rankness of the sub\-matrices returned by \svp is often smaller than that of the input matrix. 
%\svp is very fast. However, it often identifies sub\-matrices with lower low-rankness than the input matrix. 
In addition, Figure~\ref{fig:real_data_top_five_patters} provides a more fine-grained picture of the results of the experiments  for all real-world datasets, showing the raw low-rankness score and the size (i.e., the number of entries) of each of the individual top-$5$ sub\-matrices retrieved by \svp, \rpsp and \ourmethod. 
Note that, in three datasets (\NPAS, \Ozone and \Hearth), for \svp, results for less than $5$ sub\-matrices are shown because \svp is not able to discover five distinct sub\-matrices. 
%It is also interesting to look at the single top sub\-matrix since this eliminates the differences that may arise by the different strategies followed by the methods to deliver more than one sub\-matrix. 



\iffalse 
\begin{table}[t!]
\centering
\caption{\label{tab:results_real_data_appendix} Performance in real-world data. For the top $5$ local low-rank patterns identified by the methods, we show the average relative percentage increase (L-R) with respect to the low-rankness score of the input matrix, the size (in percentage of entries of the input matrix) and the runtime (in seconds) to obtain them.}
    \begin{tabular}{l ccc ccc ccc}
        \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{\svp}  & \multicolumn{3}{c}{\rpsp} & \multicolumn{3}{c}{\ourmethod} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
        & L-R & Size & Runtime & L-R  & Size & Runtime & L-R & Size & Runtime \\
        \midrule
        %\Hyperspectral  & 0.92 & 2.88 & 46.67 & 0.98 & 2.1 & 590 & 0.99 & 21.43 & 1696 \\
        \Isolet & -8.08 & 3.21 & 11 & 4.06 & 3.51 & 409 & 7.08 & 9.9 & 650 \\ 
        %Swamp & 0.99 & 2.19 &  9.32 & 1.00 & 0.03  & 364 & 1.00 & 0.05 & 502 \\
        \Olivetti & -1.39 & 4.3 & 3 & 2.23 & 2.81 & 366 & 3.83 & 5.2 & 207 \\ 
        % \MoiveLens & 0.44 & 8.59 & 1.45 & 0.43 &  2.85 & 124 & 0.61 & 1.13 & 121 \\
        \OrlRnSp & -1.51 & 4.39 & 1 & 2.84 & 1.92 & 386 & 3.65 & 4.29 & 58 \\  
        %Credit & 0.92 & 3.93  & 322 & 1.00 & 14.10 & %2792 \\
        %\Jester & 0.65 & 3.72 & 3.52 & 0.96 & 0.02  & 264 & 0.96 & 0.14 & 47 \\
        \Golub & -0.32 & 0.29 & 15 & 0.01 & 2.39 & 161 & 0.07 & 19.43 & 61 \\ 
        \Mandrill & 3.25 & 2.3 & 1 & 6.53 & 2.37 & 404 & 6.14 & 3.16 & 43 \\ 
        \Ozone & -39.92 & 0.74 & 2 & 0.03 & 3.23 & 211 & 0.16 & 16.76 & 24 \\ 
        %\SKCM & 0.82 & 5.25 & 0.43  & 0.85 & 0.03  & 295 & 0.9 & 0.03 & 24 \\
        \BRCA & 11.39 & 5.17 & 0 & 14.19 & 2.18 & 371 & 4.97 & 39.44 & 29 \\ 
        %\PRAD &  0.83 & 4.23 & 0.36 & 0.84 & 0.03  & 308 & 0.85 & 0.06 & 25 \\
        \Google & 11.22 & 4.4 & 4 & 18.78 & 2.55 & 145 & 22.63 & 7.16 & 17 \\ 
        \NPAS & -71.29 & 15.86 & 0.2 & 8.55 & 3.93 & 246 & 17.57 & 19.52 & 23 \\ 
        %\Cameraman & 0.87 & 3.64 & 0.32 & 0.91 & 0.03  & 102 & 0.98 & 0.25 & 18 \\
        \MovieTrust & -2.37 & 4.05 & 0.3 & -20.79 & 4.23 & 209 & 22.49 & 10.49 & 10 \\  
        \Hearth & -16.31 & 2.72 & 0 & 5.13 & 3.63 & 107 & 3.89 & 20.9 & 5 \\ 
        %Diabetes & 0.99 & 0.04  & 88 & 1.00 & 0.35 & 3 \\
       \Imagenet & 3.44 & 4.85 & 0.4 & 5.26 & 3.98 & 126 & 8.52 & 2.29 & 31 \\ 
        \bottomrule
    \end{tabular}
\end{table}
\fi 



\iffalse 
\begin{table}[t]
\scriptsize
\centering
\caption{\label{tab:results_real_data_appendix} Performance in real data. For the top $5$ local low-rank patterns identified by the methods, we show the low-rankness score (L-R Score), the size (in percentage of entries) and the runtime (in seconds) to obtain them. }
    \begin{tabular}{l ccc ccc ccc}
        \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{\svp}  & \multicolumn{3}{c}{\rpsp} & \multicolumn{3}{c}{\ourmethod} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
        & L-R Score & Size & Runtime & L-R Score & Size & Runtime & L-R Score & Size & Runtime \\
        \midrule
        %\Hyperspectral  & 0.92 & 2.88 & 46.67 & 0.98 & 2.1 & 590 & 0.99 & 21.43 & 1696 \\
        \Isolet & 0.81 & 3.21 & 11.40 &  0.92  & 3.51  & 409 & 0.95 & 9.90 & 650 \\
        %Swamp & 0.99 & 2.19 &  9.32 & 1.00 & 0.03  & 364 & 1.00 & 0.05 & 502 \\
        \Olivetti &  0.94 & 4.30 & 3.16 & 0.98 & 0.03  & 366 & 0.99 & 0.05 & 207 \\
        % \MoiveLens & 0.44 & 8.59 & 1.45 & 0.43 &  2.85 & 124 & 0.61 & 1.13 & 121 \\
        \OrlRnSp & 0.93 & 4.38 &  0.63 & 0.98 & 0.02  & 386 & 0.99 & 0.04 & 58 \\
        %Credit & 0.92 & 3.93  & 322 & 1.00 & 14.10 & %2792 \\
        \Jester & 0.65 & 3.72 & 3.52 & 0.96 & 0.02  & 264 & 0.96 & 0.14 & 47 \\
        \Golub  & 0.99 & 0.29 & 14.72 & 1.00 & 0.02  & 161 & 1.00 & 0.19 & 61 \\
        \Mandrill &  0.95 & 2.29 &  1.17 & 0.98  &  2.37 & 404  &  0.98 & 3.16 &  43 \\ 
        \Ozone  & 0.6 & 0.73 & 1.87 & 1.00 & 0.03  & 211 & 1.00 & 0.17 & 24 \\
        \SKCM & 0.82 & 5.25 & 0.43  & 0.85 & 0.03  & 295 & 0.9 & 0.03 & 24 \\
        \BRCA & 0.80 & 5.16 & 0.33 & 0.83 & 0.02  & 371 & 0.85 & 0.06 & 29 \\
        \PRAD &  0.83 & 4.23 & 0.36 & 0.84 & 0.03  & 308 & 0.85 & 0.06 & 25 \\
        \Google & 0.84 & 4.40 & 3.88 & 0.90 & 0.03  & 145 & 0.93 & 0.07 & 17 \\
        \NPAS & 0.24 & 15.85 & 0.22 & 0.92 & 0.04  & 246 & 1.00 & 0.20 & 23 \\
        %\Cameraman & 0.87 & 3.64 & 0.32 & 0.91 & 0.03  & 102 & 0.98 & 0.25 & 18 \\
        \MovieTrust & 0.74 & 4.05 & 0.26 & 0.61 & 4.23  & 209 & 0.94 & 10.5 & 9 \\      
        \Hearth & 0.78 & 2.72 & 0.38 & 0.99 & 0.04  & 107 & 0.97 & 0.21 & 5 \\
        %Diabetes & 0.99 & 0.04  & 88 & 1.00 & 0.35 & 3 \\
        \Imagenet & 0.95 & 4.85 & 0.41 & 0.96 & 0.04 & 126 & 0.99 & 0.02 & 31 \\
        \bottomrule
    \end{tabular}
\end{table}
\fi 






%as $\tol$ grows, our method identifies larger sub\-matrices, often at the cost of lower low-rankness. 


==> arXiv-2506.06456v1/algorithms_arxiv.tex <==
\section{Algorithms}\label{sec:algorithms}
In this section, we present \ourmethod, our method for discovering near-low-rank sub\-matrices. We first give an overview of the method, and then we present the algorithms to detect near-rank-$1$ and near-rank-\generalrank sub\-matrices.
%Once such sub\-matrices are detected, one can obtain an approximation via \svd. 
%  and is supported by approximation-quality guarantees illustrated in the following section.   %Section~\ref{sec:analysis}.  
% The approximation given by the \svd will incur at most the same error in terms of Frobenius and spectral norm~\cite{chipman2020proofs}, but not necessarily in terms of infinity norm. 

% \cnote[MC]{ The following paragraph presenting the  the general procedure from a high level (i.e. initialization + expansion - shared by all the different algorithms rank-1/rank-k, affine etc) used to be called "The general framework.". If you prefer the previous title or something else over the current title, we can change it again.   Also should we have phase or stage of the method, i.e. the method has two stages or phases? Which one you prefer? Previously "stage", switched to  "phase", but this ideally requires updating the abstract in the submission page too (which should be allowed).  }
%- however should we say the general "method"? i am not sure, we could call this paragraph "The high-level method" for example and then use method instead of framework - current .}

\subsection{High-level Overview of the Method}\label{sec:algo_overview}
\ourmethod is based on a simple two-phase procedure.
The first phase \emph{samples} small {seed} sub\-matrices, 
and the second phase \emph{expands} those seed sub\-matrices into larger near-low-rank sub\-matrices.

The main idea relies on the simple principle that any sub\-matrix of a rank-$k$ matrix 
must also have rank at most $k$. 
Thereby, a near-rank-$1$ sub\-matrix \outputmat of size $\nrowssubmatrix \times \ncolssubmatrix$ 
contains a large number of $2 \times 2$ near-rank-$1$ sub\-matrices. 
% Analogously, a near-rank-$k$ sub\-matrix \outputmat of size $\nrowssubmatrix \times \ncolssubmatrix$ contains multiple   $(\generalrank+1) \times (\generalrank +1)$ near-rank-$k$ sub\-matrices. 
Thus, if we are looking for a rank-1 sub\-matrix, 
in the first phase (initialization or sampling phase) we identify a \emph{seed}, 
% which is a \emph{minimal} subset of entries 
which is a $2 \times 2$ submatrix 
that can expanded into a larger sub\-matrix that is still close to a rank-1 approximation. 
The goal of the second phase (or expansion phase) is to expand the seed into a large near-rank-1 sub\-matrix. 
Similarly, if we are looking for a near-rank-$\generalrank$ sub\-matrix, in the first phase we identify a seed sub\-matrix of minimal size that is close to rank $\generalrank$. 
In the second phase, the seed is expanded as much as possible while preserving the proximity to rank $\generalrank$. 

\iffalse 
The details of the sampling and expansion phase of \ourmethod for the algorithm specialized to near-rank-$1$ sub\-matrix detection and for the algorithm for general near-rank-$\generalrank$ sub\-matrix detection, described later, are different. 
\fi 



%In the second phase, the seed is expanded deterministically 

%The second phase instead aims at expanding the seed into a larger submatrix while preserving the closeness to rank-\generalrank. 

The two-phase procedure is repeated~\nrep\ times, to explore different random initializations. 
Each repetition outputs a near-low-rank sub\-matrix \outputmat.
\ourmethod accepts a parameter $\tol$ that controls the trade-off between proximity to a low-rank approximation and size of the output matrices.  
%The larger $\tol$, the larger in size and further away from their low-rank approximation the output sub\-matrices tend to be. 
Higher values of $\tol$ tend to yield sub\-matrices that are larger but deviate more from a low-rank structure. 

%In practice, it is convenient to explore different values of $\tol$. 

%that
% , as explained in Section~\ref{sec:analysis}, is provably 
%is close to low rank. 
After the last repetition, we return the sub\-matrix \outputmat that maximizes the objective function %$\f{\outputmat}$, defined as 
% For each output sub\-matrix, we compute the value of an objective function $\f{\outputmat}$, and after the last repetition, we return the sub\-matrix maximizing the objective function.
% The objective function is defined as follows: 
% \begin{equation}
%    \label{eq:objective}
$\f{\outputmat} = \abs{\outputmat} - \frac{\lambda}{\abs{\outputmat}} \frobeniusnormshort{\outputerror}^2$. 
% \end{equation}
% This design of the objective function allows the user to tailor the search for low-rank sub\-matrices to their own needs by prioritizing approximation error or sub\-matrix size. 
By default, in the absence of prior information, we standardize the error term and the size, and set $\lambda=1$. 
However, \ourmethod is flexible and supports any 
objective function. 
%other reasonable objective function can be used.
% in place of the one in Equation~\ref{eq:objective} 
% and our method remains unchanged.   

\iffalse 
For the objective function, we use a weighted sum of the squared reconstruction error $\frobeniusnormshort{\outputerror}^2$ incurred in low-rank approximation and the size $| \outputmat |$. 
\fi 



\iffalse
During the expansion phase, the method returns a matrix \outputmat that maximizes a criterion, 
which captures the trade-off between size and low-rankness. 
By default, we use a weighted sum of squared reconstruction error (i.e., the squared Frobenius norm of \outputerror) and size. 
We normalize both the error and the size, and subsequently, we use an unweighted sum.
%  (e.g., by computing z-scores). 
Another criterion we explore is the minimum between (normalized) size and (normalized) low-rankness, instead of the sum. 
\fi 
%The above two phases are repeated a number $N_{rep}$ times, and the largest submatrices is finally returned. 

\iffalse
All the sub\-matrices \outputmat returned by our method,  
satisfy the bounds specified in the problems \nearrankone and \nearrankk, and hence, 
submatrix size is the primary~interest. 
% one can also simply select the largest detected sub\-matrix. 
\fi 

% \cnote[AG]{From the paragraph above it is not clear what is the criterion to return the submatrix. From our call today I understand that we are using the minimum, rather than the sum. }

% \cnote[MC]{Good point;  I have re-phrased everything. 
%
%I am not sure whether there is any "preferable" objective. I have tried both. And the method works with any choice of objective.  Clearly the sum has the advantage that we can control how much we care about size vs low-rankness. 
%I think we can speak about sum only to make it more clear. 
%The minimum between low-rankness and size is reserved to find top 5 submatrices in  real-data experiments  for different methods (it is also independent of the approximation) }


The high-level pseudocode of the \ourmethod method is given in~Algorithm~\ref{alg:general}.
The details of the initialization and expansion phase of the method for the algorithm specialized to near-rank-$1$ sub\-matrix detection and for the algorithm for general near-rank-$\generalrank$ sub\-matrix detection, described later, are different. 


\input{pseudocodes/general}

\spara{Approximating the discovered sub\-matrices.}
The discovered sub\-matrices can be approximated via \svd. 
Further, %as discussed in~\ref{ap:interpretable}, 
\ourmethod also naturally leads to a low-rank approximation that is more interpretable than the \svd since it is based on the rows (or columns) of \outputmat. 
%it expresses each row (column) of \outputmat %as a linear function of the anchor rows (columns).  
For the rank-$1$ case, this approximation is given by $\estimate{\outputmat} = \xvec \yvec^T$, where, either $\yvec^T$ is a row or $\xvec$ a column of $\outputmat$. If, e.g., $\yvec^T$ is a row of \outputmat, $\xvec$  can be chosen to minimize \( \frobeniusnormshort{\outputmat - \xvec \yvec^T}^2 \). The resulting optimal $\xvec$ is the vector of coefficients that describe the orthogonal projections of the rows of \outputmat onto $\yvec^T$. An analogous argument also applies to the columns. 
As discussed in Section~\ref{sec:analysis}, this approximation is supported by quality guarantees. 

%and the result is given by the orthogonal projection of the rows of \outputmat onto $\yvec^T$. 
Although the rank-$1$ \svd may be more accurate than the interpretable alternative, if a matrix is sufficiently close to rank $1$, the difference is typically negligible. To gain some intuition for this claim, note that a matrix that has exactly rank $1$ can be represented with no error not only by the discussed interpretable approximation, but also by the rescaled outer product \( \alpha \outputmat_{:,j}  \outputmat_{i,:}^T \) of any of its rows and columns, for some $\alpha \in \real$.  If instead the matrix deviates significantly from  rank $1$, the rank-$\generalrank$ interpretable approximation based on orthogonal projections is often not as accurate as the rank-$\generalrank$ \svd. 

%than the \svd is the preferred approach. 

\spara{Discovering multiple sub\-matrices.}
%So far we have described how \ourmethod discovers a low-rank sub\-matrix.
In practice, we may wish to discover multiple sub\-matrices within a single matrix \inputmat and eventually obtain an approximation $\estimate{\inputmat}$ of the matrix as sum of local low-rank patterns. To achieve this, we run \ourmethod iteratively. In each iteration, the method finds a single near-rank-$\generalrank$ sub\-matrix, and then updates $\estimate{\inputmat}$ and the input matrix for the next iteration. This simple procedure is summarized in~Algorithm~\ref{alg:iterated}. 

\input{pseudocodes/iterated}

%Moreover, this approximation 



%since it can be expressed as a linear function of rows and columns of the original output sub\-matrix. 


%Notably, the quality guarantees hold for an interpretable approximation that 
%The details of such approximation are given in~\ref{ap:interpretable}. 
%The rank-$1$ \svd approximation will incur lower error in terms of Frobenius and spectral norm~\cite{chipman2020proofs}, but may incur larger error in terms of max norm.
%~\ref{ap:additional_analysis} presents interesting bounds for the spectral norm of \outputerror incurred by the rank-$1$ \svd. 




\iffalse
%Thus, if we are looking for a rank-$1$ submatrix, we initialize the algorithm by identifying a minimal submatrix of rank $k$ or lower. 
In the remainder of this section, 
we explain how we can leverage this general framework to identify near-rank-$1$ sub\-matrices, as well as more general near-rank-$k$ sub\-matrices, 
possibly up to a translation. 
The near-rank-$1$ case is particularly interesting due to its practical applications, more interesting analysis, and more efficient algorithms.
\fi 

\subsection{Recovering a Near-rank-1 Sub\-matrix}
\label{sec:algo_rank1}

\iffalse
The case of rank-$1$ sub\-matrices is of primary importance. 
We thus introduce an algorithm dedicated to the case of rank-$1$ sub\-mHeratrices that is particularly efficient. 
The algorithm phases are also summarized in~\ref{ap:pseudocode} (Algorithm~\ref{alg:rankone}). 
\fi

Here, we present the initialization (sampling) and expansion phases of the algorithm to discover near-rank-$1$ sub\-matrices. Algorithm~\ref{alg:rankone} presents the pseudo\-code.  


\input{pseudocodes/rankone}



%also summarized in~\ref{ap:pseudocode} (Algorithm~\ref{alg:rankone}). 

\spara{Initialization.}
To find the initial $2 \times 2$ near-rank-$1$ sub\-matrix $\initialmat$, we sample
two distinct row indices $\{i_1,i_2\}$ and  column indices $\{j_1,j_2\}$ of the input matrix \inputmat,
and then we compute the determinant of the associated $2 \times 2$ sub\-matrix $\initialmat'$:  
\begin{equation*}
   \abs{\det(\initialmat')} = \abs{\inputmat_{i_1, j_1} \inputmat_{i_2,j_2} -  \inputmat_{i_1, j_2} \inputmat_{i_2,j_1} }. 
\end{equation*}
If $\abs{\det(\initialmat')} \leq \toleranceinit$,
for some input $\toleranceinit \in \real^+$,  $\initialmat'$
is close to rank $1$, and hence it may be contained into a larger near-rank-$1$ sub\-matrix.
Therefore, $\initialmat'$ is the seed $\initialmat$ that will be expanded. 
If instead $\abs{\det(\initialmat')} > \toleranceinit$, we sample different $2 \times 2$ sub\-matrices $\initialmat'$ until we find a seed to expand.  
In practice, \toleranceinit is initialized to a small value ($10^{-11}$ by default) and progressively increased until the seed is found. 
%into a larger sub\-matrix.
%  in the expansion phase.



\iffalse
To find the initial $2 \times 2$ near-rank-$1$ sub\-matrix $\initialmat$, we need to find a $2 \times 2$ sub\-matrix where the rows and the columns are nearly proportional. 
This condition is conveniently captured by the determinant of the $2\times2$ sub\-matrix. 
Therefore, to find \initialmat, we sample  two entries $(i_1,j_1)$ and $(i_2, j_2)$ of \inputmat, and we compute the determinant of the $2 \times 2$ sub\-matrix $\initialmat'$ that has such entries along the main diagonal. This determinant is given by: 
\begin{equation*}
   |\det(\initialmat')| = \abs{\inputmat_{i_1, j_1} \inputmat_{i_2,j_2} -  \inputmat_{i_1, j_2} \inputmat_{i_2,j_1} }. 
\end{equation*}
If $ \det(\initialmat') \leq \toleranceinit$, this suggest that $\initialmat'$ may be contained into a larger near-rank-$1$ sub\-matrix.
Thus, we have found the seed \initialmat that will be expanded into a larger sub\-matrix in the expansion phase.
\fi 



\spara{Expansion.}
To extend \initialmat into a larger sub\-matrix, %  while preserving the closeness to a low-rank structure, 
we consider one of the entries $(\anchorindexrow, \anchorindexcol)$ in \initialmat, which we call \emph{anchor}. 
Then, we divide all rows in \inputmat by the $\anchorindexrow$-th row, obtaining the row-wise ratio matrix 
$\rowratios$ and 
% $\rowratios \in \real^{n \times m}$
all columns by the $\anchorindexcol$-th column, obtaining the column-wise ratio matrix 
$\columnratios$. 
% $\columnratios \in \real^{n \times m}$
If an entry in the $\anchorindexrow$-th row or $\anchorindexcol$-th column of \inputmat is zero, we add a small positive constant to prevent division by zero. 

%we ensure that the denominators contain no zero entries by adding a small positive constant too all zero entries. 
As illustrated in Figure~\ref{fig:ratios_diagram}, if the matrix \inputmat contains a sub\-matrix \outputmat of rank $1$, 
the entries corresponding to \outputmat in \rowratios and \columnratios will be row-wise and column-wise constant, respectively.
More generally, as we explain in in Section~\ref{sec:analysis}, 
bounding the variation in all the row-wise and column-wise ratios in a sub\-matrix leads to quality guarantees for its rank-$1$ approximation. 
Therefore, the goal of the expansion stage is to identify a sub\-matrix of maximum size with bounded variation in the row-wise and column-wise ratios. 
%and 
%similarly the entries corresponding to \outputmat in %\columnratios will be column-wise constant. 

To this end, our algorithm examines the rows of \rowratios to find subsets of near-constant entries including column~$\anchorindexcol$ and 
the columns of \columnratios to find subset of near-constant entries including row $\anchorindexrow$. 
More specifically, for an input parameter $\tol \in \real^+$, 
we select, for each row of \rowratios, the $\anchorindexcol$-th entry and all other entries such that the maximum variation is less than $\tol$ in absolute value. Similarly, for each column of \columnratios, we select  the $\anchorindexrow$-th entry and all other entries such that the maximum variation is less than $\tol$ in absolute value. 
%that deviate by the $j$-th element less than $\tol$ in absolute value, and we select for each column all the entries that deviate by the $i$-th element less than $\tol$ in absolute value. 
Subsets within each row can be efficiently retrieved by sorting the row elements by their absolute deviation from the $\anchorindexcol$-th element and analogously for the columns. 
% Specifically, 


\begin{figure}[t]
\centering
\begin{tabular}{c@{\hspace{1.25cm}}c@{\hspace{1.25cm}}c} % Adjust spacing here
    \scalebox{0.55}{\input{diagrams/D.tikz}} &
    \scalebox{0.55}{\input{diagrams/ratios_rows.tikz}} &
    \scalebox{0.55}{\input{diagrams/ratios_columns.tikz}} \\
    \inputmat & \rowratios & \columnratios
\end{tabular}
\caption{\label{fig:ratios_diagram}
Example of row-wise (\rowratios) and column-wise (\columnratios) ratio matrices associated with an input matrix (\inputmat) containing a rank-$1$ sub\-matrix (highlighted in red). 
Within this rank-$1$ sub\-matrix, the entries of $\rowratios$ are constant across rows, and the entries of $\columnratios$ are constant across columns.
}
%Row-wise and column-wise ratios with a rank-1 sub\-matrix (in red).}
\end{figure}

%To find a sub\-matrix with bounded variation in the row-wise and column-wise ratios, 

Given the identified subsets, we construct two indicator matrices: $\indrows \in {0,1}^{\nrows \times \ncols}$, where the entries with value $1$ correspond to subsets of near-constant row-wise ratios; and $\indcols \in {0,1}^{\nrows \times \ncols}$, where the entries with value $1$ correspond to subsets of near-constant column-wise ratios.
\iffalse 
we create an indicator matrix $\indrows\in \{0,1\}^{\nrows \times \ncols}$ where the entries with value $1$  represent the previously identified subsets of near-constant row-wise ratios and an indicator matrix $\indcols\in \{0,1\}^{\nrows \times \ncols}$ where the $1$s  represent the previously identified subsets of near-constant column-wise ratios. 
\fi 
%we represent the outcome of the selection step in the form of an indicator matrix  for the row-wise ratios and % an indicator matrix 
% for the column-wise ratios. 
%
We can then compute the intersection of the two matrices $\indrows$ and $\indcols$ to obtain the intersection indicator matrix $\ind$ of the same dimensions. 
% The intersection operation exploits the symmetry in rank-$1$ matrices where both rows and columns are proportional, resulting in stronger guarantees and better empirical performance, although, in practice, one can obtain sensible results while considering only the rows or the columns. 
%Because, as formalized in the following section, sub\-matrices with all row-wise and column-wise ratios having bounded variations indicate near-rank-$1$ sub\-matrices, 
The problem of extracting a sub\-matrix  of maximum size  with all row-wise and column-wise ratios with bounded variations can then be framed as the problem of finding the largest possible all-ones sub\-matrix within \ind.
This problem is equivalent to the extraction of a  maximum-edge bi\-clique~\cite{lyu2020maximum} from the bipartite graph $\mathcal{G}_\ind$ that has \ind as adjacency matrix. 
%If we regard the matrix  of a bipartite graph  the problem under consideration is equivalent to the extraction of a maximum-edge bi\-clique from such bipartite graph. 
%The matrix \ind can be regarded as the adjacency matrix of a bipartite graph. 
%Then,  . 
Although this is an \np-hard problem~\cite{lyu2020maximum}, so that it cannot be solved in polynomial time, we can leverage recent algorithmic advances that solve the problem quickly in considerably dense and large bipartite graphs~\cite{lyu2020maximum}. 
In addition, to avoid possible scalability issues that may still arise, we also rely on effective heuristics, as discussed in Section~\ref{sec:scalability}. 

\iffalse
\cnote[AG]{Two questions that probably need to addressed in this section:\\
1. Should we say something about how to select the anchor? Does it matter?\\
2. Since bi-clique is \np hard, any ``recent algorithmic advances'' are heuristics. How does this affect our theoretical guarantees?}
\cnote[MC]{1. I am not sure about anchor selection: we have only used random sampling. 
I am not sure if there is a better strategy (probably no time to discuss this topic in depth); however, as discussed in later notes, the value of $\delta$ could be adpated based on the anchor row/column to make the bounds constant. Perhaps it makes more sense to adapt to $\delta$ to an anchor row than the other way around.  
2. See later note. But in general this is also an important point that we overlook; the error guarantees rely on the assumption that we extract a biclique (it does not matter if it is maximal but if it is not a biclique the error bounds could not hold). We should say this clearly. 
}
\fi


\subsection{Recovering a Near-rank-$\generalrank$ Sub\-matrix}
\label{sec:algo_general_susbpace}
% The method presented in the previous section does not extend straightforwardly to the recovery of near-rank-$k$ sub\-matrices. 
Next, we illustrate the adaptation of the initialization (sampling) and expansion phases of \ourmethod to the general case of recovery of near-rank-$k$ sub\-matrices. 
% However, our general two-phase framework can be adapted to the recovery of near-rank-$k$ sub\-matrices. 
% In the first phase, we identify a minimal candidate (seed) for a local near-rank-$k$ sub\-matrix, and in the second phase we expand the seed into a larger sub\-matrix. 
The pseudo\-code % of the algorithm to retrieve (provably) near-rank-$k$ sub\-matrices 
is given in Algorithm~\ref{alg:rankk}. 
\input{pseudocodes/rankk}


\spara{Initialization.}
To find a seed, that is, a minimal near-rank-$k$ sub\-matrix, 
we sample matrices with $k+1$ rows and columns 
until we find a matrix $\initialmat$ that, as indicated by a near-zero determinant, is close to rank $k$ or lower, and thus represents the seed to expand in the second phase. 
In particular, to determine whether a matrix $\initialmat'$ has rank $\generalrank$ or lower, we check whether $|\det(\initialmat')| \leq \toleranceinit$, for a small $\toleranceinit \in \real^+$, which, as for the algorithm tailored to near-rank-$1$ sub\-matrices, is first initialized to a to a small value and then increased until a seed \initialmat is found.   

\iffalse
\cnote[AG]{
The part below (expansion) is difficult to parse in English. 
Maybe it would be easier (and shorter and less ambiguous) to write using standard math notation. 
E.g.,  ``we construct the matrix $\initialmats$ that has the sampled rows as columns.'' $\Rightarrow$ use matrix transpose, etc.    
}

\cnote[MC]{
Thank you for noticing; i agree. I have re-written the following paragraph (expansion phase). I switched to a more intuitive explanation. The computation formulas are still visible in the pseudocode if needed.    
}
\fi

\spara{Expansion.}
Given the seed matrix $\initialmat \in \real^{\generalrank+1, \generalrank+1}$, of rank $\generalrank' \leq \generalrank$, we 
sample $\generalrank'$ anchor rows from the rows of $\initialmat$. Let $\initialmatcols$ denote the set of the $\generalrank + 1$ indices of the columns in $\initialmat$.  % and 
%$\initialmatrows$ be the set of the $\generalrank'$ indices of the anchor rows. 
%Such rows, also referred to as anchor rows, serve as the basis of a $\generalrank'$-dimensional subspace, and the goal of the expansion stage is to identify subsets of points that are close to such subspace  .
Considering only the columns in $\initialmatcols$, we compute the coefficients of the orthogonal projection of each row of \inputmat onto the subspace spanned by the $\generalrank'$ anchor rows. 
\iffalse 
We then compute the orthogonal projection of each each row subset $\inputmat_{i, \initialmatcols}$ onto the subspace spanned by the %{\color{red}two}
\fi 

We then compute the matrix of orthogonal projections $\estimate{\inputmat}^{\perp} \in \real^{\nrows \times \ncols}$ expressing each row as a linear combination of the anchor rows with weights given by the orthogonal-projection coefficients. 
The coefficients are obtained by considering only the columns in $\initialmatcols$, identified in the initialization phase. Nevertheless, the matrix $\estimate{\inputmat}^{\perp} \in \real^{\nrows \times \ncols}$, similarly to the ratio matrices in the rank-$1$ case, indicates which additional columns and rows are close to a rank-$\generalrank$ approximation. More specifically,
all entries $\inputmat_{i,j}$ that are closely approximated by $\estimate{\inputmat}^{\perp}_{i,j}$ lie close to the $\generalrank$-dimensional subspace identified in the initialization phase.


Therefore, to find a near-rank-\generalrank sub\-matrix of maximum size, we need to identify the largest sub\-matrix of $\estimate{\inputmat}^{\perp}_{i,j}$ where all entries nearly match the corresponding entries of \inputmat. 
To obtain such a sub\-matrix, we calculate the matrix of absolute errors $\errors = | \inputmat - \estimate{\inputmat}^{\perp} |$, and from it, the indicator matrix $\indrows$, which takes value $1$ for entry $\generalentry$ if $\errors_{i,j} \leq \tol$ and $0$ otherwise, for some input $\tol \in \real^+$.
Figure~\ref{fig:linear_combination_diagram} presents an example of the matrices $\estimate{\inputmat}^{\perp}$ and $\errors$. % while 
%Figure~\ref{fig:example_plane} illustrates $3$-dimensional data with varying distance to their orthogonal projection in a plane identified in the initialization phase. 

The same procedure followed to determine $\indrows$, 
but on input $\inputmat^T$ and $\initialmat^T$ yields~${\indcols}$ . 
Similarly to the case of near-rank-$1$ sub\-matrix discovery, the intersection of $\indrows$ and~${\indcols}^T$ gives the matrix $\ind$ and the associated bipartite graph $\mathcal{G}_{\ind}$. 
The desired output near-rank-$\generalrank$ sub\-matrix is then given by a sub\-matrix of $\ind$ consisting of all ones, or, equivalently, by a maximum-edge bi\-clique of $\mathcal{G}_{\ind}$. 


\begin{figure}[t]
\centering
\begin{tabular}{c@{\hspace{1.25cm}}c@{\hspace{1.25cm}}c}
    \scalebox{0.55}{\input{diagrams/D2.tikz}} &
    \scalebox{0.55}{ \input{diagrams/linear_combs.tikz}} &
     \scalebox{0.55}{\input{diagrams/E.tikz}} \\
     \hspace*{0.2cm}\inputmat & \hspace*{0.2cm}$\estimate{\inputmat}^\perp$ & \hspace*{-0.4cm}\errors \\
\end{tabular}
\caption{\label{fig:linear_combination_diagram}
Example of matrices of projections ($\estimate{\inputmat}^\perp$) and absolute errors (\errors) associated with an input matrix (\inputmat) containing a rank-$\generalrank$ sub\-matrix (highlighted in red). Within this rank-$\generalrank$ sub\-matrix, the entries of $\estimate{\inputmat}^\perp$ are equal to those of \inputmat, and the entries of $\errors$ are all identically zero. 
}
\end{figure}


\subsection{Scalability Considerations}\label{sec:scalability}
One limitation of \ourmethod is its reliance on solving the maximum-edge biclique problem, 
which is  \nphard. 
While the algorithm we use to extract these bicliques is often efficient in practice~\cite{lyu2020maximum}, scalability issues may still arise.
%in general, 
%scalability issues arise as the size of the input matrix increases.
%
To address such issues, % a key advantage of the methods we introduce over previous work is the flexibility:
the algorithm for finding maximum-edge bicliques can be replaced with a more scalable heuristic.  
%The general framework in Algorithm~\ref{alg:general} provides a flexible framework that can be adapted to different purposes. 
%Nevertheless, 
Among many possible different heuristic approaches, by default,
we rely on spectral bi\-clustering~\cite{kluger2003spectral}, which is empirically found to be particularly effective in quickly identifying a dense sub\-matrix of \ind.
%  applied to the matrix \ind, which is particularly effective. 
Even more efficient and scalable approaches include
\iffalse 
efficient algorithms for extracting dense subgraphs in bipartite graphs~\cite{sariyuce2018peeling}, 
\fi 
algorithms to extract dense bipartite subgraphs, 
a greedy algorithm removing rows and columns from \ind, e.g., based on the  amount of ones, and a randomized algorithm sampling sub\-matrices from \ind according to the amount of ones they contain~\cite{boley2011direct}. 
A comprehensive evaluation of the performance of various heuristics for approximating maximum-edge bicliques is left to future work.




%If the chosen heuristic is not guaranteed to return a bi\-clique, however, the analysis presented in Section~\ref{sec:analysis} may not hold.. 

%More details on spectral bi\-clustering, the greedy algorithm, and other possible heuristic approaches are provided 
%{\color{red}in~\ref{ap:heuristics}.} 

\iffalse
\cnote[AG]{I am guessing that the biclique algorithm we are using is exact but exponential in the worst case. 
This needs to be made more explicit.}
\cnote[MC]{This is a very good question i have been thinking about. There is no mention in the paper of anything related to output quality. I assumed the paper would find actually optimal solutions by pruning the search space a lot. This intuition of mine comes also from the fact that there is also no guarantee of polynomial time (the worst-case is exponential). Which i have also observed in the experiments. Note: only the synthetic-data experiments use this algorithm; this algorithm does not scale to large and dense graphs, hence the heuristics (real-data experiments use spectral biclustering algorithm). 
}
%\cnote[MC]{We can give more details here but in the appendix}
%In particular, a limitation of our methods is that they require solving maximum-edge biclique, an \nphard problem. 
%While the algorithm that we use to extract such bicliques tends to be efficient in practice, scalability issues may arise, as the number of edges and bicliques in the input graph grows.
\fi

%Other possible choices of heuristic approach are discussed in Appendix~\ref{ap:heuristics}. 


\iffalse
\subsection{Putting everything together: iterated local low-rank approximation}

The algorithms presented in Sections~\ref{sec:algo_rank1}~and~\ref{sec:algo_general_susbpace} pave the way for an iterative procedure for the more general task of local low-rank approximation, where the goal is to obtain a representation of the input matrix as a sum of local low-rank patterns.

At each iteration, the iterative procedure invokes Algorithm~\ref{alg:rankone}~and~\ref{alg:rankk} for different ranks $\generalrank$ and 
subsequently select the submatrix that optimizes a criterion combining low-rankness. 

%and selects a single matrix that optimizes an objective function combining a measure of low-rankness and the size of the submatrix, analogous to the objective function considered in Algorithm~\ref{alg:rankone}~and~\ref{alg:rankk}. 

%In particular, for each output submatrix, we compute low-rankness and size. 
%Then, we standardize the values of low-rankness and size (subtracting the mean and dividing by the standard deviation). 
%Finally we select submatrices based on a combination of the standardized low-rankness score and size. Standardizaton ensures that both size and low-rankness weight on the selection. 
%Alternatively, we may select submatrices to maximize the minimum between low-rankness score and size, which often results in submatrix striking a more desirable balance between the two objectives. 

The selected sub\-matrix is subtracted from the input matrix. 
This deflation operation ensures that the identified low-rank pattern is not considered in subsequent iterations of the algorithm. 
The pseudocode of the algorithm is given in~\ref{ap:pseudocodes}, where we define the subroutine \textsc{FindLowRankSubmatrix}, which represents Algorithm~\ref{alg:rankone} if the input rank is $1$ and Algorithm~\ref{alg:rankk} otherwise. 

\fi


% Recovery near-rank-$k$ submatrices 

==> arXiv-2506.06456v1/analysis_arxiv.tex <==
\section{Analysis}\label{sec:analysis}
%In this section, we study the theoretical aspects of the method we introduce. 
%In Section~\ref{sec:experiments}, we present experiments evaluating the performance of our methods in practice. 
%In Section~\ref{sec:algorithms}, we have described a method to discover near-rank-$1$ or near-rank-$\generalrank$ submatrices. 
In this section, we explain how the proposed methods yield sub\-matrices 
with bounded approximation error.
% satisfying the requirements specified in Problem~\ref{prob:rank-1}~and~\ref{prob:rank-k}. 
We also provide a brief discussion on the probabilistic aspects and on the computational complexity of the methods.

%of the method and computational comple
%However, we have not explained how the method we hav

%We begin by presenting results on the guarantees provided by our methods regarding the error incurred in approximating the retrieved submatrices. 
%Specifically, we discuss how the algorithms illustrated in Section~\ref{sec:algorithms} yield submatrices of bounded spectral, Frobenius and infinity norm. 

%In addition, we briefly discuss the computational complexity of the methods and provide a simple probabilistic analysis of their randomized components.

\iffalse
\cnote[AG]{Below it was written: 
``We are primarily interested in \emph{entry-wise} approximation-error guarantees (i.e., in terms of infinity norm).''
However, the matrix infinity norm is not ``\emph{entry-wise}.''
The definition, also given in the preliminaries, is 
$\infinitynormshort{\inputmat} = \max_i\sum_j |\inputmat_{i,j}|$.
I have rephrased it now, removing the word ``\emph{entry-wise}.''
}
\cnote[MC]{The infinity norm definition that we are considering is entry-wise (no sum). Now it is called max-norm, which is more precise. }
\fi

\subsection{Approximation Error Guarantees}

%\cnote[AG]{I do not understand the first sentence below. 
%What does it mean ``approximate only matrix entries that admit a faithful low-rank representation''? 
%A single matrix entry does not admit a ``faithful low-rank representation''.
%The low rank is a property of a whole matrix (or, submatrix), not of a single entry.\\
%Consequently, I do not really agree with the argument being made 
%that the max norm is more intuitive/appropriate for our problem, 
%than Frobenius and spectral.
%}

\iffalse 

\cnote[MC]{
Thank you for noticing. 
The argument i wanted to make is the following: 
the \svd and other methods for global low-rank approximation find a representation of the entire input matrix. 
In this representation, no matter if optimal in frob/specral norm, some entries can be very far from the corresponding entry in the original matrix. In terms of data points and dimensions for example, a data point may be badly misplaced in its lower-dimensional even if the projection onto the svd susbapace is optimal in frob/specral norm. 
For example the rank-1 svd may capture very well the 80 percent of the data that get accurate projection onto it. The remaining 20 percent might not be captured well at all (it would by increasing the rank of the svd). 
In view of this, i wanted to express that an important motivation underlying our work is that we do not necessarily need to approximate the entire matrix. We can drawback of global methods and only approximate those entries that *we know* can be approximated to little error. This is a strong guarantee that global approaches like svd cannot achieve. 

I am not sure if you understand what i mean, i will try to rephrase in any case. 
We could of course avoid saying anything about this max norm central role, however it is also nice for the rank k algorithm that gives interesting guarantees on max norm only.
}

\cnote[AG]{\\
 $\gg$ i wanted to express that an important motivation underlying our\\
 $\gg$ work is that we do not necessarily need to approximate the entire\\
 $\gg$ matrix.\\
 OK, but this is achieved by considering a submatrix, instead of the whole matrix. 
 I am still not convinced that the max norm has a special place.     
}

\cnote[MC]{\\
    I understand that the max norm has not a special place. However it gives a very "strong" guarantee. For global low-rank approximation it may not be meaningful, e.g., if the data has a single outlier optimizing a global low rank approximation for  the max norm would be terrible. However, in our case, it is certainly interesting and (in some inuitive sense) poses stronger requirement that frob/spectral norm. 
    Let us then avoid to convey that the max norm has a special place, but simply remark that it is interesting/strong. 
}
\cnote[AG]{OK, I let you proceed with finalizing the section according to this plan.\\
Btw, the ``strong'' guarantee of max norm may also be a drawback, in the sense that max norm is sensitive to outliers: a single entry that is off could be sufficient to mislead you, and suggest large error, while in reality that could be only one outlier.
}

\cnote[MC]{Yes, i rephrased. I undersstand this point. But i can imagine that it can be interesting to have approximation that do not include outliers at all and all entries are close "enough" in the low-rank approximation. Of course approximating for the max norm would be bad also in our case.   
}
\fi 

% As discussed, a crucial aspect of the methods we introduce is that they yield submatrices with bounded low-rank approximation error. 

\iffalse 
In this work, we seek to approximate only matrix entries that admit a faithful low-rank representation. 
\fi 
%A drawback of global low-rank approximation methods like the \svd is that, 


%An important advantage of approaches to local low-rank approximation like \ourmethod over techniques that compute 
%Unlike approaches to global low-rank approximation, \ourmethod does not need to approximate all rows and columns of a matrix. 
In global low-rank approximation, 
the presence of outliers in the data may lead to situations where
the whole matrix cannot be approximated with a low-rank structure 
without compromising the overall approximation quality. 
However, as our problem definition lifts the requirement that the whole matrix must be approximated, 
it is interesting to control the \emph{entry-wise} maximum approximation error in the discovered sub\-matrices. 
%techniques like the \svd optimize 
%do not provide guarantees in terms of maximum approximation error. 
%average out errors across the entire matrix
%A global low-rank approximation optimized for the maximum error w extremely sensitive to outliers. 
%If the data consist of 
We thus provide
% \emph{entry-wise} 
approximation-error guarantees in terms of the max norm.
%  since a fundamental principle underlying our work is that only those matrix entries that admit a faithful representation in terms of a low-rank structure should be approximated. 
%In this work, we only want to approximate those matrix entries  
%The primary objective of this work is thus to have an \emph{entry-wise} approximation-error guarantee (i.e., in terms of infinity norm). 
%i.e., we want each entry to be provably close to its low-rank approximation. 
%However, in addition to the infinity norm, it is also desirable to bound the Frobenius and spectral norms. 
%guarantees on the entry-wise approximation error also result in bounded error in terms of Frobenius or spectral norm.
%In the case of near-rank-$1$ matrices,  moreover, Algorithm~\ref{alg:rankone} is additionally supported by approximation error guarantees in terms of Frobenius norm that are tighter than those implied by the infinity-norm guarantees. 
A bound on the max norm yields  bounds on the Frobenius and spectral norms, albeit loose.
In the case of near-rank-$1$ sub\-matrix discovery, 
we also provide interesting bounds on the spectral and Frobenius norms  that are not a direct consequence of the bound on the max~norm. 
%The case of near-rank-$1$ submatrices leads to a particularly interesting analysis. 
%Specifically, in the case of near-rank-$\generalrank$ submatrix recovery, approximation-error guarantees for the spectral and Frobenius norm are derived from th


% Specifically, in this case, we can derive approximation-error guarantees for Algorithm~\ref{alg:rankone} in terms of Frobenius and spectral norm that can be tighter than those implied by the infinity-norm. 

\iffalse 
\cnote[AG]{
Can we already refer to our methods by a name, 
instead of Algorithm~\ref{alg:rankone} and Algorithm~\ref{alg:rankk}?
Also, maybe we should avoid character '\&' (as in \ourmethod)? 
It could be, perhaps, SE, or \textsc{SnE}, or \textsc{SampleAndExpand}.
}
\cnote[MC]{
Ok. Perhaps SampleAndExpand is reasonably short (will try). Otherwise we can switch. It is however needed to distinguish between rank $1$ and rank $k$ algorithms (same method, two different algorithms). The theorem applies to the outputs of only the algorithm specialized to the rank-1 case. Thus to be precise we should say something like " the near-rank-$1$ submatrices returned by \ourmethod "  to refer to the specialized algorithm. 
}
\fi 


%Let us consider first the initialization stage of Algorithm~\ref{alg:rankone}. 
%As also formalized in~\ref{ap:proofs}, 

\iffalse
\cnote[AG]{Martino: the following paragraph is difficult for me to understand.
The sentences are too convoluted and too cryptic. 
Would it be possible to rewrite it in simpler terms and with very simple sentences?
Some examples of what does not work:\\ 
``As also formalized in~\ref{ap:proofs},'' we should avoid pointing to core statements in the appendix, 
only additional results that can be skipped by the reader.\\
``implicitly defines'' why implicitly? this is ambiguous. Everything should be explicit.\\
``The condition imposed in the ratios in the expansion phase'' the reader may not remember what you are talking about \\
``at its core'' this is ambiguous.\\
``the provable proximity'' ?
}
\cnote[MC]{
I re-write everything. 
}
\cnote[AG]{
Just the next paragraph. The rest is OK.
}
\fi 

\iffalse 
The bound that \ourmethod imposes on the absolute value of the $2 \times 2$ determinants in the initialization phase implicitly defines a notion of closeness to rank $1$, and $2 \times 2$ matrices with near-zero determinants are provably close to a rank-$1$ approximation.
The condition imposed in the ratios in the expansion phase is, at its core, a rescaled variant of the determinant condition. Thereby, the provable proximity to a rank-$1$ approximation is preserved in the expansion phase, as formalized in Theorem~\ref{th:expansion}. 
%The submatrices $\outputmat$ returned by  \ourmethod 
%satisfy the error guarantees given in Theorem~\ref{th:expansion}.
All proofs are provided in~\ref{ap:proofs}. 
\fi 
%Sub\-matrices which contain many near-rank-$1$ smaller sub\-matrices are themselves 
\spara{Near-rank-$\mathbf{1}$ submatrices.}
As mentioned in Section~\ref{sec:algo_overview}, $\nrowssubmatrix \times \ncolssubmatrix$ near-rank-$1$ sub\-matrices contain many near-rank-$1$  $2 \times 2$ sub\-matrices. Building on this intuition, \ourmethod starts by locating a $2 \times 2$ sub\-matrix \initialmat with bounded determinant, and hence close to rank $1$. 
%in the initialization phase. 
Then, it computes row-wise and column-wise ratios dividing all rows (columns) by a single anchor row (column) with index sampled from those of \initialmat, 
and finds sub\-matrices with rows (columns) of nearly-constant ratios. 
Nearly-constant ratios correspond to bounded $2 \times 2$ determinants. For instance, if  
\( \left| \frac{\inputmat_{i,j_{1}}}{x^r_{j_1}} - \frac{\inputmat_{i,j_{2}}}{x^r_{j_2}} \right| \leq \tol\), where the left-hand side is a difference of ratios, 
then 
\( 
| \inputmat_{i,j_{1}} x^r_{j_2}  - \inputmat_{i,j_{2}}  x^r_{j_1} | \leq \tol  | x^r_{j_1} | | x^r_{j_2} | \), 
where the left-hand side is a $2 \times 2$ determinant.
%As long as \outputmat extracts a biclique in the last step, 
Bounding the variation of all the ratios within each row and column of a sub\-matrix, and thus the corresponding $2 \times 2$ determinants, \ourmethod yields sub\-matrices composed of $2 \times 2$ near-rank-$1$ sub\-matrices, which, as formalized in Theorem~\ref{th:expansion},  results in approximation guarantees.  









%\cnote[MC]{This lemma is not strictly required}

\iffalse
\cnote[AG]{
The main questions/action points are the ones we discussed on the video call today: \\
1. How good are these bounds? e.g., with $\min\mathbf{D}_{i,j}^2$ in the denominator and 
$\max\mathbf{D}_{i,j}^3$ in the numerator, the errors could very large.\\
2. We need to simplify the presentation of the bounds.\\
Also, \\
3. at the beginning of the section it was mentioned that 
we primarily focus on the bounds on the infinity norm, 
and the bounds on Frobenious and spectral are more loose. 
However, from the theorem below, the opposite seems to be the case.\\
4. As I pointed out to another note, before, what is the strategy and the effect
of choosing the anchor rows and columns? From the theorem it seems that there is some effect.
}
\cnote[MC]{
1. There was a typo in the infinity norm bound, the scale depends is on the anchor row and anchor column. 
I think we do not need to talk about such bounds in general terms but only as a function $\delta$; they simply tell map the choice of $\delta$ to some guarantee. 
2. Agree. 
3. thanks for pointing out, i think that sentence referred to the trivial bounds that always hold for any matrix (infinity norm  gives loose bound on Frob. and Frob. on spectral. 
4. This is also true, we do not discuss this at the moment, but the algorithm could have in principle adapted the value of $\tol$ to the anchor row / column which scales $\tol$ in the error bounds. I would mention this as future work perhaps. 
}
\fi

\begin{theorem}\label{th:expansion}
Let $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ be a near-rank-$1$ sub\-matrix output by \ourmethod with anchor row $\anchorrow$, anchor column $\anchorcolumn$ and input tolerance $\tol$. 
%be any row and any column of $\outputmat$,
%If, as for the matrices \outputmat output by Algorithm~\ref{alg:rankone}, the maximum absolute deviation between two entries in the matrices of ratios obtained by dividing all rows by $\anchorrow$ and all columns by column $\anchorcolumn$  are
%obtained by dividing all rows (columns) by a single row (column) is 
%bounded by $\delta$,
There exists a rank-$1$ approximation $\estimate{\outputmat}$ of \outputmat such that for $\outputerror = \outputmat - \estimate{\outputmat}$ it~holds:
\begin{equation}
\label{eq:initialization_guarantee_infinity}
\infinitynormshort{\outputerror} \leq \min\left\{
\tol \gmax{\anchorrow}, 
\tol \gmax{\anchorcolumn}
\right\},
%\tol  \frac{\max_{i} |{\anchorrow}_i|^3 }{2 \min_{i} {\anchorrow}^2}, 
%\tol  \frac{\max_{j} |{\anchorcolumn}_{j}|^3 }{2 \min_{j} {\anchorcolumn}_{j}^2
%) }
%\min( \frac{\delta}{2 \min_{i} | \anchorrow_i |}  , \frac{\delta}{2 \min_{j} | \anchorcolumn_j |}  ), 
\end{equation}
and 
\begin{equation}\label{eq:expansion_guarantee}
       % \| \initialerror \| \leq \min( \frac{\toleranceinit}{\| \yvec \|} , \frac{\toleranceinit}{\| \xvec \|}) = \toleranceinit \frac{1}{\max(\| \yvec \| \| \xvec \|)}. 
      %\frobeniusnormshort{\outputerror}  \leq \min( \frac{1}{\gamma_{max}^r} \sum_{r=1}^{\nrowssubmatrix}  \tol^2 \omega_r  , \frac{1}{\gamma_{max}^c} \sum_{c=1}^{\ncolssubmatrix}  \tol^2 \omega_c    ), 
      %\frobeniusnormshort{\outputerror}  \leq \min( \sqrt{ \nrowssubmatrix \frac{ \tol^2 \sum_{i < j} |x^r_i|^2 |x^r_j|^2 }{\|\anchorrow\|_2^2} } ,  
      %\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
  \spectralnormshort{\outputerror}  \leq 
\frobeniusnormshort{\outputerror}  \leq \min\left\{ \tol  \sqrt{ (\nrows-1) \gF{\anchorrow} } , 
\tol  \sqrt{ (\ncols-1) \gF{\anchorcolumn} } 
\right\},
%\sqrt{ (\ncolssubmatrix -1) \omega_c} \right\}, 
      %\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
\end{equation}
where 
$\gmax{\xvec} = \frac{\max_{i} |{x}_i|^3 }{2 \min_{i} {x}_i^2}$ and $\gF{\xvec} = \frac{\sum_{i < j} {x_i}^2 {x_j}^2 }{\|\xvec\|_2^2}$.  

%account for the scale of \anchorrow and \anchorcolumn. 
\end{theorem}

\iffalse 
\begin{theorem}[explicit approximation] \label{th:expansion}
Let $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ be a near-rank-$1$ sub\-matrix output by \ourmethod, with anchor row $\anchorrow$, anchor column $\anchorcolumn$ and tolerance $\delta$. 
%be any row and any column of $\outputmat$,
%If, as for the matrices \outputmat output by Algorithm~\ref{alg:rankone}, the maximum absolute deviation between two entries in the matrices of ratios obtained by dividing all rows by $\anchorrow$ and all columns by column $\anchorcolumn$  are
%obtained by dividing all rows (columns) by a single row (column) is 
%bounded by $\delta$,
There exists a rank-$1$ approximation $\estimate{\outputmat} \propto \xvec \yvec^T$ of \outputmat, where either $\xvec$ is a column or $\yvec^T$ a row of \outputmat, such that the matrix $\outputerror = \outputmat - \estimate{\outputmat}$ satisfies: 

\begin{equation}\label{eq:initialization_guarantee_infinity}
\infinitynormshort{\outputerror} \leq \min\{ 
\tol \gmax{\anchorrow}, 
\tol \gmax{\anchorcolumn}
\}
%\tol  \frac{\max_{i} |{\anchorrow}_i|^3 }{2 \min_{i} {\anchorrow}^2}, 
%\tol  \frac{\max_{j} |{\anchorcolumn}_{j}|^3 }{2 \min_{j} {\anchorcolumn}_{j}^2
%) }
%\min( \frac{\delta}{2 \min_{i} | \anchorrow_i |}  , \frac{\delta}{2 \min_{j} | \anchorcolumn_j |}  ), 
\end{equation}
and 
\begin{equation}\label{eq:expansion_guarantee}
       % \| \initialerror \| \leq \min( \frac{\toleranceinit}{\| \yvec \|} , \frac{\toleranceinit}{\| \xvec \|}) = \toleranceinit \frac{1}{\max(\| \yvec \| \| \xvec \|)}. 
      %\frobeniusnormshort{\outputerror}  \leq \min( \frac{1}{\gamma_{max}^r} \sum_{r=1}^{\nrowssubmatrix}  \tol^2 \omega_r  , \frac{1}{\gamma_{max}^c} \sum_{c=1}^{\ncolssubmatrix}  \tol^2 \omega_c    ), 
      %\frobeniusnormshort{\outputerror}  \leq \min( \sqrt{ \nrowssubmatrix \frac{ \tol^2 \sum_{i < j} |x^r_i|^2 |x^r_j|^2 }{\|\anchorrow\|_2^2} } ,  
      %\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
  \spectralnormshort{\outputerror}  \leq 
\frobeniusnormshort{\outputerror}  \leq \min\left\{ \tol  \sqrt{ (\nrows-1) \gF{\anchorrow} } , 
\tol  \sqrt{ (\ncols-1) \gF{\anchorcolumn} } 
\right\} 
%\sqrt{ (\ncolssubmatrix -1) \omega_c} \right\}, 
      %\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
\end{equation}
where 
$\gmax{\xvec} = \frac{\max_{i} |{x}_i|^3 }{2 \min_{i} {x}_i^2}$ and $\gF{\xvec} = \frac{\sum_{i < j} |x_i|^2 |x_j|^2 }{\|\xvec\|_2^2}$.  

%account for the scale of \anchorrow and \anchorcolumn. 
\end{theorem}


\begin{theorem}[Simplified statement]\label{th:expansion}
Let $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ be a near-rank-$1$ sub\-matrix output by \ourmethod, with anchor row $\anchorrow$ and anchor column $\anchorcolumn$.   
%be any row and any column of $\outputmat$,
%If, as for the matrices \outputmat output by Algorithm~\ref{alg:rankone}, the maximum absolute deviation between two entries in the matrices of ratios obtained by dividing all rows by $\anchorrow$ and all columns by column $\anchorcolumn$  are
%obtained by dividing all rows (columns) by a single row (column) is 
%bounded by $\delta$,
Given an error threshold $\errorbound \in \real^{+}$, 
there exist a value of the tolerance parameter $\tol$ 
such that the matrix \outputerror where $\outputmat \in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ is a sub\-matrix output by \ourmethod with anchor row $\anchorrow$ and anchor column $\anchorcolumn$  and $\estimate{\outputmat}$ a rank-$1$ approximation, such that: 
\begin{equation}\label{eq:initialization_guarantee_infinity}
\infinitynormshort{\outputerror} \leq \errorbound
%\tol  \frac{\max_{i} |{\anchorrow}_i|^3 }{2 \min_{i} {\anchorrow}^2}, 
%\tol  \frac{\max_{j} |{\anchorcolumn}_{j}|^3 }{2 \min_{j} {\anchorcolumn}_{j}^2
%) }
%\min( \frac{\delta}{2 \min_{i} | \anchorrow_i |}  , \frac{\delta}{2 \min_{j} | \anchorcolumn_j |}  ), 
\text{ and }
\spectralnormshort{\outputerror}  \leq \frobeniusnormshort{\outputerror} \leq \errorbound 
% \| \initialerror \| \leq \min( \frac{\toleranceinit}{\| \yvec \|} , \frac{\toleranceinit}{\| \xvec \|}) = \toleranceinit \frac{1}{\max(\| \yvec \| \| \xvec \|)}. 
%\frobeniusnormshort{\outputerror}  \leq \min( \frac{1}{\gamma_{max}^r} \sum_{r=1}^{\nrowssubmatrix}  \tol^2 \omega_r  , \frac{1}{\gamma_{max}^c} \sum_{c=1}^{\ncolssubmatrix}  \tol^2 \omega_c    ), 
%\frobeniusnormshort{\outputerror}  \leq \min( \sqrt{ \nrowssubmatrix \frac{ \tol^2 \sum_{i < j} |x^r_i|^2 |x^r_j|^2 }{\|\anchorrow\|_2^2} } ,  
%\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
%\frobeniusnormshort{\outputerror}  \leq \min\left\{ \tol  \sqrt{ (\nrows-1) \gF{\anchorrow} } , 
%\tol  \sqrt{ (\nrowssubmatrix-1) \gF{\anchorrow} } 
%\right\} 
%\sqrt{ (\ncolssubmatrix -1) \omega_c} \right\}, 
  %\sqrt{ \ncolssubmatrix \frac{ \tol^2 \sum_{i < j} |x^c_i|^2 |x^c_j|^2 }{\|\anchorcolumn\|_2^2} } )
\end{equation}
\end{theorem}
\cnote[MC]{If we are not presenting the associated results, it could make to erase the spectral norm completely from the paper... }
\fi 

\iffalse 
Nevertheless, Lemma~\ref{lemma:initialization} only refers to the initialization stage of the methods we introduce. It is important to investigate whether the error guarantees exist also beyond the intialization stage. 
Next, we extend Lemma~\ref{lemma:initialization} to general submatrices, providing an affirmative answer to the following question: does the bound \tol that we consider on the pairwise ratios in the expansion stage lead to a guarantee for the rank-$1$ approximation?  
\fi 


% write result -> proof 
%In the algorithm to recover near-rank-$1$ matrices, we select entries that satisfy a particular condition in terms of the entries of the anchor row and column. 
%However, we have not yet explained how this condition translates into guarantees on the approximation error. In this section, we provide a detailed discussion of these guarantees.

%\spara{Near-rank-$1$ submatrices.}
%We start by discussing guarantees in terms of Frobenius norm for Algorithm~\ref{alg:rankone} in near-rank-$1$ submatrix recovery. 
%We consider both the initialization stage as well as the subsequent expansion stage. 
%considering the initialization stage, 

%In the initialization stage, we identify a $2 \times 2$-submatrix  \initialmat with determinant lower than $\toleranceinit$. 
%In this case, we have the following result. 
%The bound on the Frobenius norm in Theorem~\ref{theorem:expansion} also implies a bound on the spectral norm, since the spectral norm is always lower than or equal to the Frobenius norm~\cite{strang2022introduction}. 
Theorem~\ref{th:expansion} suggests that the low-rank-approximation error incurred 
by the near-rank-$1$ sub\-matrices discovered by \ourmethod 
can be bounded by a function of the input parameter $\tol$ and of the scale of $\anchorrow$ or $\anchorcolumn$. 
Therefore, given the anchor row and column, 
%and the associated row-wise and column-wise ratios, 
one can set the value of \tol to guarantee that the maximum or the total approximation error 
is bounded by a user-specified threshold $\errorbound \in \real^+$, as requested by Problem~\ref{prob:rank-1}. 
However, the approximation-error guarantees given in Theorem~\ref{th:expansion} only hold if \ourmethod extracts a biclique in the last step. Alternative heuristic approaches that do not extract a biclique can be effective in practice, but they are not supported by approximation-error guarantees. 

%However, note that if an heuristic approach is used for approximating maximum-edge bicliques which does not return bicliques, the approximation guarantees may not hold.  
Notably, the approximation-error guarantees are achieved by the interpretable rank-$1$ approximation discussed in Section~\ref{sec:algo_overview}. 
In addition, for the rank-1 \svd approximation $\estimate{\outputmat}$,  
Theorem~\ref{th:expansion_appendix} in~\ref{ap:additional_analysis} bounds the spectral norm of the error \( \outputerror = \outputmat - \estimate{\outputmat} \).



%Theorem~\ref{th:expansion} assumes that the output sub\-matrix corresponds to a bi\-clique. if an heuristic like spectral biclustering is used to approximate 

%If an heuristic approach is used to approximate a maximum-edge bi\-clique, however effective in practice, this is not guaranteed and the theorem may not hold. 




%For the approximation given by the  rank-$1$ \svd, it is particularly interesting to study the spectral norm of the error. 
%Theorem~\ref{th:expansion_appendix} provides an interesting bound on the spectral norm of the matrix $\outputerror = \outputmat - \estimate{\outputmat}$ in case $\estimate{\outputmat}$ is the rank-$1$ \svd. 








\iffalse 
The bounds given in this section may not be the only possible ones. 
In fact, the bound on the Frobenius norm given in Theorem~\ref{th:expansion}, coupled with the notion that the residuals of the orthogonal projection are orthogonal to the projection basis, we can derive a bound on the infinity norm that is a simple function of the bound in Theorem~\ref{th:expansion}. 
Besides, the bound on the infinity norm always implies a bound on the Frobenius norm, namely: 
\(
\frobeniusnormshort{\outputmat} \leq \sqrt{ \nrowssubmatrix \times \ncolssubmatrix \times \frac{\delta}{\min_{i,j} \outputmat_{i,j} }},
\)
and the bound on the Frobenius norm always leads to a bound on the spectral norm~\cite{strang2022introduction}, that is: 
\(
\spectralnormshort{\outputmat} \leq \frobeniusnormshort{\outputmat}. 
\)
%Thus, the algorithm presented in Section~\ref{sec:algo_rank1} provides approximation guarantees for the spectral, Frobenius and infinity norm. 
However, such bounds which are direct consequences of the bound on the infinity norm can be less tight than the refined bounds given in Theorem~\ref{th:expansion} since they are simply derived under the assumption that all entries have value equal to the submatrix maximum. 
\fi 

\iffalse 

\fi 

\spara{Near-rank-$\mathbf{k}$ sub\-matrices.}
The algorithm for the more general task of identifying near-rank-$\generalrank$ sub\-matrices does not admit the same analysis as the algorithm for identifying near-rank-$1$ sub\-matrices.  
However, the algorithm for the rank-$\generalrank$ case, by design, discovers sub\-matrices \outputmat such that
%guarantee a bound on the max norm of 
$\outputerror = \outputmat - \estimate{\outputmat}$ satisfies 
\( \infinitynormshort{\outputerror} \leq \delta \). 
%reflecting our primary objective. 
%In particular, the procedure followed by the algorithm to compute $\ind$ guarantees that 
%\(  \infinitynormshort{\outputerror} \leq \delta \). 
\iffalse 
In particular, the algorithm obtains the matrix $\ind$ 
in such a way that it is guaranteed that there is, for each entry \generalentry such that $\ind_{\generalentry}=1$, a linear combination of $k$ rows and of $k$ columns that reconstruct \generalentry with a maximum deviation of $\delta$. Thus, the algorithm 
guarantees by design that \(  \infinitynormshort{\outputerror} \leq \delta,  \). 
\fi 
As mentioned, the bound on the max norm leads to a straightforward bound on the Frobenius and spectral norms, namely \( \spectralnormshort{\outputerror} \leq \frobeniusnormshort{\outputerror} \leq \tol \sqrt{  (\nrows-\generalrank) (\ncols-\generalrank) }  \), which can also be used to set the value of $\tol$ based on a user-specified error threshold $\errorbound$ on the Frobenius or spectral norm. 

%in case the user specifies an error threshold on the Frobenius or spectral norm. 
%To compute the bound before excracting the output sub\-matrix, one can use 

%and on the spectral norm, i.e., 
%\( 
%\spectralnormshort{\outputerror} \leq \sqrt{  \nrowssubmatrix  %\ncolssubmatrix  \delta^2 }  \). 



\iffalse
\cnote[AG]{
Are we bounding $\|{\outputmat}\|$ or $\|\outputerror\|$?
I am guessing we are bounding $\|\outputerror\|$, 
since $\|{\outputmat}\|$ cannot be bounded (as it is part of the input).
But if we are bounding $\|\outputerror\|$, 
then the bounds stated below (for rank $k$) seem to be better than
the bounds stated in Theorem 1 (for rank 1).
How can this be true?\\
Furthermore, from the discussion it seems that an ``entry-wise'' definition
of the infinity norm is used (see earlier comment).
}
\cnote[MC]{Yes, there is a typo. We are bounding $\outputerror$.
The bounds look cleaner indeed. Simpler algorithm (for the special case) lead to a bit more complex analysis. 
This algorithm (which holds for any rank, also $1$) is a bit less clever, but straightforward analysis. 
I am not sure whether we should compare bounds; they are a function of $\delta$. 
However, the bounds on the Frob / spectral norm are actually trivial in this case, which is not desirable (i.e., only the bound on the infinity norm is good and follows directly from the algorithm, the other bounds are just based on the worst-case where all errors equal the maximum.  We do not want to present them as an important result. 
}
\fi

%Similarly, in view of the relationship between the spectral and Frobenius norm, we have that



%As already mentioned, however, if the infinity norm is bounded, than also the Frobenius norm and spectral norm are bounded. %, although the bounds on the Frobenius and spectral norms are expected to be often loose since they are derived under the assumption that all errors are equal to the maximum error. 

%To conclude this section, we discuss in more detail the guarantees offered by the algorithm we introduce to retrieve near-rank-$\generalrank$ matrices. Infinity-norm guarantees for the submatrices identified by Algorithm~\ref{alg:rankk}, unlike in the case of Algorithm~\ref{alg:rankone}, are a direct consequence of the construction of the matrix $\ind$. 
%For the algorithm introduced to detect near-rank-\generalrank submatrices, 
%the matrix $\ind$ is obtained i
%Clearly, Algorithm~\ref{alg:rankk} can also be used to find near-rank-$1$ submatrices too. % with such guarantees. 
%Given that Algorithm~\ref{alg:rankk}




\subsection{Probabilistic Analysis}
% \cnote[MC]{Not sure what to do with the rest of this section, does not appear as very important and it could go (at least for the most part) to appendix if needed. }
In this section, we discuss simple probabilistic aspects of our method. 

\spara{Probability of discovering a near-rank-$\mathbf{1}$ sub\-matrix.} 
Let \outputmat be a target near-rank-$1$ sub\-matrix of size $| \outputmat |$ within $\inputmat \in \real^{\nrows \times \ncols}$. 
The probability that \ourmethod 
 discovers \outputmat by one sample is 
\(\pfirststar = \frac{\p}{\nrows \ncols}\frac{\p-1}{\nrows \ncols-1}\). 
Hence, the probability of discovering \outputmat in \nrep iterations is \( 1 -  (1 - \pfirststar)^{\nrep} \), and
therefore the number of iterations required to discover $\outputmat$ with probability at least $\alpha_p$ is 
\(\nrep \ge \frac{\ln(1 - \alpha_p)}{\ln(1 - \pfirststar)}.\)
For instance, if \( \pfirststar = 0.1 \) and \( \alpha_p = 0.9 \), we need \(
\nrep > \frac{\ln(1 - 0.9)}{\ln(1 - 0.1)} \approx 22 
\) iterations. 

Basic probability theory implies that, 
in expectation, 
the number of iterations necessary to discover \outputmat is $\frac{1}{\pfirststar}$, 
and we discover it $\pfirststar\nrep$ times in \nrep iterations. 

\spara{Probability of discovering a near-rank-$\mathbf{\generalrank}$ sub\-matrix.} 
The simple probabilistic analysis presented above for near-rank-$1$ sub\-matrices also applies
to near-rank-$\generalrank$ sub\-matrices. 
The only difference is that, in this case, we have 
\(
\pfirststar = \frac{\p}{\nrows \ncols} \frac{\p-1}{\nrows \ncols} \dots  \frac{\p-\generalrank}{\nrows \ncols-\generalrank},  
\)
which can become small as $\generalrank$ grows. Yet, larger values of \generalrank tend to be associated with larger values of  $\p$ and, in practice, we are interested in small values of \generalrank. 

\spara{Probability of occurrence of a $\mathbf{2 \times 2}$ near-rank-$\mathbf{1}$ matrix.} 
%So far we have studied the probability of recovering a near-rank-$1$ matrix from a larger matrix.
%However, we have not discussed the probability of observing a submatrix that is identified as a seed by our method.
We conclude the section by investigating the probability with which 
\ourmethod identifies a seed $2 \times 2$ sub\-matrix with near-zero determinant in random matrices.
% To this aim, 
Let \inputmat be a random matrix with i.i.d. entries distributed according to \distributionz, and let $E(\distributionz) = \mu$ and  
$\var(\distributionz) = \sigma^2$ be the expectation and variance of \distributionz. 
To study the probability of occurrence of $2 \times 2$ sub\-matrices with near-zero determinant, we consider the random variable $\mathcal{W} = x_1 y_2 - x_2 y_1$, where $x_1$, $x_2$, $y_1$ and $y_2$ are the entries of a $2 \times 2$ sub\-matrix.

By independence, 
\(
E(x_1 y_2)    = E(x_1) E(y_2)
\) and 
\(
\var(x_1 y_2) = \var(x_1) \var(y_2) + E(y_2)^2 \var(x_1) + E(x_1)^2 \var(y_2) = \sigma^4 + 2 \mu^2 \sigma^2, 
\)
and similarly for $x_2 y_1$.

Further, since $x_2 y_1$ and $x_2 y_1$ are independent, 
\begin{align*}
E(x_1 y_2 - x_2 y_1) & = E(x_1 y_2) - E(x_2 y_1) = 0 \text{ and} \\ 
\var(x_1 y_2 - x_2 y_1) & = \var(x_1 y_2) + \var(x_2 y_1)=2 \sigma^4 + 4 \mu^2\sigma^2.
\end{align*}
Chebyshev’s inequality~\cite{saw1984chebyshev} then implies that: 
\begin{equation*}
    P(|\mathcal{W}| \geq \toleranceinit) \leq \frac{2 \sigma^4 + 4 \mu^2\sigma^2}{\toleranceinit^2},
\end{equation*}
giving a bound on the probability that a $2\times2$-submatrix deviates significantly from rank $1$. 
The preliminary experiments presented in~\ref{ap:additional_experiments} additionally provide an empirical investigation of this probability.
%However, notice that $\tol$ is close to the expected value of $\epsilon$ and this bound might be loose. 
Assumptions on \distributionz may lead to tighter bounds, a question that we leave open for future work.  


\iffalse 
\spara{Probability of recovering a near-rank-$1$ matrix.}
%amount of entries that belong to a target low-rank submatrix \outputmat. 
To recover near-rank-$1$ sub\-matrices, our method starts by sampling $2$ entries uniformly at random without replacement. If the entries belong to \outputmat, assuming no noise, the algorithm will then expand the $2 \times 2$-matrix to \outputmat. 
The probability of sampling two points belonging to \outputmat is: 
\begin{align*}
\pfirststar = \frac{\p}{\nrows \ncols} \frac{\p-1}{\nrows \ncols-1}. 
\end{align*}
%For simplicity, we let $ = \pfirst$. 
Thus, the probability of sampling two points that do not both belong to \outputmat is $1 - \pfirststar$. 
%Later, we will investigate in more detail the probability \pfirststar of observing near-rank-$1$ matrices in synthetic data. 
As the $2$ entries are independently sampled at every iteration, the probability that we find two entries in $\outputmat$ at least once in $N$ independent iterations %follows a Binomial distribution~\cite{johnson2005univariate} and 
is 
\(
%  \pN = 
1 -  (1 - \pfirststar)^N, 
\)
%\end{align*}
approaching $1$ as $N$ grows, for fixed $\pfirststar$. 
More specifically, simple algebra shows that the number of samples required to discover $\outputmat$ with probability at least $\alpha_p$ is: 
\[
N > \frac{\ln(1 - \alpha_p)}{\ln(1 - \pfirststar)}. 
\]
For instance, if \( \pfirststar = 0.1 \) and \( \alpha_p = 0.9 \), we get \(
N > \frac{\ln(1 - 0.9)}{\ln(1 - 0.1)} \approx 22. 
\)


In expectation, we recover the target \outputmat $N \pfirststar$ times in $N$ iterations, with a variance of $N \pfirststar (1 - \pfirststar)$. 
Further, as the number of initializations required to retrieve \outputmat is described by the geometric distribution~\cite{johnson2005univariate}, the expected number of iterations necessary to recover \outputmat is $\frac{1}{\pfirststar}$, with variance $\frac{1-\pfirststar}{\pfirststar}$.



\iffalse 
In practice, \ourmethod does not expand all $2 \times 2$ sub\-matrices, but only those that, as indicated by the determinant, are nearly rank-deficient, and thus the algorithm in practice requires significantly less iterations that those indicated by the previous inequality. 
\fi 
\iffalse
However, it is perhaps more interesting to consider the probability distribution of the number of initializations required to retrieve \outputmat, which .
In particular,  the probability of recovering the ground truth after $N$ iterations is given by: 
\[
  \pN = (1 - \pfirststar)^{N-1} \pfirststar. 
\]
%\end{align*}
The expected number of iterations necessary to recover \outputmat is $\frac{1}{\pfirststar}$ with variance $\frac{1-\pfirststar}{\pfirststar}$.
\fi 

\iffalse 
Another straightforward observation is that,  
if in a matrix there are multiple target low-rank submatrices, the probability that, given that we have hit a target, we have hit the largest one is \( 
\frac{1}{p_{tot}} \frac{1}{p_{tot}-1}  \frac{p_{max}}{p_{tot}} \frac{p_{max} - 1}{p_{tot}-1}  
\), 
where $p_{tot}$ and $p_{max}$ denote the total size of all target submatrices and of the largest one, respectively. 
Without going into specifics, note that if there is a large target low-rank submatrix in the data, instead of randomly sampling entries, it would be beneficial to introduce sampling weights e.g. based on statistical leverage. 
\fi 

\spara{Probability of recovering a near-rank-$\generalrank$ matrix.}
The simple probabilistic analysis presented above for the case of near-rank-$1$ matrices also applies to the discovery of near-rank-$\generalrank$ submatrices. 
The only difference is that in this case, we need to sample $\generalrank+1$ row and column indices, and thus: 
\[
\pfirststar = \frac{\p}{\nrows \ncols} \frac{\p-1}{\nrows \ncols} \dots  \frac{\p-\generalrank}{\nrows \ncols-\generalrank}, 
\] 
which can become very small as $\generalrank$ grows. However, for larger values of \generalrank, larger values of $p$ are expected and, in practice, we are interested in small values of \generalrank for which Algorithm~\ref{alg:rankk} quickly samples  $\generalrank+1 \times \generalrank+1$ rank-deficient sub\-matrices. 




%Another important questions concerns the probability of occurrence of $2 \times 2$ matrices that are close to rank-$1$, which is identified as a seed by Algorithm~\ref{alg:rankone} in the initialization stage. 


%Let us consider an arbitrary $2\times2$-submatrix in \inputmat: 
We consider an arbitrary $2\times2$-submatrix 
\[
\initialmat = 
\begin{bmatrix}
x_1 & x_2 \\
y_1 & y_2
\end{bmatrix}.
\]
If 
%such a matrix is close to rank-$1$ if 
\(
    | x_1 y_2 - x_2 y_1 | \leq \toleranceinit
\), then \initialmat is close to rank $1$. 
Thus, to study the probability of occurrence of a $2\times2$ near-rank-$1$ matrix, we need to study the probability of the random variable $\mathcal{W} = x_1 y_2 - x_2 y_1$.
First, let us consider the two products. 
%As concerns the distribution of $ad$, we know that, 
By independence, $E(x_1 y_2) = E(x_1) E(y_2)$ and similarly $\var(x_1 y_2) = \var(x_1) \var(y_2) + E(y_2)^2 \var(x_1) + E(x_1)^2 \var(y_2) = \sigma^4 + 2 \mu^2 \sigma^2$.
By symmetry, we also have: 
$E(x_2 y_1) = E(x_2)E( y_1)$ and $\var(x_2 y_1) =\sigma^4 + 2 \mu^2 \sigma^2$. 



%So far in this section, we have characterized the probability with which our method samples particular near-low-rank submatrices in the initialization stage. 

\fi 

%of hitting the largest one is given by $\frac{p*_{max}}{p*_{tot}}$ where $p*_{max}$ is the probability of sampling two points belonging to the largest target low-rank submatrix and 


%covering in total a proportion $p_{tot}$ of the total amount of entries, the probability of hitting 

\subsection{Computational Complexity}
Finally, we discuss the computational complexity of \ourmethod. 

Consider a single iteration of the method.
The runtime bottleneck is due to finding a maximum-edge bi\-clique, which, in the worst case can take exponential time. However, the algorithm introduced by Lyu et al.~\cite{lyu2020maximum} prunes large portions of the search space and can be very efficient in practice. 
% Moreover, its complexity is polynomial in the number of maximal bicliques. 
As discussed in Section~\ref{sec:scalability}, to improve scalability, we can use a more scalable heuristic for finding an approximate maximum-edge biclique.
The spectral bi\-clustering algorithm, which is the heuristic we rely on by default, has computational complexity determined by the computation of the (truncated) \svd, 
which is $\bigO \left( \min(\nrows^2 \ncols, \ncols^2 \nrows) \right)$. 
If an even more scalable heuristic is leveraged, 
such as a basic linear-time algorithm removing rows and columns of \ind with less than a given proportion of ones, 
%{\color{red}%(say explicitly which is this more scalable heuristic)} 
%this step is no longer the bottleneck, 
\ourmethod for the rank-$1$ case and for the general rank-\generalrank case incurs computational complexity $\bigO( \nrows +  \ncols)$ and $\bigO( \nrows \generalrank \ncols)$, respectively. 

As \ourmethod generally explores different initializations, if $\tau$ is the complexity of a single iteration, then $\bigO(\nrep \tau)$ is the overall complexity. 


==> arXiv-2506.06456v1/conclusions_arxiv.tex <==
\section{Conclusion}\label{sec:conclusion}
Low-rank approximation finds applications in many data-analysis tasks. 
%including data compression, noise reduction, fast computations in machine learning, image processing and large-scale data analysis.  
Typically, methods assume that the entire matrix exhibits low-rank structure, 
while in real-world data this is often true only for certain sub\-matrices.
%There can be submatrices that are accurately described by a single row and column. 
In this work, we study the problem of finding sub\-matrices 
that are provably close to a 
% (possibly interpretable) 
% rank-$1$ approximation, or more generally to a 
rank-$\generalrank$ approximation. 
%
%sub\-matrix of small rank. 
%provably close to a small rank. 
We introduce a novel method that finds such sub\-matrices, study the properties of the method, 
and, with a thorough experimental evaluation, we show
that our method outperforms strong~baselines.
%In particular, the sub\-matrices retrieved by %<our method have bounded deviation from an% intepretable low-rank approximation. %  along with interpretable low-rank approximations thereof. % such that each submatrix entry is provably close to its approximation.
%The strong guarantees our methods are endowed with means that they are also suitable for applications where trustworthiness is an important requirement. 
%A thorough experimental evaluation demonstrates that our method offers high efficiency and is effective in recovering near-low-rank sub\-matrices, 
% A thorough experimental evaluation demonstrates that our method 
% typically outperforms existing alternative approaches, while also offering error guarantee. % and more trustworthiness. 
%

There are several directions for future work. 
For instance, future work could study a more robust initialization strategy, 
develop more efficient and scalable alternative algorithms, and optimize the selection of the anchor rows and columns.
%It would also be interesting to study more in depth probabilistic aspects of our method.
It would also be valuable to investigate more the probabilistic aspects of our method.
From a practical perspective, it would be interesting to explore further the benefits 
of our approach in different applications. 

%With respect to the analysis, it would be valuable to obtain tighter guarantees on the approximation error or to investigate more in depth the occurrence of near-low-rank sub\-matrices in different types of random matrices. 

\clearpage

\iffalse 
Local low-rank approximation represents an highly challenging task. 
In this work, we have introduced a novel perspective on local low-rank approximation of a matrix that is simple and based on geometrical intuition. 
We have introduced and analysed methods to efficiently retrieve submatrices where each entry is provably close to a low-rank approximation. As a byproduct, our methods also compute approximations that are interpretable.

We have focused particularly on the import case of near-rank-$1$ matrices. This case corresponds to the search of data points distributed along a line in a vector space. 
We have demonstrated that our methods outperform existing methods in the task of identifying near-rank-$1$ submatrices from larger matrices. 
\fi 


==> arXiv-2506.06456v1/defines.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quThe \svd decomposes a matrix into ality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
% \usepackage{natbib}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{float}
%\usepackage{tikz}
\usepackage{varwidth}
\usepackage{caption}
\usepackage{enumitem}
% space set according to
% http://ftp.acc.umu.se/mirror/CTAN/macros/latex/contrib/enumitem/enumitem.pdf
% \setlist[itemize]{nosep, leftmargin=16pt}
% \setlist[enumerate]{nosep, leftmargin=16pt}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{dateplot}

% paragraph top margin
\setlength{\parskip}{0pt}

% for footnote cross-referencing
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

% \usepackage{amsthm}
%\usepackage[ruled, vlined, nofillcomment, linesnumbered]{algorithm2e}

\usepackage[show]{chato-notes}
% \usepackage[hide]{chato-notes}

\DeclareMathOperator*{\argmin}{\arg\min}
\DeclareMathOperator*{\argmax}{\arg\max}

% algorithm


%\newtheorem{lemma}{Lemma}
%\newtheorem{problem}{Problem}
%\newtheorem{observation}{Observation}

%¤\newtheorem{theorem}{Theorem}
% \newtheorem*{definition*}{Definition}

\newcommand{\journal}[1]{\textcolor{red}{#1}}

%\newcommand{\journal}[1]{} 



\newcommand{\aris}[1]{\smallskip\noindent{\color{cyan}$\Rightarrow$~Aris:~~{#1}}\xspace}

\newcommand{\para}[1]{\noindent{\bf{#1}}}
\newcommand{\spara}[1]{\smallskip\noindent{\bf{#1}}}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\abs}[1]{{\left|#1\right|}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\real}{\ensuremath{\mathbb{R}}\xspace}

\newcommand{\hamming}{\ensuremath{\mathbb{H}}\xspace}
\newcommand{\realnn}{\ensuremath{\real_{\ge 0}}\xspace}
\newcommand{\pr}[1]{\ensuremath{\left(#1\right)}\xspace}
\newcommand{\spr}[1]{\left[#1\right]}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\np}{\ensuremath{\mathbf{NP}}\xspace}
\newcommand{\bigO}{\ensuremath{\mathcal{O}}\xspace}

\newcommand{\define}{\leftarrow}
\newcommand{\integer}{\ensuremath{\mathbb{Z}_{+}}\xspace}

\newcommand{\featspace}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\numfeat}{\ensuremath{d}\xspace}
\newcommand{\labelspace}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\numlabel}{\ensuremath{k}\xspace}
\newcommand{\dataset}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\ds}{\dataset}
\newcommand{\dsdef}{\ensuremath{\dataset=\set{\dr_i}_{i=1}^{\numpts}}\xspace}

\newcommand{\inputmat}{\ensuremath{\mathbf{D}}\xspace}
\newcommand{\outputmat}{\ensuremath{\mathbf{X}}\xspace}

\newcommand{\outputmatestimate}{\ensuremath{\hat{\mathbf{X}}\xspace}}

\newcommand{\distributionz}{\ensuremath{\mathcal{Z}}\xspace}

\newcommand{\bfA}{\ensuremath{\mathbf{A}}\xspace}
\newcommand{\bfB}{\ensuremath{\mathbf{B}}\xspace}
\newcommand{\bfX}{\ensuremath{\mathbf{X}}\xspace}
\newcommand{\bfY}{\ensuremath{\mathbf{Y}}\xspace}
\newcommand{\bfU}{\mathbf{U}\xspace}
\newcommand{\bfSigma}{\mathbf{\Sigma}\xspace}
\newcommand{\bfV}{\mathbf{V}\xspace}

\newcommand{\estimate}[1]{\hat{#1}}
\newcommand{\error}[2]{\left\| {#1} - {#2} \right\|_F^2}


% Frobenius norm command
\newcommand{\frobeniusnorm}[1]{\left\| {#1} \right\|_F}
\newcommand{\frobeniusnormshort}[1]{\| {#1} \|_F}

% Spectral norm command
\newcommand{\spectralnorm}[1]{\left\| {#1} \right\|_2}
\newcommand{\spectralnormshort}[1]{\| {#1} \|_2}

% Infinity norm command
\newcommand{\infinitynorm}[1]{\left\| {#1} \right\|_{\max}}
\newcommand{\infinitynormshort}[1]{\| {#1} \|_{\max}}

\newcommand{\infinitynormold}[1]{\left\| {#1} \right\|_{\infty}}

% General norm command
\newcommand{\generalnorm}[1]{\left\| {#1} \right\|_{*}}
\newcommand{\generalnormshort}[1]{\| {#1} \|_{*}}

% low-rankness score
\newcommand{\lowrankness}[1]{\ensuremath{\mathit{{\ell}{r}}({#1})}\xspace}



\newcommand{\nphard}{\ensuremath{\mathbf{NP}}-hard\xspace}

\newcommand{\noisescale}{\ensuremath{\epsilon_{\text{noise}}}\xspace}

\newcommand{\initialmat}{\ensuremath{\mathbf{P}}\xspace}
\newcommand{\ind}{\ensuremath{\mathbf{I}}\xspace}
\newcommand{\indrows}{\ensuremath{\mathbf{I}^r}\xspace}
\newcommand{\indcols}{\ensuremath{\mathbf{I}^c}\xspace}
\newcommand{\generalrank}{\ensuremath{k}\xspace}
\newcommand{\generalrow}{\ensuremath{i}\xspace}
\newcommand{\generalcol}{\ensuremath{j}\xspace}
\newcommand{\truerank}{\ensuremath{r}\xspace}
\newcommand{\generalranknospace}{\ensuremath{k}}
\newcommand{\initialmatnospace}{\ensuremath{\mathbf{P}}}
\newcommand{\initialmatsnospace}{\ensuremath{\initialmatnospace}_k}
\newcommand{\initialmats}{\ensuremath{\initialmatnospace_{k}}\xspace}
\newcommand{\initialerror}{\ensuremath{\mathbf{E}_{\initialmatnospace}}\xspace}
%\newcommand{\outputerror}{\ensuremath{\mathbf{E}_{\outputmat}}\xspace}
\newcommand{\identitymat}{\ensuremath{\mathbf{I}}\xspace}

%
\newcommand{\outputerror}{\ensuremath{\mathbf{E}_{\outputmat, \estimate{\outputmat}}}\xspace}
\newcommand{\rank}{\ensuremath{\mathrm{rank}}\xspace}
\newcommand{\truncSigma}{\mathbf{\Sigma}_k}
\newcommand{\truncU}{\mathbf{U}_k}
\newcommand{\truncV}{\mathbf{V}_k}
\newcommand{\frobnorm}[1]{\left\| #1 \right\|_F}
\newcommand{\indicatorfun}[1]{\mathbf{1}\{#1\}}
\newcommand{\pseudoinverseinitialmat}
{\ensuremath{\initialmatsnospace^{\dagger}}\xspace}
\newcommand{\initialmatcols}{\ensuremath{\mathcal{C}_{\initialmatnospace}}\xspace}

\newcommand{\initialmatrows}{\ensuremath{\mathcal{R}_{\initialmatnospace}}\xspace}

\newcommand{\gmax}[1]{g_{\max}(#1)}
\newcommand{\gF}[1]{g_{F}(#1)}

\newcommand{\rowset}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\colset}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\sinematrix}{\ensuremath{\mathbf{S}_{\mathcal{C}}}\xspace}

\newcommand{\nearrankone}{{LNROS}\xspace}
\newcommand{\nearrankk}{{LNR\ensuremath{k}S}\xspace}

%\theoremstyle{thmstyleone}%
%\newtheorem{theorem}{Theorem}%  meant for continuous numbers
%%\newtheorem{theorem}{Theorem}[section]% meant for sectionwise numbers
%% optional argument [theorem] produces theorem numbering sequence instead of independent numbers for Proposition
%\newtheorem{proposition}[theorem]{Proposition}
\newcommand{\orthogonalprojection}{\ensuremath{$\hat{\inputmat}$}\xspace}
\newcommand{\nrows}{\ensuremath{n}\xspace}
\newcommand{\ncols}{\ensuremath{m}\xspace}
\newcommand{\nrowssubmatrix}{\ensuremath{n'}\xspace}
\newcommand{\ncolssubmatrix}{\ensuremath{m'}\xspace}

%\newcommand{\tolerance}{\ensuremath{\delta}\xspace}
\newcommand{\toleranceinit}{\ensuremath{\delta_{\mathit{init}}}\xspace}
\newcommand{\tol}{\ensuremath{\delta}\xspace}

\newcommand{\errorbound}{\ensuremath{\epsilon}\xspace}

\newcommand{\simplifiedproblem}{LNROSR\xspace}

\newcommand{\affineproblem}{LNRkAS\xspace}


\newcommand{\f}[1]{f(#1)}




\newcommand{\errors}
{\ensuremath{\mathbf{E}^{abs}}\xspace}
\newcommand{\svd}{{SVD}\xspace}
\newcommand{\svp}{\textsc{SVP}\xspace}
\newcommand{\pca}{{PCA}\xspace}
\newcommand{\sparsePCA}{\textsc{Sparse\-PCA}\xspace}
\newcommand{\cvx}{\textsc{CVX}\xspace}
\newcommand{\rpsp}{\textsc{RPSP}\xspace}
\newcommand{\ourmethod}{\textsc{Sample\-And\-Expand}\xspace}

\newcommand{\gram}
{\ensuremath{\mathbf{G}}\xspace}
\newcommand{\anchorrow}
{\ensuremath{\mathbf{x}^r}\xspace}
\newcommand{\anchorrowentryi}
{\ensuremath{x^r_i}\xspace}
\newcommand{\anchorrowentryis}
{\ensuremath{{x^r_i}}\xspace}
\newcommand{\anchorrowentryj}
{\ensuremath{x^r_j}\xspace}
\newcommand{\anchorrowentryjs}
{\ensuremath{{x^r_j}}\xspace}

\newcommand{\anchorindexrow}
{\ensuremath{i_a}\xspace}
\newcommand{\anchorindexcol}
{\ensuremath{j_a}\xspace}

\newcommand{\anchorcolumn}
{\ensuremath{\mathbf{x}^c}\xspace}
\newcommand{\anchorcolumnentryj}
{\ensuremath{x^c_j}\xspace}
\newcommand{\anchorcolumnentryjs}
{\ensuremath{{x^c_j}}\xspace}

\newcommand{\nrep}{\ensuremath{N_{\mathit{init}}}\xspace}
\newcommand{\p}{\ensuremath{|\outputmat|}\xspace}
\newcommand{\pfirst}{\ensuremath{\mathit{Pr}(\mathit{itr}=1)}\xspace}
\newcommand{\pfirststar}{\ensuremath{p}\xspace}
\newcommand{\pN}{\ensuremath{\mathit{Pr}(\mathit{itr}=N)}\xspace}
\newcommand{\generalentry}{\ensuremath{(i,j)}\xspace}
\newcommand{\offset}{\vecv}


\newcommand{\xbf}{\ensuremath{\mathbf{x}}}
\newcommand{\xonebf}{\ensuremath{\mathbf{x}_1}\xspace}
\newcommand{\xtwobf}{\ensuremath{\mathbf{x}_2}\xspace}
\newcommand{\rowratios}{\ensuremath{\mathbf{R}^r}\xspace}
\newcommand{\columnratios}{\ensuremath{\mathbf{R}^c}\xspace}

\newcommand{\rowratiosij}{\ensuremath{\mathbf{R}^r_{i,j}}\xspace}
\newcommand{\columnratiosij}{\ensuremath{\mathbf{R}^c_{i,j}}\xspace}


% datasets 
\newcommand{\Hyperspectral}{\textsc{Hyperspectral}\xspace}
\newcommand{\Isolet}{\textsc{Isolet}\xspace}
\newcommand{\Olivetti}{\textsc{Olivetti}\xspace}
\newcommand{\MoiveLens}{\textsc{MovieLens}\xspace}
\newcommand{\MovieLens}{\textsc{MovieLens}\xspace}
\newcommand{\OrlRnSp}{\textsc{ORL}\xspace}
\newcommand{\Jester}{\textsc{Jester}\xspace}
\newcommand{\Golub}{\textsc{AL-Genes}\xspace}
\newcommand{\Mandrill}{\textsc{Mandrill}\xspace}
\newcommand{\Ozone}{\textsc{Ozone}\xspace}
\newcommand{\SKCM}{\textsc{SKCM1}\xspace}
\newcommand{\BRCA}{\textsc{BRCA-Genes}\xspace}
\newcommand{\PRAD}{\textsc{PRAD1}\xspace}
\newcommand{\Google}{\textsc{Google}\xspace}
\newcommand{\NPAS}{\textsc{NPAS}\xspace}
\newcommand{\Cameraman}{\textsc{Cameraman}\xspace}
\newcommand{\MovieTrust}{\textsc{MovieTrust}\xspace}
\newcommand{\Hearth}{\textsc{Hearth}\xspace}
\newcommand{\Imagenet}{\textsc{Imagenet}\xspace}

\newcommand{\maxnorm}{\ensuremath{\gamma_{max}}\xspace}

\newcommand{\indicator}{\ensuremath{\mathbf{I}}\xspace}

%\newcommand{\tol}{\ensuremath{\delta}\xspace}
\newcommand{\basisvec}{\ensuremath{x}\xspace}

\newcommand{\errorvec}{\ensuremath{\boldsymbol{\epsilon}}\xspace}

%\newcommand{\xvec}{\ensuremath{\mathbf{x}}\xspace}

%\newcommand{\yvec}{\ensuremath{\mathbf{y}}\xspace}


%
\newcommand{\vecu}{\ensuremath{\mathbf{u}}\xspace}
%
\newcommand{\vecv}{\ensuremath{\mathbf{v}}\xspace}
%
\newcommand{\vecw}{\ensuremath{\mathbf{v}}\xspace}
%
\newcommand{\budget}{\ensuremath{\mathcal{B}}\xspace}
%
%
%
\newcommand{\zvec}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\vvec}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\yvec}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\xvec}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\proj}[2]{\operatorname{Proj}_{{#1}} #2}

\newcommand{\var}{\ensuremath{\mathit{Var}}\xspace}


\newcommand{\ie}{i.e.,}
\newcommand{\eg}{e.g.,}

\newcommand{\halfKron}{\mathbin{\tikz[baseline=-0.4ex] \draw[thick] (-0.,0) arc (180:360:0.18em) (0,0.1) arc (180:0:0.18em)  (0.06,0.05) node {\small $\times$};}}

\newcommand{\halfKronCol}{\mathbin{\tikz[baseline=-0.4ex] \draw[thick] (0,0.1) arc (90:270:0.2em) (0.1,0.1) arc (90:-90:0.2em)  (0.05,0.05) node {\small $\times$};}}





==> arXiv-2506.06456v1/diagrams/firstfigure.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{c c !{\vrule width 2pt} c c}  % 2pt thick vertical black line
        % First image
        \adjustbox{valign=m}{\includegraphics[width=0.24\textwidth]{images/D_sub_lines.pdf}} &
        % Second image
        \adjustbox{valign=m}{\includegraphics[width=0.24\textwidth]{images/D_sub_lr_lines_with_firebrick_line.pdf}} &
        % Third image (source of the arrow)
        \adjustbox{valign=m}{\includegraphics[width=0.18\textwidth]{images/D_sub.pdf} 
            \begin{tikzpicture}[overlay, remember picture]
                \draw[thick, ->, black] (-1.5,1.75) to[out=30, in=150] (0.5,1.75);
            \end{tikzpicture}
        } &
        % Fourth image (destination of the arrow)
        \adjustbox{valign=m}{\includegraphics[width=0.25\textwidth]{images/D_sub_lr2.pdf}} 
    \end{tabular}
    \caption{\label{fig:first_figure} \Hyperspectral dataset. On the left, we show the values of the rows in a $50 \times 50$ matrix and the nearly-proportional values of the rows in a near-rank-$1$ $11 \times 44$ sub\-matrix discovered by our method. On the right we show the matrix and, next to it, the discovered sub\-matrix (top) and its accurate approximation expressing each row as collinear with the row highlighted in red (bottom). 
    %to have the discovered sub\-matrix on the top left corner and its accurate approximation obtained by expressing each row as a linear combination of the row highlighted in red.
    }
\end{figure}



==> arXiv-2506.06456v1/experiments_arxiv.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we evaluate the performance of \ourmethod against existing approaches.  %, hereinafter also referred to as \ourmethod 
%(\underline{s}ample and \underline{e}xpand) for brevity, in extensive experiments. 
%(\underline{p}rovably -\underline{a}ccurate \underline{l}ocal \underline{l}ow-rank \underline{a}pproximation) for brevity, in extensive experiments. 
We consider both synthetic data and real-world data. %, where a notion of \emph{ground truth} is available. % and real-world data. 
%We compare our methods primarily against the \rpsp method, introduced in Section~\ref{sec:related}, which represents the state-of-the-art as well against other existing approaches. 
% First, we briefly summarize the experimental setup in Section~\ref{sec:exp_setup}, 
% and then in Section~\ref{sec:exp_results} we present results. 
More details on the experimental setup are provided in~\ref{ap:additional_experimental_setup}, and
additional experimental results are presented in~\ref{ap:additional_experiments}. 

%, e.g., investigating the impact of noise or of the parameter $\tol$ that controls the approximation quality in our methods. 

\subsection{Experimental Setup}\label{sec:exp_setup}
%We start with preliminary experiments that aims at provide valuable insight into the problems studied in this work as well as the given methods.
% In this section, we present the datasets used in our experiments, the evaluation metrics, the baseline methods for comparison, and the parameter settings of the algorithms under comparison.

\iffalse 
We evaluate our method, hereinafter also referred to as \ourmethod (\underline{s}ample and \underline{e}xpand)
%(\underline{p}rovably -\underline{a}ccurate \underline{l}ocal \underline{l}ow-rank \underline{a}pproximation)
for brevity, against the baselines in synthetic data. We consider both a simple scenario where a single near-rank-$1$ matrix is planted in a larger matrix, and a more challenging scenario where the data are generated with a sum of near-rank-$1$ submatrices. 
%recovery where a synthetic near-rank-$1$ matrix is planted in the data. 
%Finally, we assess the performance of our methods in general local low-rank approximation in both synthetic and real-world data.  
\fi 

\para{Datasets.}
We conduct experiments on both synthetic and real-world datasets.

The synthetic data are generated by planting near-rank-$1$ sub\-matrices into larger matrices. 
To make the % near-rank-$1$ sub\-matrix recovery 
discovery task as challenging as possible, the entries of the planted sub\-matrices and of the background 
are generated % i.i.d. 
from the same distributions. 
We consider six different distributions. 
The details of the data-generating mechanisms are given in~\ref{ap:additional_experimental_setup}. 
% and we consider both the setting where there is a single planted sub\-matrix as well as the setting where there are multiple, possibly overlapping, planted sub\-matrices. 
%Our results on synthetic data are presented in the next section, 
%and additional results in~\ref{ap:additional_experiments}. 
% In~\ref{ap:additional_experiments}, we present preliminary experiments results on synthetic data, capturing salient characteristics of the data and of the behavior of our method in such data. 
%In particular, such experiments shed light on the probability of observing near-rank-$1$ $2 \times 2$ sub\-matrices in the initialization as well as on the expansion stage both in matrices with planted near-rank-$1$ sub\-matrices and without. 

Additionally, we consider $15$ real-world datasets from different applications, 
%  from various domains that are relevant for low-rank approximation, 
including user ratings, images, and gene-expression data. 
% While not strictly necessary, for convenience, real-world data matrices are preprocessed by normalizing the value to range between $0$ and $1$. 
We report summary characteristics for the real-world datasets in Table~\ref{tab:real_world_datasets}, 
%while the same information for the other datasets is provided in~\ref{ap:additional_experimental_setup}. 
%along with the results 

\begin{table}[t]
\centering
\caption{\label{tab:real_world_datasets} Summary characteristics for real-world datasets. We report the number of rows, columns,  the low-rankness score, the entry-wise maximum squared deviation from the rank-1 \svd (Max rank-$1$ deviation) and a reference.}
    \label{tab:datasets}
\begin{tabular}{lrrrrr}  % l = left-aligned, r = right-aligned
    \toprule
    {{{Dataset}}} & 
    {{~\# Rows}} & 
    {{~\# Columns}} & 
    {{~Low-rankness}} & 
    {{~Max rank-${1}$}} & 
    {{~Reference}} \\
    & & & {{score}} & {{deviation}} & \\
    \midrule
    \Hyperspectral & 5\,554 & 2\,151 & 0.89 & 0.23 & \cite{leone2022hyperspectral} \\
    \Isolet & 7797 & 617 & 0.88  & 0.98  & \cite{asuncion2007uci} \\
    \Olivetti & 400  & 4096 & 0.95  & 0.53  & \cite{asuncion2007uci} \\
    \MoiveLens & 943 & 1682 & 0.30  & 1.00 & \cite{harper2015movielens} \\ 
    \OrlRnSp & 400 & 1024 & 0.95  & 0.55  & \cite{orl_faces} \\
     \Golub & 7129 & 38 & 1.00  & 0.28  & \cite{esposito2021review} \\
    \Mandrill & 512 & 512 & 0.92  & 0.36  & \cite{usc-sipi} \\
    \Ozone & 2536 & 72 & 1.00  & 0.08  & \cite{asuncion2007uci} \\
    \BRCA & 317 & 496 & 0.72  & 0.89  & \cite{tomczak2015review} \\
    \Google & 5456 & 24 & 0.76  & 0.77  & \cite{asuncion2007uci} \\
    \NPAS & 1418 & 78 & 0.85  & 0.15  & \cite{kaggle} \\
    \Cameraman & 256 & 256 & 0.86  & 0.56  & \cite{usc-sipi} \\
    \MovieTrust & 200 & 200 & 0.77  & 1  & \cite{kaggle} \\
    \Hearth & 920 & 15 & 0.94  & 0.08  & \cite{asuncion2007uci} \\
    \Imagenet & 64 & 27 & 0.92  & 0.22  & \cite{deng2009imagenet} \\
    \bottomrule
\end{tabular}
\end{table}


\spara{Baselines.}
We compare \ourmethod against baselines discussed in Section~\ref{sec:related}. 
Specifically, we consider 
a method (\cvx) based on convex optimization~\cite{doan2013finding}, 
PCA with sparsity constraints (\sparsePCA)~\cite{mairal2009online}, 
\svp~\cite{ruchansky2017targeted}, and \rpsp~\cite{dang2023generalized}.
In the experiments with real data, we restrict the comparison to  the most recently introduced methods, \svp and \rpsp, which  specifically aim at discovering (possibly multiple) near-low-rank sub\-matrices.  
%Sparse PCA and \cvx instead are not inteded to discover 


\iffalse 
\begin{itemize}
    \item \rpsp
    \item Sparse PCA~\cite{mairal2009online}. 
    \item Convex optimization~\cite{doan2013finding}. 
\end{itemize}
\fi 

\iffalse 
Among such methods, only \rpsp is designed specifically for the general problem of local low-rank approximation. 
Thus, in the experiments with real-world data, we restrict the comparison to \rpsp, which has also been shown to achieve unprecedented performance in recovering low-rank submatrices. 
\fi 

%More details on both the synthetic and real-world data matrices are provided in Appendix~\ref{ap:additional_experimental_setup}.  

%The details of the data-generating mechanism are given
%Table~\ref{tab:real_world_datasets} in Appendix~\ref{ap:additional_experimental_setup} provides summary characteristics.  

\spara{Metrics.}
%In the experiments with synthetic data, we measure the ability of a method in recovering the ground truth using the $F_1$ score. 
In experiments with synthetic data, 
% we assess the ability of a method to recover the ground truth by measuring its $F_1$ score. 
all methods output matrices $\estimate{\inputmat}$ that contain low-rank approximations of the identified sub\-matrices and zero entries for all indices that are not part of such sub\-matrices.
%have zero entries for all the indices the indices that are not part of the discovered sub\-matrices.   
%composed of all zeros except in the indices of the identified low-rank sub\-matrices.
To measure the ability of a method in recovering the indices of the planted ground-truth sub\-matrices,
we report the $F_1$ score.
Based on the same output,  we also report the error (squared Frobenius norm averaged over the entries) incurred in approximating the ground-truth sub\-matrices. 
\ourmethod approximates sub\-matrices through the interpretable approach discussed in Section~\ref{sec:algo_overview} for $\generalrank=1$ and via \svd for $\generalrank>1$. All baselines approximate sub\-matrices via \svd.   

% Further, we monitor the error (in terms of squared Frobenius norm) incurred in approximating the ground truth sub\-matrices. 
%any of the algorithms under comparison in recovering the 
%For synthetic data, we measure the error incurred in approximating the planted submatrices \outputmat by the squared Frobenius norm 
%\(
%\frobeniusnorm{ \estimate{\outputmat} - \outputmat}^2, 
%\)
%where $\estimate{\outputmat}$ denotes the estimate of %\outputmat given by any of the methods being compared. 

%\cnote[AG]{Is the reported error wrt ground-truth submatrices or wrt discovered submatrices?}
%\cnote[MC]{Ground truth in synthetic data - clarified }

In real-world datasets, where no ground truth is available, 
we report the size and low-rankness score (introduced in Section~\ref{sec:preliminaries})
%~\cite{dang2023generalized} 
of the returned sub\-matrices.  
%The low-rankness score is given by the ratio of the first singular value squared to the sum of the squared singular values. 

In all cases, we measure run\-times in seconds.




\spara{Parameters.} % appendix bound 
%In the experiments with synthetic data, we always consider matrices of dimensions $250 \times 250$. 
%The noise multiplier $\epsilon_{noise}$ is set to $10^{-5}$. 
The important parameter to set for our method 
% The crucial parameter that affects the results given by our method 
is the tolerance $\tol$ controlling the trade-off between low-rankness and size. 
As explained in Section~\ref{sec:analysis}, 
% in real-world applications, 
one can set $\tol$ to match an input bound \errorbound on the allowed low-rank-approximation error. 
In our experiments, however, we explore few fixed values of $\tol$. 
Specifically, for experiments with synthetic data, we set $\tol$ to $0.05$ 
and the number of initializations $\nrep$ to $25$. 
For experiments with real-world data, we let $\tol$ vary in $\{ 10^{-1}, 10^{-2}, 10^{-3}, 10^{-4} \}$, 
and we consider $\nrep = 25$ initializations for each value of \tol. 
Finally, the initialization parameter $\toleranceinit$ is set to $10^{-11}$ and  
is increased by $10$ every $10000$ samples that do not result in a sub\-matrix to expand. 

\iffalse 
In the experiments with synthetic data, 
when the number of planted patterns is $1$, we run Algorithm~\ref{alg:rankone}, when it is between $2$ and $4$, we run  Algorithm~\ref{alg:rankone}~and~\ref{alg:rankk} with $\generalrank=2$ and finally when there are $5$ patterns, we additionally run Algorithm~\ref{alg:rankk} with $\generalrank=2$. In all cases, we set $\nrep = 25$.  

In the experiments with real-world data, we consider $\toleranceinit=10^{-10}$ and $\tol$ in $\{ 10^{-1}, 10^{-2}, 10^{-3}, 10^{-4} \}$. For each value of $\tol$, we explore $25$ initialization.

The details on the parameter settings of the baseline methods are given in~\ref{ap:additional_experimental_settings}. 
\fi 

%we run $100$ repetitions of Algorithm~\ref{alg:rankone}, 

\spara{Implementation.}
Our Python implementation is available online\footnote{\url{https://github.com/maciap/SaE}}.
Experiments are performed on a computer with
$2 \times 10$ core Xeon E5 processor and 256 GB memory. All reported results are averages over $10$ runs. %More details on the implementation of our method and of the baseline methods are given in~\ref{ap:additional_experimental_settings}. 


\subsection{Experiment Results}\label{sec:exp_results}
We first present results for the experiments in synthetic data %where a notion of ground-truth is available,
and then the results for the experiments in real-world datasets. 
%preliminary experiments, then for the task of near-rank-$1$ matrix recovery and finally for the task of general local-low-rank approximation. 
%In the preliminary experiments, we consider synthetic data with or without a planted near-rank-$1$ matrix. 
% PLASMA	Provably Low rAnk SubMAtrices 
% PLANE	Provably Low rANk Expansion	& PANORAMA	ProvAbly Near lOw RAnk subMAtrix	
% BELLS – Bounded-Error Low-rank Submatrices (memorable and smooth)
% PLOP	Provably LOwrank Patterns
% Acronym	Expanded	Score 
% NORRIS	Near lOw Rank matRIx Subsets

\spara{Results on synthetic datasets.}
Figure~\ref{fig:near_rank_one_recovery} presents results for the task of near-rank-$1$-submatrix discovery in $250 \times 250$ matrices of entries generated from six different probability distributions. %Figure~\ref{fig:near_rank_one_recovery_appendix} in~\ref{ap:additional_experiments} provides analogous results for other $5$ distributions. 
%Figure~\ref{fig:near_rank_one_recovery} shows results of the experiments for near-rank-$1$ submatrix recovery in the simple scenario where a single near-rank-$1$ submatrix is planted. 
The results show that our method  consistently recovers the ground truth (as indicated by $F_1$ score close to $1$ and reconstruction error close to $0$), which is not the case for the baseline approaches. 
More specifically, \rpsp tends to recover the ground-truth sub\-matrix as its size increases, but it is also considerably slower than the other methods. 
\sparsePCA and \svp are the fastest algorithms, but, like \cvx, they often fail in detecting the ground truth. 

We also observe significant variability in the results associated with different data-generating distributions. 
In particular, as suggested by Figure~\ref{fig:near_rank_one_recovery},  the only case where \ourmethod does not achieve an average $F_1$ score close to $1$ in near-rank-$1$ sub\-matrix recovery is for Poisson-distributed data with a planted near-rank-$1$ sub\-matrix accounting for the $10 \%$ percent of the total amount of entries.
The synthetic data are not scaled in pre\-processing. Thus, it is 
possible that the $F_1$ score would approach $1$ also in this case after suitably adjusting the parameter $\tol$ input to \ourmethod or normalizing the input matrix \inputmat. 


\begin{figure}[p]
\begin{center}
\input{images/tikz/legend_with_svp}
%\vspace*{-0.45cm}
    % Adjust cell width and image scale as needed
    %\setlength{\tabcolsep}{5pt} % Space between columns
    %\renewcommand{\arraystretch}{1.5} % Space between rows
    \begin{tabular}{ccc}
        & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_normal_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_normal_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_normal_125_250_1e05_4.pdf} \\
         & \textsc{Uniform} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_uniform_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_uniform_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_uniform_125_250_1e05_4.pdf} \\

        & \textsc{Exponential} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_exponential_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_exponential_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_exponential_125_250_1e05_4.pdf} \\


        & \textsc{Beta} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_beta_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_beta_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_beta_125_250_1e05_4.pdf} \\


        & \textsc{Gamma} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_gamma_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_gamma_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_gamma_125_250_1e05_4.pdf} \\


        & \textsc{Poisson} & \\
         \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/avg_rec_error_with_svp_poisson_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/f1_scores_with_svp_poisson_125_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryPlots/runtimes_with_svp_poisson_125_250_1e05_4.pdf} \\
        \vspace*{-0.65cm}
    \end{tabular}
\end{center}
\caption{
\label{fig:near_rank_one_recovery}
Full-rank synthetic $250 \times 250$ matrices generated from different probability distributions with a planted near-rank-$1$ submatrix.
Performance of different methods in the task of near-rank-$1$ submatrix discovery.  
We show the average (per-entry) reconstruction error (left), the $F_1$ score (center) and the runtime (right) of different methods as a function of planted submatrix size.
}
\end{figure}

\iffalse
The results indicate that our method outperforms the baselines in terms of $F_1$ score and reconstruction error, highlighting that our method retrieves the ground truth in most cases, which is not the case for the alternative approaches (an $F_1$ score of $1$ indicates that a method retrieves the ground truth \emph{exactly}). 
Unlike the other baselines, \rpsp tends to retrieve the ground truth when the size of the planted sub\-matrix increases. 
However, \rpsp is the slowest approach. 
Instead, \sparsePCA is the fastest algorithm, but it generally fails in retrieving the ground truth. 
It is interesting to notice that the dataset with the smallest planted sub\-matrix drawn from the Poisson distribution lead to the poorest results for our method, as this is the only case where our method fails to retrieve the ground truth. 
However, also in this case our method would uncover the ground truth after properly adjusting the parameters. 
\fi 

Figure~\ref{fig:local_low_rank_approximation_by_submatrices}  %in~\ref{ap:additional_experiments} show,
shows the same metrics as in Figure~\ref{fig:near_rank_one_recovery}, for synthetic data with entries generated from the same probability distributions,  
but in the setting where multiple, possibly overlapping, near-rank-$1$ sub\-matrices are planted and discovered. 
%Figure~\ref{fig:local_low_rank_approximation_by_submatrices_appendix} in~\ref{ap:additional_experiments} shows the same results 
%for matrices generated from other five distributions. 
% The overlap between different sub\-matrices can be close to a rank $\generalrank$ larger than one. 
%Thus, as outlined in~\ref{ap:additional_experimental_setup},  in this case, \ourmethod invokes both Algorithm~\ref{alg:rankone}~and~\ref{alg:rankk} to discover sub\-matrices close to rank $1$, $2$ and $3$.  
%in this case, as the number of planted submatrices grows, we also use Algorithm~\ref{alg:rankk} with $\generalrank$ set to $2$ or $3$ which increases runtime. 
%The results largely confirm the main findings of the experiments in the simpler setting where a single matrix is generated. 
% Like the results of the experiments in the simpler setting where a single matrix is generated, 
The results in this more challenging setting highlight that \ourmethod is the only method 
that consistently retrieves the ground-truth sub\-matrices.
%  showcasing the advantages of \ourmethod against existing approaches. 
Among the baselines, \sparsePCA stands out for its accurate reconstruction. 
However, the estimate $\estimate{\inputmat}$ of the input matrix it generates quickly becomes very dense as more sub\-matrices are discovered, and hence this approach fails to identify the locations of the ground-truth sub\-matrices. 
%\ourmethod becomes the number of planted sub\-matrices 

%\cnote[AG]{What becomes dense?}
%\cnote[MC]{Same as previous note - the estimate}

\iffalse 
%In this case, however, the performance generally deteriorates for all methods as the number of generated near-rank-$1$ submatrices increases. 
Sparse PCA performs well in this scenario, quickly providing accurate reconstructions consistently as the number of planted patterns increases and the number of PCA components increase accordingly. 
However, it produces dense matrices so that it is not possible to identify the location of the planted low-rank patterns, resulting in low $F_1$ score. 
On the other hand, our method with little runtime overhead, guarantees both small reconstruction error and high $F_1$ score. 
\fi 

% now figure for multiple planted submatrices 
%Figure~\ref{fig:prelimary_full_rank} presents results for matrices without planted near-rank-$1$ submatrices, and Figure~\ref{fig:prelimary_planted} shows results for matrices with a planted near-rank-$1$ submatrix. 
%\spara{Near-rank-$1$ Submatrix Recovery}
\begin{figure}[p]
\begin{center}
\input{images/tikz/legend_with_svp}
    \begin{tabular}{ccc}
         & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_normal_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_normal_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_normal_5_250_1e05_4.pdf} \\
        
         & \textsc{Uniform} & \\
         \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_uniform_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_uniform_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_uniform_5_250_1e05_4.pdf} \\

         & \textsc{Exponential} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_exponential_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_exponential_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_exponential_5_250_1e05_4.pdf} \\


         & \textsc{Beta} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_beta_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_beta_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_beta_5_250_1e05_4.pdf} \\


         & \textsc{Gamma} & \\
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_gamma_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_gamma_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_gamma_5_250_1e05_4.pdf} \\


         & \textsc{Poisson} & \\
         \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/avg_rec_error_with_svp_poisson_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/f1_scores_with_svp_poisson_5_250_1e05_4.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/nearRankOneRecoveryFiveSubmatricesPlots/runtimes_with_svp_poisson_5_250_1e05_4.pdf} \\
        \vspace*{-0.65cm}
    \end{tabular}
\end{center}
\caption{
\label{fig:local_low_rank_approximation_by_submatrices}
Full-rank synthetic $250 \times 250$ matrices generated from different probability distributions with multiple (possibly overlapping) planted near-rank-$1$ submatrices.
Performance of different methods in discovering planted submatrices. 
We show the average (per-entry) reconstruction error (left), the $F_1$ score (center) and the runtime (right) as a function of the number of planted submatrices. 
}
\end{figure}

% here we need the results for the local low rank apprx 
Finally,  
Figure~\ref{fig:noise} in~\ref{ap:additional_experiments} 
demonstrates the robustness of our method with respect to noise. 
% shows the same metrics shown in Figure~\ref{fig:near_rank_one_recovery}, but as a function of the level of noise, demonstrating the robustness of our method in the presence of noise. 

\spara{Results on real-world data.}
% \cnote[MC]{I have chosen 3 (hopefully representative) datasets to show both characteristics of data and result tables, but then move all the others to appendix. }
Table~\ref{tab:results_real_data} reports low-rankness score and size averaged over the top-$5$ 
sub\-matrices retrieved by our method, \svp and \rpsp in real-world datasets. 
%Similar results for the other $12$ datasets are given in~\ref{ap:additional_experiments} (Table~\ref{tab:results_real_data_appendix}). 
%Specifically, the tables report the relative percentage increase in low-rankness score and the size as percentage on entries of the input matrix 
To determine the top-$5$ sub\-matrices returned by each method, 
we select those that maximize the minimum between the low-rankness score and the size. 
%The top-$5$ submatrices are selected so as to maximize the minimum between the low-rankness score and the size. 
Moreover, to offer a more complete picture, in the appendix (Figure~\ref{fig:real_data_top_five_patters}), we additionally display the low-rankness and size of the individual top-$5$ patterns. 

%
%Finding a large sub\-matrix is easier than finding a sub\-matrix with large low-rankness score.  
%and thus, considering the low-rankness score is important. 
Finding sub\-matrices with high low-rankness is not an easy task. 
\svp returns large sub\-matrices. 
However, those sub\-matrices usually have smaller low-rankness 
compared to those discovered by our method and \rpsp, and, in several cases, compared to the input matrix. 
%Therefore, \svp is mostly useful when runtime is of primary importance. 
\ourmethod and \rpsp % perform more computations than \svp, and 
are more likely than \svp to return sub\-matrices with large low-rankness.
Furthermore, \ourmethod tends to discover sub\-matrices that strike a more desirable balance between low-rankness and size compared to \rpsp. 

As concerns runtime, \ourmethod is drastically faster than \rpsp in smaller datasets, but it can become slower in larger datasets. 
Nonetheless, the runtime of our method could be significantly reduced by leveraging a more efficient approach to maximum-edge-bi\-clique extraction and by reducing the number of iterations, which, however, could deteriorate the quality of the results. As mentioned in Section~\ref{sec:scalability}, future work will study the performance of different heuristic approaches to maximum-edge-bi\-clique extraction in terms of quality of the results, efficiency and scalability. 



%it would be sufficient to leverage a more efficient appraoch 
% Thus, the results demonstrate the advantages offered by our method over the state of the art in real-world datasets, although they are not as evident as when a ground truth is available.
%\svp is very fast, but generally returns sub\-matrices of lower low-rankness 
%Our method 


For our method, 
we also explore the trade-off between size and low-rankness by varying the value of $\tol$;
the results are presented in~\ref{ap:additional_experiments}.
%In~\ref{ap:additional_experiments} we show how size and low-rankness vary with $\tol$ in three example datasets.
% In~\ref{ap:additional_experiments}, we show, for four datasets, how the low-rankness score and the size of the sub\-matrices output by our method vary as a function of the tolerance parameter $\tol$. 





\iffalse 
Our method is often, but not always, considerably faster in returning the output submatrices $\outputmat$ than \rpsp. 
In this regard, it is important to observe that the flexibility inherent in our method  means that the method can be made significantly faster simply by using a faster heuristic in place of the spectral biclustering procedure. 
\fi 

%The results shown for our method depends on the choice of the parameter $\tol$. 


\begin{table}[t]
\centering
\caption{\label{tab:results_real_data} Performance in real-world data. For the top $5$ local low-rank patterns identified by the methods, we show the average relative percentage increase (L-R) with respect to the low-rankness score of the input matrix, the size (in percentage of entries of the input matrix) and the runtime (in seconds) to obtain them. }
    \begin{tabular}{l rrr rrr rrr}
        \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{\svp}  & \multicolumn{3}{c}{\rpsp} & \multicolumn{3}{c}{\ourmethod} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
        & L-R & Size & Runtime & L-R & Size & Runtime & L-R & Size & Runtime \\
        \midrule
        \Hyperspectral & 4.05 & 2.88 & 47.0 & 9.84 & 2.10 & 590 & 11.09 & ~21.43 & 1\,697 \\ 
        %\Isolet & 0.81 & 3.21 & 11.40 &  0.92  & 3.51  & 409 & 0.95 & 9.90 & 650 \\
        %Swamp & 0.99 & 2.19 &  9.32 & 1.00 & 0.03  & 364 & 1.00 & 0.05 & 502 \\
        %\Olivetti &  0.94 & 4.30 & 3.16 & 0.98 & 0.03  & 366 & 0.99 & 0.05 & 207 \\
       
        %\OrlRnSp & 0.93 & 4.38 &  0.63 & 0.98 & 0.02  & 386 & 0.99 & 0.04 & 58 \\
        %Credit & 0.92 & 3.93  & 322 & 1.00 & 14.10 & %2792 \\
        %\Jester & 0.65 & 3.72 & 3.52 & 0.96 & 0.02  & 264 & 0.96 & 0.14 & 47 \\
        %\Golub  & 0.99 & 0.29 & 14.72 & 1.00 & 0.02  & 161 & 1.00 & 0.19 & 61 \\
        %\Mandrill &  0.95 & 2.29 &  1.17 & 0.98  &  2.37 & 404  &  0.98 & 3.16 &  43 \\ 
        %\Ozone  & 0.6 & 0.73 & 1.87 & 1.00 & 0.03  & 211 & 1.00 & 0.17 & 24 \\
        %\SKCM & 0.82 & 5.25 & 0.43  & 0.85 & 0.03  & 295 & 0.9 & 0.03 & 24 \\
        %\BRCA & 0.80 & 5.16 & 0.33 & 0.83 & 0.02  & 371 & 0.85 & 0.06 & 29 \\
        %\PRAD &  0.83 & 4.23 & 0.36 & 0.84 & 0.03  & 308 & 0.85 & 0.06 & 25 \\
        %\Google & 0.84 & 4.40 & 3.88 & 0.90 & 0.03  & 145 & 0.93 & 0.07 & 17 \\
        %\NPAS & 0.24 & 15.85 & 0.22 & 0.92 & 0.04  & 246 & 1.00 & 0.20 & 23 \\
        %\MovieTrust & 0.74 & 4.05 & 0.26 & 0.61 & 4.23  & 209 & 0.94 & 10.5 & 9 \\      
        %\Hearth & 0.78 & 2.72 & 0.38 & 0.99 & 0.04  & 107 & 0.97 & 0.21 & 5 \\
        %Diabetes & 0.99 & 0.04  & 88 & 1.00 & 0.35 & 3 \\
        %\Imagenet & 0.95 & 4.85 & 0.41 & 0.96 & 0.04 & 126 & 0.99 & 0.02 & 31 \\

        \Isolet & -8.08 & 3.21 & 11 & 4.06 & 3.51 & 409 & 7.08 & 9.9 & 650 \\ 
        %Swamp & 0.99 & 2.19 &  9.32 & 1.00 & 0.03  & 364 & 1.00 & 0.05 & 502 \\
        \Olivetti & -1.39 & 4.3 & 3 & 2.23 & 2.81 & 366 & 3.83 & 5.2 & 207 \\ 
        % \MoiveLens & 0.44 & 8.59 & 1.45 & 0.43 &  2.85 & 124 & 0.61 & 1.13 & 121 \\
         \MovieLens & 49.61 & ~8.59 & 1.0 & ~46.69 & ~2.88 & 373 & ~116.42 & 1.06 & 152 \\ 
        \OrlRnSp & -1.51 & 4.39 & 1 & 2.84 & 1.92 & 386 & 3.65 & 4.29 & 58 \\  
        %Credit & 0.92 & 3.93  & 322 & 1.00 & 14.10 & %2792 \\
        %\Jester & 0.65 & 3.72 & 3.52 & 0.96 & 0.02  & 264 & 0.96 & 0.14 & 47 \\
        \Golub & -0.32 & 0.29 & 15 & 0.01 & 2.39 & 161 & 0.07 & 19.43 & 61 \\ 
        \Mandrill & 3.25 & 2.3 & 1 & 6.53 & 2.37 & 404 & 6.14 & 3.16 & 43 \\ 
        \Ozone & -39.92 & 0.74 & 2 & 0.03 & 3.23 & 211 & 0.16 & 16.76 & 24 \\ 
        %\SKCM & 0.82 & 5.25 & 0.43  & 0.85 & 0.03  & 295 & 0.9 & 0.03 & 24 \\
        \BRCA & 11.39 & 5.17 & 0 & 14.19 & 2.18 & 371 & 4.97 & 39.44 & 29 \\ 
        %\PRAD &  0.83 & 4.23 & 0.36 & 0.84 & 0.03  & 308 & 0.85 & 0.06 & 25 \\
        \Google & 11.22 & 4.4 & 4 & 18.78 & 2.55 & 145 & 22.63 & 7.16 & 17 \\ 
        \NPAS & -71.29 & 15.86 & 0.2 & 8.55 & 3.93 & 246 & 17.57 & 19.52 & 23 \\ 
        %\Cameraman & 0.87 & 3.64 & 0.32 & 0.91 & 0.03  & 102 & 0.98 & 0.25 & 18 \\
        \Cameraman & 1.69 & 3.64 & 0.3 & 5.67 & 3.44 & 102 & 14.44 & 24.83 & 18 \\ 
        \MovieTrust & -2.37 & 4.05 & 0.3 & -20.79 & 4.23 & 209 & 22.49 & 10.49 & 10 \\  
        \Hearth & -16.31 & 2.72 & 0 & 5.13 & 3.63 & 107 & 3.89 & 20.9 & 5 \\ 
        %Diabetes & 0.99 & 0.04  & 88 & 1.00 & 0.35 & 3 \\
       \Imagenet & 3.44 & 4.85 & 0.4 & 5.26 & 3.98 & 126 & 8.52 & 2.29 & 31 \\ 

       
        \bottomrule
    \end{tabular}
\end{table}





\iffalse 
\begin{table}[t]
\scriptsize
\centering
\caption{\label{tab:results_real_data} Performance in real-world data. For the top $5$ local low-rank patterns identified by the methods, we show the avelow-rankness score (L-R Score), the size (in percentage of entries) and the runtime (in seconds) to obtain them. }
    \begin{tabular}{l ccc ccc ccc}
        \toprule
        \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{\svp}  & \multicolumn{3}{c}{\rpsp} & \multicolumn{3}{c}{\ourmethod} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
        & L-R Score & Size & Runtime & L-R Score & Size & Runtime & L-R Score & Size & Runtime \\
        \midrule
        \Hyperspectral  & 0.92 & 2.88 & 46.67 & 0.98 & 2.1 & 590 & 0.99 & 21.43 & 1696 \\
        %\Isolet & 0.81 & 3.21 & 11.40 &  0.92  & 3.51  & 409 & 0.95 & 9.90 & 650 \\
        %Swamp & 0.99 & 2.19 &  9.32 & 1.00 & 0.03  & 364 & 1.00 & 0.05 & 502 \\
        %\Olivetti &  0.94 & 4.30 & 3.16 & 0.98 & 0.03  & 366 & 0.99 & 0.05 & 207 \\
        \MoiveLens & 0.44 & 8.59 & 1.45 & 0.43 &  2.85 & 124 & 0.61 & 1.13 & 121 \\
        %\OrlRnSp & 0.93 & 4.38 &  0.63 & 0.98 & 0.02  & 386 & 0.99 & 0.04 & 58 \\
        %Credit & 0.92 & 3.93  & 322 & 1.00 & 14.10 & %2792 \\
        %\Jester & 0.65 & 3.72 & 3.52 & 0.96 & 0.02  & 264 & 0.96 & 0.14 & 47 \\
        %\Golub  & 0.99 & 0.29 & 14.72 & 1.00 & 0.02  & 161 & 1.00 & 0.19 & 61 \\
        %\Mandrill &  0.95 & 2.29 &  1.17 & 0.98  &  2.37 & 404  &  0.98 & 3.16 &  43 \\ 
        %\Ozone  & 0.6 & 0.73 & 1.87 & 1.00 & 0.03  & 211 & 1.00 & 0.17 & 24 \\
        %\SKCM & 0.82 & 5.25 & 0.43  & 0.85 & 0.03  & 295 & 0.9 & 0.03 & 24 \\
        %\BRCA & 0.80 & 5.16 & 0.33 & 0.83 & 0.02  & 371 & 0.85 & 0.06 & 29 \\
        %\PRAD &  0.83 & 4.23 & 0.36 & 0.84 & 0.03  & 308 & 0.85 & 0.06 & 25 \\
        %\Google & 0.84 & 4.40 & 3.88 & 0.90 & 0.03  & 145 & 0.93 & 0.07 & 17 \\
        %\NPAS & 0.24 & 15.85 & 0.22 & 0.92 & 0.04  & 246 & 1.00 & 0.20 & 23 \\
        \Cameraman & 0.87 & 3.64 & 0.32 & 0.91 & 0.03  & 102 & 0.98 & 0.25 & 18 \\
        %\MovieTrust & 0.74 & 4.05 & 0.26 & 0.61 & 4.23  & 209 & 0.94 & 10.5 & 9 \\      
        %\Hearth & 0.78 & 2.72 & 0.38 & 0.99 & 0.04  & 107 & 0.97 & 0.21 & 5 \\
        %Diabetes & 0.99 & 0.04  & 88 & 1.00 & 0.35 & 3 \\
        %\Imagenet & 0.95 & 4.85 & 0.41 & 0.96 & 0.04 & 126 & 0.99 & 0.02 & 31 \\
        \bottomrule
    \end{tabular}
\end{table}
\fi 



\iffalse 
\subsection{Experimental Plan}

\spara{Preliminary experiments.}
Preliminary experiments seek to answer the following questions: 
\begin{itemize}
    \item What is the likelihood of observing near-rank-$1$ matrices? We can consider submatrices of size $2 \times 2$, $4 \times 4$ etc.. 

    \item What is the size of such near-low-rank matrices? 

\end{itemize}

We can investigate in both synthetic data (i.i.d.) and real-world data. 

Another important question concerns what is the best heuristic to eschew maximum-edge biclique? 

\spara{Recovery near-rank-1 submatrices}
We can carry out experiments primarily in synthetic data with ground truth to evaluate the ability of our method in recovering near-rank-1 submatrices. 
\begin{itemize}
    \item We compare against RPSP, convex optimization, sparse PCA... 

    \item We expect our method to achieve the most savings over baselines in this setting. 

    \item We can also consider the more challenging setting where there are more than one rank-1 submatrices, possibly overlapping. 

    \item We also evaluate the impact of noise by showing results for different noise levels... 
    
\end{itemize}

\spara{General local low-rank approximation}
We carry out experiments primarily to investigate the performance our method in real-data for the task of local-low-rank approximation. 
\begin{itemize}
    \item RPSP is expected to be most useful in this setting and represents our strongest baseline. 

    \item Unlike RPSP, our method needs as input the ranks we are looking for (or at least an upper bound). 

    \item We will need heuristic to guarantee efficiency in real-data and avoid maximum edge-biclique when the problem size is too large.. 
\end{itemize}



In this section, we present experiments to evaluate the methods we introduce. 

\spara{Baselines}
We compare our methods against several baselines. 
In the task of recovering a near rank-1 submatrix injected into a larger matrix, we consider: 
\begin{itemize}
    \item RPSP~\cite{dang2023generalized}.
    \item Sparse PCA~\cite{mairal2009online}. 
    \item Nuclear norm minimization~\cite{doan2013finding}. 
\end{itemize}

\spara{Synthetic data}
We conduct experiments on both synthetic and real-world datasets. 

For near-rank-1 submatrix recovery,  we consider the following data-generating mechanism to generate synthetic data.

\begin{itemize}
    \item First, we generate vectors $\mathbf{u} \in \real^n$ and $\mathbf{v} \real^n$ according to a given probability distribution $\mathcal{P}$. 

    \item We compute the rank-1 matrix $\mathbf{X} = \mathbf{u} \mathbf{v}^T \in \real^{n' \times m'}$ and we inject additive noise generated according to the probability distribution $\mathcal{P}$, rescaled by a factor $\epsilon_{noise}$ and re-centered. 

    \item We finally generate a larger matrix $\mathbf{D} \in \real^{n \times m}$ by resampling the entries of the submatrix $\mathbf{X}$.
\end{itemize}

The above data-generating mechanism is designed to make the near-rank-1 matrix recovering as challenging as possible. 
We consider different choices for the distribution $\mathcal{P}$, namely standard normal, uniform in $[0,1]$, exponential of rate $1$, Beta of parameters $2$ and $3$, Gamma of shape $2$ and scale $1$ and Poisson of rate $5$. 

\spara{Metrics.}
To evaluate the performance of a method in near-rank-1 submatrix recovery, we rely on the $F_1$ score and the average reconstruction error, i.e., the squared $L_2$ norm of the difference between the rank-1 reconstruction and the original submatrix.


\subsection{Results}

\spara{Near rank-$1$ matrix recovery.}
Figure~\ref{fig:synthetic_near_rank_one_recovery} presents results for near-rank-1 matrix recovery. 


\begin{figure}[t]
\begin{center}
    % Adjust cell width and image scale as needed
    \setlength{\tabcolsep}{5pt} % Space between columns
    \renewcommand{\arraystretch}{1.5} % Space between rows

    \begin{tabular}{ccc}

        & \textsc{Normal} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scorenormal_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_normal_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_normal_25_50.pdf} \\

        & \textsc{Uniform} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scoreuniform_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_uniform_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_uniform_25_50.pdf} \\

        & \textsc{Exponential} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scoreexponential_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_exponential_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_exponential_25_50.pdf} \\

        & \textsc{Beta} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scorebeta_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_beta_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_beta_25_50.pdf} \\

        & \textsc{Gamma} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scoregamma_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_gamma_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_gamma_25_50.pdf} \\

        & \textsc{Poisson} & \\
        \includegraphics[width=0.3\textwidth]{images/f1_scorepoisson_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/avg_error_poisson_25_50.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/runtime_poisson_25_50.pdf} \\
    \end{tabular}
\end{center}
\caption{
\label{fig:synthetic_near_rank_one_recovery}
Near-rank-1-submatrix recovery on synthetic data. 
We show $F_1$ score (left), average reconstruction error (center) and runtime (right) for matrices with i.i.d. entries drawn from six different distributions. 
}
\end{figure}


\spara{Impact of initialization.}
To evaluate the importance of the initialization strategy we introduce, we compare the results of our method with those that would be obtained via random initialization. 
More specifically, in random initialization, the rows and columns in $\initialmat$ are chosen uniformly at random, regardless of the determinant of \initialmat. 
Figure~\ref{fig:initialization_impact} presents the comparison in synthetic data. 

\begin{figure}[t]
\begin{center}
    \begin{tabular}{ccc}
        \textsc{Normal} & \textsc{Uniform} & \textsc{Exponential} \\
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_size_normal_50_100.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_size_uniform_50_100.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_size_exponential_50_100.pdf} \\
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_avg_error_normal_50_100.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_avg_error_uniform_50_100.pdf} & 
        \includegraphics[width=0.3\textwidth]{images/ablation_initialization_avg_error_exponential_50_100.pdf} \\
    \end{tabular}
\end{center}
\caption{
\label{fig:initialization_impact}
Impact of initialization strategy. 
On synthetic matrices with i.i.d. entries drawn from different distributions, we show the size of the retrieved matrix and the associated reconstruction error. 
}
\end{figure}


\spara{Performance of heuristic approach to maximum-edge biclique.}
\fi 

==> arXiv-2506.06456v1/images/tikz/legend_only_rpsp.tex <==
\begin{tikzpicture}[scale=0.1]
\matrix [matrix of nodes, 
column sep=1.5pt, 
row sep=0pt, 
nodes={anchor=center}] (m) {
% Dark Magenta Transparent Rectangle with Thick, Less Transparent Border
\node[draw=darkmagenta, fill=darkmagenta, line width=1pt, fill opacity=0.3, draw opacity=0.9, rectangle, inner sep=2.9pt] {}; 
& {\small \svp}
& 
% Red Transparent Rectangle with Thick, Less Transparent Border
\node[draw=crimson, fill=crimson, line width=1pt, fill opacity=0.3, draw opacity=0.9, rectangle, inner sep=2.9pt] {}; 
& {\small \rpsp} 
& 
% Orange Transparent Rectangle with Thick, Less Transparent Border
\node[draw=orange, fill=orange, line width=1pt, fill opacity=0.3, draw opacity=0.9, rectangle, inner sep=2.9pt] {}; 
& {\small \ourmethod} \\
};
\end{tikzpicture}


==> arXiv-2506.06456v1/images/tikz/legend_with_svp.tex <==
\begin{tikzpicture}[scale=0.1]
\matrix [matrix of nodes, 
column sep=1.0pt, % moderately reduced
row sep=0pt, 
nodes={anchor=center}] (m) {
% Blue Circle with Line
\tikz \draw[slateblue, thick] (-0.18,0) -- (0.18,0) 
node[fill=slateblue, circle, inner sep=2.1pt] {};
& {\small Sparse PCA}
& 
% Green Upward Triangle with Line
\tikz \draw[darkolivegreen, thick] (-0.18,0) -- (0.18,0) 
node[fill=darkolivegreen, regular polygon, regular polygon sides=3, inner sep=1.4pt] {};
& {\small \cvx}
& 
\tikz \draw[darkmagenta, thick] (-0.18,0) -- (0.18,0) 
node[fill=darkmagenta, regular polygon, regular polygon sides=3, inner sep=1.7pt, rotate=180] {};
& {\small \svp}
& 
% Red Diamond with Line
\tikz \draw[crimson, thick] (-0.18,0) -- (0.18,0) 
node[fill=crimson, diamond, inner sep=1.7pt] {};
& {\small \rpsp} 
& 
% Orange Square with Line
\tikz \draw[orange, thick] (-0.18,0) -- (0.18,0) 
node[fill=orange, rectangle, inner sep=2.6pt] {};
& {\small \ourmethod} \\
};
\end{tikzpicture}


==> arXiv-2506.06456v1/introduction_arxiv.tex <==
\section{Introduction}\label{sec:introduction}

% \cnote[MC]{Introduction should be about two pages. Note negative vspace to save space is not allowed. }

% Low rank approximation 
Low-rank approximation has emerged as a fundamental task in many data-analysis applications, including machine-learning pipelines~\cite{wang2017research}, large language models~\cite{hu2021lora}, recommender systems~\cite{lee2016llorma}, 
image compression and de\-noising~\cite{guo2015efficient}.
%Recently, with the rise of large language models, low-rank approximation has been proven to be a valuable tool for compressing such  
The goal of low-rank approximation is to represent an input matrix as accurately as possible using a small number of row and column vectors. 
%The rank of a matrix indicates the maximum number of linearly independent rows or columns, and 
%the lower the rank, the more a matrix can be compressed. 
%  with small information loss. 
%The goal of low-rank approximation is to represent an input matrix using a small number of basis vectors. 
%  that capture the important structure of the matrix. 
% 
% Over the years, low-rank approximation has achieved remarkable success across diverse applications. 
%, from data compression and dimensionality reduction to signal processing and machine learning. 
% For instance, 
%Low-rank approximation has been extensively used in machine-learning pipelines~\cite{wang2017research}, recommender systems~\cite{lee2016llorma}, 
%image compression and de\-%noising~\cite{guo2015efficient}. 

% The SVD 
% \spara{The singular value decomposition.}
For decades, the \emph{singular value decomposition} (\svd), 
with the closely related principal component analysis (PCA), 
has remained the gold standard for low-rank approximation~\cite{golub2013matrix}.
% , celebrated for % its mathematical elegance and  its optimality guarantees.
%holds a central position in low-rank approximation.  
%In particular, for decades, the \svd  has remained the gold standard for low-rank approximation, celebrated for its mathematical elegance and optimality guarantees (the Eckart-Young-Mirsky theorem~\cite{chipman2020proofs} guarantees that the \svd provides the closest low-rank approximation to an input matrix in terms of Frobenius or spectral norm). 
%The \svd decomposes a matrix into two unitary matrices of singular vectors and a diagonal matrix of singular values. 
%Singular values reveal the low-rankness property of a matrix. 
% 
% \spara{The need for new (and local) low-rank approximation methods.}
%Despite its well-justified success, the \svd also has certain drawbacks in some applications. 
%Despite its well-founded success, SVD has limitations for some applications.
Despite its %  well-founded 
success, \svd has certain limitations. 
%First, it may not scale to very large matrices. 
% First,  the \svd may lack interpretability:
% for instance, even if the data are non-negative,  the singular vectors may still contain negative values.  
%  in terms of the original data/
%  making it challenging to understand the specific contributions of individual rows or columns to the overall structure.
% Second, and more relevant to this work, 
Among others, when applying \svd we aim to find a low-rank approximation for the entire input matrix. 
%  well-approximated by a low-rank structure. 
%As shown in Figure~\ref{fig:movielens_example}, 
This assumption can be rather restrictive, as in real-world data
it might be that only certain sub\-matrices are well approximated by low-rank structures.
% and not the entire input matrix. 
% there can often be low-rank sub\-matrices that arise naturally from phenomena that are \emph{local} in nature. 
% The \svd may completely fail to identify such localized phenomena. 
% In other words, in real-world data matrices, there can be sub\-matrices that are very well approximated by a low-structure and others that are not; 
% the \svd does not distinguish between them. 
%On the other hand, other sub\-matrices, may not be accurately represented by any low-rank structure. 
\iffalse
% insert examples here 
For example, in approaches to recommender systems based on low-rank approximation, the crucial assumption is that there exist a set of underlying latent factors determining whether a user would like an item or not. 
In the case of movie recommendations, such factors may e.g. represent the affinity of a user with a certain director and main actor.
The factors are learned from the entire matrix and thus capture affinities that are assumed to hold for all users and items. 
In the real world, however, this assumption can be too simplistic. 
A user may share similar taste in
drama movies with a certain group of users, while having similar preferences with a different group of users in thriller movies.
As a consequence, there may be latent factors that explain particularly well only some regions of the rating matrix. 
In addition to recommender systems, similar local patterns are observed in data coming from very different domains, such as market-basket analysis, image processing and biology~\cite{dang2023generalized}. 
\fi 
%For example, in data originating in movie recommender systems, 
%a subset of users may share a similar taste only for a subset of movies. 
For instance, in ratings data originating in movie recommender systems, 
%such as the ones considered in Figure~\ref{fig:movielens_example},
low-rank submatrices occur because subsets of users may share a similar taste only for a subset of movies. 
%As a consequence, low-rank structures arising from a small number of latent factors
%may be present only on sub\-matrices of the movie-rating data. 
%In addition to recommender systems, 
Similar local patterns could be observed in data coming from other domains, 
such as market-basket analysis, image processing, and~biology~\cite{dang2023generalized}. 
The \svd can fail to identify  local low-rank submatrices. 


\spara{Existing approaches to find local low-rank sub\-matrices.}
% Although the \svd 
%and other standard approaches for low-rank approximation 
% may disregard local patterns, 
The task of identifying sub\-matrices that are well described by low-rank structures has been largely overlooked until recently~\cite{dang2023generalized}. 
%Only recently work has been carried out to formally address the problem
Existing work in this direction is based primarily on 
the \svd, and 
%repeated expensive computation of the \svd for particular sub\-matrices. 
%Further, existing work 
does not provide any guarantee on the quality of the approximation for the identified sub\-matrices.  %and they do not offer ease of interpretation. 
%Finding sub\-matrices that are \emph{provably} close to their low-rank approximation 
%and easy to interpret can make the approximation more trustworthy, and would thus particularly useful for applications in high-stakes domains.  

\begin{figure}[t]
    \centering
    \begin{tabular}{c@{\hspace{1.5cm}}c}  % Two columns
         \scalebox{0.375}{\input{diagrams/line_in_three_d.tikz}} & 
        \scalebox{0.375}{\input{diagrams/plane_in_three_d.tikz}} \\
        %(a) Line structure in 3D & (b) Plane structure in 3D
        \textbf{(a)} & \textbf{(b)} \\ 
    \end{tabular}
    \caption{\label{fig:line_three_d} Example. A subset of data points (in orange) in the $3$-dimensional space are close to their projection (in red) onto a line in the $xy$-plane (a) or to a plane in the $3$-dimensional space (b), while other points (in blue) can be further away. }
\end{figure}



\spara{Our approach.}
In this work, we adopt a different perspective on discovering local low-rank patterns, and we address the problem of identifying sub\-matrices 
%without relying on the \svd, 
%while offering guarantees on the approximation quality
%of the discovered sub\-matrices. 
that are guaranteed to be close to a low-rank approximation. 
Our quality guarantees hold with respect to an approximation that can be easily interpreted 
in terms of the original data, which can be particularly valuable for applications in different domains. 
For example, near-rank-$1$ sub\-matrices can be accurately approximated 
by each row in the submatrix being colinear with a single row.  
%, and, if needed, a provably-accurate approximation of the submatrices that can be interpreted in terms of the original data.
%In addition, the discovered submatrices can be interpreted more easily in terms of the original data. 
%  and the possibility of interpreting the retrieved sub\-matrices in terms of the original data. 
Unlike previous work, our work does not directly rely on the \svd. % which can also yield computational advantages. 
Nearly-low-rank sub\-matrices correspond to subsets of points (matrix rows) 
that approximately lie on a low-dimensional sub\-space, 
for a subset of dimensions (matrix columns).
For rank equal to~$1$, which is a particularly interesting case, the points approximately lie on a line through the origin, and for rank equal to~$2$ the points are close to a plane through the origin, as in the example of Figure~\ref{fig:line_three_d}, which shows data points 
identifying a $15 \times 2$ near-rank-$1$ sub\-matrix and a $15 \times 3$ near-rank-$2$ sub\-matrix. 
%For simplicity of exposition, 
%We often discuss the near-rank-$1$ case, which is particularly interesting,
%and then explain how to generalize to sub\-matrices close to a rank greater than~$1$.
%The \svd is not expected to reveal such line. 

While \svd may fail to reveal dense lines in the data,
it is possible to find such structures by sampling. 
A na\"ive approach would be to sample subsets of points and dimensions 
until a large set of nearly-collinear points is found. 
However, this procedure quickly becomes inefficient. 
%The method that we introduce instead resort to sampling, but only in the initialization stage. 
Instead, to identify points approximately distributed along a line, we introduce a method that only relies on sampling in an initialization phase to find a minimal structure that can exhibit this property, i.e., two points in two-dimensions. 
%we introduce a novel method that only relies on sampling in the initialization stage.
%To retrieve the points approximately distributed along a line, we start by sampling 
%or equivalently a $2 \times 2$ matrix. 
In a subsequent phase, the $2 \times 2$ sub\-matrix is expanded deterministically to obtain the entire subset of points and dimensions associated with the target line. 
Based on such a two-phase method, we discover arbitrary sub\-matrices that admit low-rank approximations that can be easily interpreted in terms of the original sub\-matrix rows or columns, and are supported by quality guarantees. A real-world example is given in Figure~\ref{fig:first_figure}. % which shows a near-rank-$1$ sub\-matrix and its provably accurate approximation obtained by expressing each row as proportional to a single row. 


%, and, more generally, to find sub\-matrices that are provably close to a low-rank approximation. 
%This two-stage procedure is efficient because checking whether a $2 \times 2$ matrix belong to the target 
%sub\-matrix is fast, 
% only requiring two multiplications and one subtraction of scalars, 
%and thus, in the initialization stage we can quickly explore many regions of the data matrix. 
%In this work, we leverage a similar two-stage procedure to find sub\-matrices with entries that are \emph{provably} close to their low-rank approximation. 
%Based on the two-stage procedure sketched above, in this work we identify sub\-matrices that are provable close to a low-rank approximation.   

\spara{Our contributions.}
Our main contributions can be summarized as follows. 

\begin{itemize}
    \item We formalize the problem of finding sub\-matrices that are provably close to a low-rank approximation. 
    % \cnote[HM]{I'm not certain I understand this. If we find a low-rank submatrix, isn't it then its own low-rank approximation? Should it be "finding sub\-matrices that are provably close to their low-rank approximation"? }
    % \cnote[MC]{Yes}
    
    \item We introduce an effective method for finding sub\-matrices that are provably close to rank $1$. Then, we generalize this method to the %rank-$\generalrank$ case. 
    %\cnote[HM]{The expression "provably close to rank 1": does it mean that it is close to a rank-1 matrix"? Guaranteed to b}
    case of rank-\generalrank sub\-matrices. 

    %\item We generalize our methods to finding sub\-matrices that are provably close to a rank-$k$ approximation. 
    %  for any $k$, or sub\-matrices that are close to a rank-$k$ approximation after a suitable translation.
    \item We analyze the theoretical properties of the method we introduce. 

    \item We demonstrate the advantages of our method over previous work. %in extensive experiments. 
    % in detecting low-rank sub\-matrices. 
\end{itemize}
%\cnote[HM]{Does "provably close" mean something different from "close"? I understand the need to say that our results are different from those of SVP which just gives a submatrix that will or will not be close to rank 1, but somehow  saying provable sounds like there would be a complex proof behind this. Perhaps I'm misunderstanding something.}

\spara{Roadmap.} The rest of the paper is organized as follows. 
In Section~\ref{sec:related} we discuss related work. 
Section~\ref{sec:preliminaries} introduces the notation used throughout the paper as well as key preliminary concepts. 
In Section~\ref{sec:prob} we present the problem we study and in Section~\ref{sec:algorithms} we illustrate our method to address it. In 
Section~\ref{sec:analysis} we analyze the properties of the method, and in Section~\ref{sec:experiments} we assess its empirical performance.
%Section~\ref{sec:experiments} contains the empirical evaluation of our method. 
Finally, Section~\ref{sec:conclusion} provides conclusions. 



%Of course, 

\input{diagrams/firstfigure}






\iffalse 

\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth]{images/ratings_reordered_with_highlited_} & \includegraphics[width=0.33\linewidth]{images/ratings_approximated.pdf}
 & 
\includegraphics[width=0.33\linewidth]{images/ratings_approximated_svd.pdf}   \\
%Rating matrix & Rank-$1$ submatrix & \svd approximation
\end{tabular}
\caption{\label{fig:movielens_example} MovieLens user-item rating matrix of dimensions $943 \times 943$ ($0$ indicates missing ratings). %Rows and columns indicate users and movies respectively. Missing ratings have value $0$. For a matrix of ratings of dimensions $943 \times 943$,
We show the original ratings (re-ordered) with a (perfectly) rank-$1$ submatrix detected by our method  highlighted in grey (left). 
This submatrix refers to the ratings of $144$ users on $3$ movies (namely, 'Airheads'  'Killing Zoe' and 'Down Periscope'). 
We also the actual values of the submatrix (center) as well as the approximation provided by the global rank-$1$ \svd (right).
%The submatrix has exactly rank $1$ because all the $144$ users have given the same rating to the $3$ movies. 
}
\end{figure}
\cnote[HM]{Figure 1: Would there be another example (from another dataset?) where the rank-1 submatrix would have more columns? Now 144x3 sounds somewhat small.}
\cnote[MC]{ Yes, we need to find a better example or none.}
\fi 





%It assumes that the input data can be written as the sum of a number of rank-$1$ matrices of the same dimensions. 
%Such matrices are typically hard to interpret, as they are not even guaranteed to be in the same range as the data (e.g., even if the data contain only positive values, the rank-$1$ matrices of the \svd may contain negative values). 





%is the first thing that comes to mind when thinking about low-rank approximation


% limitations 
%For decades, the Singular Value Decomposition %(SVD) In particular, the famous 

\iffalse 
Recently, work has been done to challenge the role of the SVD as a gold standard for low rank approximation. 
For instance, Ciaperoni et al.~\cite{ciaperoni2024hadamard} introduce an extension of the SVD that accounts for multiplicative effects and retrieves more concise yet equally accurate representations of matrices and
%\cnote[]{We could cite the paper where they study reshaping of the data before SVD but i cannot find it}
Gleich~\cite{gleich2024better} shows that one can achieve a better low-rank approximation by computing the SVD after reshaping the original matrix. 
In this work, the authors seek to relax the crucial assumption underlying the SVD that the data have been generated as the sum of rank-1 matrices. 

Beside additivity, another important assumption of the SVD is its global nature. Each of the rank-1 matrices in the sum that the SVD uses to approximate an input matrices is dense and thus impacts all the entries in the input matrix. Thereby, the SVD implicitly assumes a global model where the input matrix is entirely approximated by a low-rank matrix. 
In some cases, however, only particular sub\-matrices will exhibit a low-rank structure. 
For example, in a matrix of ratings for recommender systems, a user may share similar taste in
drama movies with a certain group of users, while having similar preferences with a different group of users in thriller movies.
Similarly, in market-basket data, some customers may have similar purchasing habits only for a subsets of items. 
The SVD may fail to recognize such simple patterns. 
Thus, recently work has been carried out to investigate local low-rank structures~\cite{dang2023generalized,lee2016llorma}. 

Another relevant limitation of the SVD is that its components—singular vectors and singular values—lack direct interpretability in terms of the original data, making it challenging to understand the specific contributions of individual rows or columns to the overall structure.
To overcome such limitations, researchers have introduced more interpretable alternatives to the SVD such as the CUR decomposition~\cite{mahoney2009cur} and column subset selection algorithms~\cite{boutsidis2009improved}. 

Not only the SVD is difficult to interpret in terms of the original data points and dimensions, it may also yield approximation of some particular entries of the matrix that are far from the original values as the optimality guarantee only hold for the total approximation error and not for the approximation error at the level of the single error.
Previous work has also studied the problem of global low-rank approximation to minimize the maximum entry-wise deviation~\cite{gillis2019low}. 

% our goals 
In this work, we seek to relax the rather restrictive of existing low-rank approximation method and we introduce a simple yet effective method that: 
\begin{itemize}
    \item retrieves local low-rank structures in the input matrix; 

    \item offers guarantees on the approximation error of each entry in the matrix; 

    \item is highly interpretable in terms of the original data. 
\end{itemize}


A crucial idea underlying our work is that the problem of identifying local low-rank sub\-matrices can be approached in an \svd-independent manner. 

% general description 
In large data matrices, there are often subsets of points that lie close to a simple structure, such as a line or a plane. 
The method we introduce quickly retrieves such points in arbitrary subsets of dimensions and computes an interpretable low-rank approximation for the subsets of points. 
The algorithm starts by sampling minimal sets of entries that may lie in a low-rank structure, and then deterministically extend such set. 
We can show that if the target substructure is large enough, our algorithm quickly returns the desired approximation. 

\fi 



==> arXiv-2506.06456v1/long_defines.tex <==

\newcommand{\tikzgraphstyles}{
\tikzstyle{textbox}=[inner sep=0pt]
\tikzstyle{node}=[circle, minimum size=18pt, inner sep=3pt, fill=gray!50, text=white]
\tikzstyle{processed}=[fill=red!50]
\tikzstyle{edge}=[draw=gray, very thick]
\tikzstyle{uedge}=[draw=gray, very thick]
\tikzstyle{bedge}=[draw=gray, very thick, <->]
\tikzstyle{edgelabel}=[above=0.25em]
}



\newcommand{\brows}[1]{%
  \begin{bmatrix}
    \begin{array}{@{\protect\rotvert\;}c@{\;\protect\rotvert}}
      #1
    \end{array}
  \end{bmatrix}
}
\tikzset{%
  point/.style={circle, inner sep=2pt}, 
  other point/.style={fill=black, point}  
}



\makeatletter
\providecommand*{\cupdot}{%
  \mathbin{%
    \mathpalette\@cupdot{}%
  }%
}
\newcommand*{\@cupdot}[2]{%
  \ooalign{%
    $\m@th#1\cup$\cr
    \sbox0{$#1\cup$}%
    \dimen@=\ht0 %
    \sbox0{$\m@th#1\cdot$}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}

\providecommand*{\bigcupdot}{%
  \mathop{%
    \vphantom{\bigcup}%
    \mathpalette\@bigcupdot{}%
  }%
}
\newcommand*{\@bigcupdot}[2]{%
  \ooalign{%
    $\m@th#1\bigcup$\cr
    \sbox0{$#1\bigcup$}%
    \dimen@=\ht0 %
    \advance\dimen@ by -\dp0 %
    \sbox0{\scalebox{2}{$\m@th#1\cdot$}}%
    \advance\dimen@ by -\ht0 %
    \dimen@=.5\dimen@
    \hidewidth\raise\dimen@\box0\hidewidth
  }%
}
\makeatother




==> arXiv-2506.06456v1/preliminaries_arxiv.tex <==
\section{Preliminaries}\label{sec:preliminaries}


% Before we introduce the main ideas behind the proposed methods, we introduce notation and preliminary notions that are used throughout the paper. 

\para{Notation and basic definitions.}
%We consider an arbitrary data matrix, which may contain boolean, integer, or real values. 
Matrices are denoted by upper-case boldface letters, and we use $\inputmat$ to denote the input data matrix.  
%
$\inputmat_{i,j}$ indicates the entry of \inputmat in row $i$ and column $j$, while the $i$-th row and $j$-th column of \inputmat are denoted by $\inputmat_{i,:}$ and $\inputmat_{:,j}$, respectively. 
% 
Sets are denoted by upper-case letters and scalars by lower-case letters. % The $i$-th entry of vector \xvec is denoted by $x_i$.  
Vectors are denoted by lower-case boldface letters, e.g., $\xvec = (x_1, \dots, x_d)$.
We denote the $L_2$ (or Euclidean) norm of a vector $\xvec$ as $\| \xvec \|_2$ and 
the inner product between two vectors \xvec and \yvec as $\xvec^T \yvec$. 
%
We consider different matrix norms: 
the Frobenius norm  $\frobeniusnormshort{\inputmat} = (\sum_{i,j} |\inputmat_{i,j}|^2)^{1/2}$, 
the spectral norm $\spectralnormshort{\inputmat} = \sup_{||\xvec||_2\le 1} ||\inputmat\xvec||_2$, and 
the max norm % (or entry-wise infinity norm) 
$\infinitynormshort{\inputmat} = \max_{i,j} |\inputmat_{i,j}|$.
We use $\generalnormshort{\inputmat}$ with $*= \{ 2, F, \text{max}\}$ to indicate the above norms. 
We refer to the total number of entries of a (sub)matrix  \inputmat\ as its \emph{size}, which is also simply  denoted by~$\abs{\inputmat}$, if there is no risk of confusion with the entry-wise absolute value. 
\iffalse
Given a matrix \inputmat $\in \real^{\nrows \times \ncols}$, 
we generally denote by \outputmat $\in \real^{\nrows' \times \ncols'}$, 
with $\nrows'\le\nrows$ and $\ncols'\le\ncols$, 
a sub\-matrix of \inputmat. 
A sub\-matrix \outputmat is uniquely defined by a subset $\rowset'$ of the rows $\rowset$ of \inputmat and 
a subset $\colset'$ of columns  of the columns  $\colset$ of \inputmat. 
\fi
For a matrix \outputmat, we denote by $\estimate{\outputmat}$ a low-rank approximation of \outputmat and by 
$\outputerror$
%and by $\estimate{\outputmat}_{\generalrank}$ an approximation of rank $\generalrank$. 
%We use $\outputerror$ to denote 
the difference
% between \outputmat and $\estimate{\outputmat}$, that is, 
$\outputerror = \outputmat - \estimate{\outputmat}$. 


%We write $\det(\outputmat)$ to denote the determinant of \outputmat. %, and 
%$\rank(\outputmat)$ to denote the rank of \outputmat. 
%The rank of a matrix indicates the minimum number of linearly independent basis vectors 
%that span the row and column spaces of \inputmat. 
%The determinant does not reveal the rank of a matrix, 
%however, it indicates whether a matrix has full rank.
%  (i.e., it has the maximum possible rank) or rank-deficient. 

% \cnote[Aris]{I think that $\det(\cdot)$ and $\rank(\cdot)$ are not used elsewhere in the paper; so we do not need to define notation that is not used. }

\spara{Orthogonal projections.}
Given a nonzero vector $\xvec$ and a  vector $\yvec$, the \emph{orthogonal projection} of $\yvec$ onto $\xvec$ 
is given by
$\proj{\xvec}{\yvec} = ({\yvec^T \xvec})/({\xvec^T \xvec}) \xvec$.
% This projection operation gives the component of $\yvec$ that lies along $\xvec$, and the residual vector $\mathbf{r} = \yvec - \proj{\xvec}{\yvec}$ is orthogonal to $\xvec$, i.e., $\mathbf{r}^T \xvec = 0$
Similarly, given a matrix~$\bfB$ and a matrix $\bfA$ with linearly independent columns, 
the \emph{orthogonal projection} of~$\bfB$ onto the column space of $\bfA$ is given by
%$\proj{\bfA}{\bfB} = \bfA (\bfA^T \bfA)^{-1} \bfA^T \bfB$.
$\proj{\bfA}{\bfB} =  \bfA \bfA^+ \bfB$, where $\bfA^+ = (\bfA^T \bfA)^{-1} \bfA^T$ is the 
%
%Using the 
\emph{Moore-Penrose pseudoinverse} of $\bfA$.  %$\bfA^+ = $, 
%we can express $\proj{\bfA}{\bfB}$ more concisely as
%$\proj{\bfA}{\bfB} = \bfA \bfA^+ \bfB$.
The orthogonal projection
$\proj{\bfA}{\bfB}$ is the closest matrix to \bfB in the column space of \bfA under the Frobenius~norm.

%We use $\proj{\xvec}{\yvec}$ to denote the orthogonal project of a vector $\yvec$ onto the span of $\xvec$. 

% reconstructione error 


\spara{Low-rank approximation and \svd.}
The \emph{singular value decomposition} (\svd) of a matrix \(\inputmat \in \mathbb{R}^{\nrows \times \ncols}\) 
is given by $\inputmat = \bfU \bfSigma \bfV^T$,
where
\(\bfU \in \mathbb{R}^{\nrows \times \nrows}\) and  \(\bfV \in \mathbb{R}^{ \ncols  \times  \ncols  }\) 
are unitary matrices, and
\(\bfSigma \in \mathbb{R}^{ \nrows \times \ncols }\) is a diagonal matrix 
with singular values $\{ \sigma_1, \sigma_2 \dots \sigma_{\min\{\nrows,\ncols\}} \}$  as diagonal entries, conventionally sorted in decreasing order.
If the matrix is not clear from the context, we denote as $\sigma_i(\outputmat)$ the $i$-th singular value of $\outputmat$. 

It is known that 
the optimal rank-\generalrank approximation of \inputmat for the Frobenius and the spectral norm (but not for the max norm) is obtained from the \svd
by retaining the first 
\generalrank~singular values, along with the associated \generalrank~columns  of $\bfU$ and \generalrank~rows of $\bfV^T$\,\cite{golub2013matrix}. 
% and  \(\bfV \in \mathbb{R}^{ \ncols  \times  \ncols  }\) is an orthogonal matrix.
% \cnote[Aris]{We could simplify notation by saying that we assume  $\nrows\le\ncols$ and just use $\nrows$ instead of ${\min\{\nrows,\ncols\}}$. }
% \cnote[MC]{If this is not really used elsewhere, we can also keep it as it is?}
The largest singular value of a matrix equals its spectral norm, and the number of non-zero singular values indicates the rank of the matrix. 
% If a matrix \inputmat has at least a singular value equal to zero, it is said to be \emph{singular} (or not full-rank) and its determinant, denoted by $\det(\inputmat)$, is also equal to zero. 
As real-world data are often noisy, the singular values are seldom exactly zero.  
Accordingly, to measure the proximity of a matrix to rank $1$, in this work, 
we use the \emph{low-rankness score}~\cite{dang2023generalized}, which is given by 
\( \lowrankness{\outputmat} = \frac{\sigma_1(\outputmat)^2}{  \sum_{i = 1}^{\min(\nrows, \ncols)} \sigma_i(\outputmat)^2} \). 
% For the purpose of this work, 
A matrix whose singular values after the $\generalrank$-th one are close to zero
can be accurately approximated by a rank-\generalrank matrix, and is loosely referred to as \emph{near-rank-\generalrank} matrix. 
% Near-rank-\generalrank matrices, which are the focus of our work, 
% admit close approximation in terms of rank-\generalrank matrices. 
% More formally, they are such that $\generalnormshort{\outputerror}$ is bounded by a small scalar. % $\tol$. 

% For space reasons, more details on the \svd and its role in low-rank approximation are given in~\ref{ap:technical_details}.

% \cnote[AG]{I introduced the notation $\lowrankness{\cdot}$ here but I am not sure if it is used elsewhere.}











\iffalse
The \svd holds a central position in low-rank approximation because it provides the optimal rank-\generalrank approximation of \inputmat in terms of Frobenius or spectral norm. However, it does not offer guarantees in terms of error at the individual-entry level. In this work, we seek to approximate solely those entry that admit an accurate representation in terms of a low-rank structure. 
\fi 

% \cnote[MC]{Moved the rest of the section to the appendix.}





\iffalse 
For the sake illustration,  we do not shuffle the data so that the submatrix entries appear contiguous. However, neither \rpsp nor our method require the submatrix entries to be contiguous. 
\rpsp extracts clusters of rows and columns from the scoring matrix via co-clustering. 
Our methods also extracts the near-rank-$1$ submatrix. 
In particular, our method recovers exactly the near-rank-$1$ submatrix, achieving an $F_1$ score of $1$, while \rpsp achieves an $F_1$ score of $0.67$. 
\fi 






%As noticed by~\citet{dang2023generalized}, \svd (or the closely related principal components analysis) with sparsity constraint can recover the near-rank-$1$ submatrix only when such matrix 
%Co-clustering methods may also be able to identify local low-rank submatrices in case their mean deviates significantly from the background. 























\iffalse 
% matrix product
Given two matrices \A and \B of dimensions $\nrows \times p$ and $p \times \ncolumns$, respectively, their 
standard matrix product is a matrix $\Pprod = \A \B$ of dimensions $\nrows \times \ncolumns$ where $\Pprod_{i,j}$ is obtained as the dot product between the $i$-th row of \A and $j$-th column of \B. 

% introduce the Hadamard product 
Furthermore, given two matrices \done and \dtwo both of dimensions $\nrows \times \ncolumns$,
we define their Hadamard (or element-wise) product as the matrix $\inputmat = \done \odot \dtwo$ 
of dimensions $\nrows \times \ncolumns$,
where entry $\inputmat_{i,j}$ is obtained as the (scalar) product $[\done]_{i,j}[\dtwo]_{i,j}$. 

We next state the simple bounds on the rank of a Hadamard product and on expressing a low-rank matrix as a Hadamard product.
\fi 

\iffalse
\cnote[HM]{Add some references to the proposition.}{}{}
\cnote[MC]{Added two references mentioning the properties of the Hadamard product, particularly for rank.}{}{}
\fi
\smallskip

\iffalse 
\begin{proposition}
\label{prop:simplerankboundofHadamard}
(\rev{See, e.g., \cite{styan1973hadamard,horn1990hadamard}}.)
If $\done$ and $\dtwo$ are rank-$\rank$ matrices, then their Hadamard product $\done \odot \dtwo$ has rank at most $\rank^2$.
On the other hand, if $\inputmat$ is a rank-$\rank$ matrix, then $\inputmat$ can be represented as a Hadamard product of a rank-$\rank$ matrix and a rank-$1$ matrix. 
\end{proposition}
\smallskip

The first part follows immediately from Equation~\ref{eq:Dwrittenout}. 
The second part follows since any $\inputmat$ can be represented as a Hadamard product $\inputmat \odot {\mathbf 1}$, where ${\mathbf 1}$ is the identity matrix with respect to the Hadamard product, i.e., the matrix whose entries are all $1$.
\fi 


==> arXiv-2506.06456v1/problem_formulation_arxiv.tex <==
\section{Problem Formulation}\label{sec:prob}

% \cnote[MC]{ I am not very sure about using the words largest. Our algorithms are not guaranteed to return the largest low-rank submatrix (if in the initialization stage we do not hit it). }
Next, we formalize the problems we study in this paper. 
To provide better insight, we first present a special case,
and then introduce the more general problems.

%To facilitate a more intuitive understanding, we start by presenting an insightful special case. 
% Then, we introduce the problems of recovering near-rank-$1$ and near-rank-$\generalrank$ sub\-matrices, 
% near-rank-$\generalrank$ sub\-matrices. 
% and briefly discuss a generalization.
% a more general problems that encompasses the recovery of both rank-$1$ and rank-$\generalrank$ sub\-matrices. 
% \ref{ap:affine} presents an interesting problem variant 
% of the problems of recovering rank-$1$ and rank-$\generalrank$ sub\-matrices 
% that accounts for translations. 
%our formulation of the local low-rank approximation problem. %, as conceived in this work. 

\spara{Searching for a near-rank-$\mathbf{1}$ subset of rows or columns.}
As a warm-up, 
% Before introducing the problem of recovering near-rank-$1$ or near-rank-$k$ submatrices, it is insightful to 
we introduce a simpler problem that fixes the matrix columns or rows.
% and asks only for a subset of rows.
In other words, in this simplified scenario, we are not looking for 
 arbitrary sub\-matrices, but for sub\-matrices that  include all rows or all columns of the input matrix. 
% The problem is formalized as follows. 

\begin{problem}[Largest near-rank-$1$ subset of rows (\simplifiedproblem)]
\label{prob:simplified}
    Given a matrix \inputmat $\in \real^{\nrows \times \ncols}$  with set of rows \rowset and a threshold $\errorbound \in \real^+$, 
    find the largest subset of rows $\rowset' \subseteq \rowset$ such that there exist a 
    rank-$1$ matrix $\estimate{\outputmat} \propto \xvec \yvec^T$, where 
    $\yvec^T \in \real^\ncols$ is a row of \inputmat, 
    %and $\xvec \in \real^\nrows$, 
    %\propto \xvec \yvec^T $, where $\xvec \in \real^{|\rowset'|}$ and $\yvec \in \real^\ncols$ are respectively a subset of a column of \inputmat and a row of \inputmat, 
    satisfying
    \begin{equation}
    \label{equation:problem-rows-only}
        \|\inputmat_{i,:} - \estimate{\outputmat}_{i,:}\|_2 \leq \errorbound, \quad ~~\mbox{for all}~~ i \in \rowset'. 
    \end{equation}
    %\begin{equation}
    %    |\outputmat_{i,j} - %\estimate{\outputmat}_{i,j}| \leq \delta, \quad \forall i=1 \in \rowset, j=1, \dots \ncolssubmatrix. 
    %\end{equation}
\end{problem}

% \cnote[MC]{Aris, I have added acronym also for the special case problem, (LNROSR) in line with the others. Is there a reason to avoid doing so? Also the bound is now changed to $\epsilon$ for clarity, because $\delta$ is the input parameter on our method (bound on ratio for rank 1 / bound on absolute entry-wise rank-k approximation error for rank k) }

% \cnote[MC]{ I am not sure about ``largest'' --- since our methods do not necessarily find the largest submatrices in general, and we do not really focus on it. In other words, while we take the size of the submatrices into account, we do not necessarily discover the largest one with limited number of initializations. Thus maybe we can change the problem formulation to only ask for a submatrix or for all submatrices.  }

% \cnote[AG]{But in Problem \ref{prob:simplified} we are asking for \emph{maximum size subset}.\\
% Asking for \emph{any} submatrix sounds too easy: just return a $2\times 2$ submatrix. Is it good enough? \\
% Asking for \emph{all} submatrices is an enumeration problem and not really what we do, right? }

% \cnote[MC]{Yes. Agree; we just cannot claim that we solve this problem to optimality in general (which we are not doing, so we are fine). Also this make sense because intuitively we are looking for optimizing size and proximity to low-rank approximation.  }

\iffalse 
\cnote[Aris]{Is the problem here to find the maximum $|\rowset'|$ 
for which (\ref{equation:problem-rows-only}) holds?
To make the problem statement more clear, 
we can explicitly state the dimensions of vectors \xvec and \yvec, as $|\rowset'|$ and  \ncols, respectively, 
and the dimensions of $\estimate{\outputmat}$, as $|\rowset'|\times\ncols$.
Also, in this problem the error is defined entry-wise, 
while in the following problem statements we are using a more general norm.
I guess this is intentional, as this is a simpler problem.
Does the problem remain computationally solvable when the error is defined using a more general norm?}


\cnote[MC]{ The inequality was actually given in terms of euclidean (vector) norm.
I suggest to take out the $\propto  \xvec \yvec^T$ expression. My point is that either $\xvec$ or $\yvec$ in the outer product can be a row and column of \outputmat, as indicated by the analysis that does not rely on the \svd. In fact, this can be an advantage since the approximation holds also for a rank-1 matrix that is more intepretable than that given by the \svd. 
Although, of course, the \svd will have non-larger error at least for spectral and Frobenius norm by the Eckart-Young theorem. 
However, i believe maybe it is better to keep the problem general and explain this point elsewhere.} 
\fi 

Problem~\ref{prob:simplified} asks to find the largest near-rank-$1$ sub\-matrix
defined over a subset of rows of \inputmat and all columns.
% Problem~\ref{prob:simplified} aims specifically at finding a subset of rows. However, the formulation of the problem with respect to subsets of columns $\colset'$ is symmetric. 
% Intuitively, Problem~\ref{prob:simplified} and its column-based variant ask for a provably-accurate representation of a subset of rows (while  the columns are given in input) or of a subset of columns (while the rows are given in input) in terms of a single row and column of the input matrix. 
This problem % , which asks for the \emph{largest} subset or rows %or columns 
is computationally tractable. % , as stated next. 

% \cnote[AG]{ Which problem exactly is computationally tractable? Is it the problem of finding the \emph{largest} subset or rows?  }
% \cnote[MC]{ yes, rows or columns. The problem can be solved in polynomial time quite simply (as discussed in Appendix A). For the column, it suffices to do the same with the transpose of the input matrix. }

\begin{proposition}
The \simplifiedproblem 
problem can be solved in polynomial time.
\end{proposition}
The proof, via a simple algorithm, 
is presented in~\ref{app:specialcase}.

While Problem~\ref{prob:simplified} asks for a subset of rows, the symmetric problem asking for a subset of columns can be solved simply by considering~$\inputmat^T$ in place of $\inputmat$. 


\iffalse 
\begin{proposition}
Problem~\ref{prob:simplified}  can be solved in polynomial time.
\end{proposition}
\fi 

% While the \simplifiedproblem asks for a subset of rows, the symmetric problem asking for a subset of columns can be solved simply by considering  $\inputmat^T$ instead of $\inputmat$. 


%one can ask to find a sub\-matrix defined over all rows and a subset of columns, and an optimal solution to this symmetric problem can be found in polynomial time.

% In~\ref{app:specialcase}, we describe a simple algorithm to solve Problem~\ref{prob:simplified} to optimality. 

\spara{Searching for a near-rank-$\mathbf{1}$ sub\-matrix.}
%Problem~\ref{prob:rank-1} formalizes the problem of finding a near-rank-$1$ submatrix within an input matrix \inputmat. 
%The problem of identifying a near-rank-$1$ submatrix holds a central position in this work. 
Next, we discuss the more challenging problem of finding a near-rank-$1$ sub\-matrix,
without fixing neither the rows nor the columns of the input matrix. 
% This problem holds a central position in this work. 

\begin{problem}[Largest near-rank-$1$ sub\-matrix (\nearrankone)]
\label{prob:rank-1}
    Given a matrix \inputmat $\in \real^{\nrows \times \ncols}$, and a threshold $\errorbound \in \real^+$, 
    find a sub\-matrix \outputmat $\in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ of maximum size 
    such that there exist a rank-$1$ matrix $\estimate{\outputmat}$ %$ \propto \vecu \vecv^T $, 
    %where $\vecu$ and $\vecv$ are respectively a column and row of \outputmat,
    satisfying
    \begin{equation}
    \label{problem:near-rank-1-submatrix}
       \generalnormshort{\outputerror} =  \generalnormshort{\outputmat - \hat{\outputmat}} \leq \errorbound, ~
            \text{ where } * \text{ can be any of the norms } \{F, 2, \text{max} \}. 
    \end{equation}
\end{problem}

\iffalse
\cnote[Aris]{
What is the meaning of the phrase: 
``where $\vecu$ and $\vecv$ are respectively a column and row of \inputmat''? 
Can't they be any row and column of appropriate dimensions?
It would be good to discuss this distinction.
Also, if $\vecu$ and $\vecv$ are a column and a row of \inputmat
then $\estimate{\outputmat}$ is a ``full'' matrix, not a submatrix.
}
\cnote[MC]{
We will omit $\vecu$ and $\vecv$, which actually are such that either one of them is a row (\vecu) or a column ($\vecv$) of \outputmat.  See the note above with the details of this. 
}
\fi

% Problem~\ref{prob:rank-1} asks for a submatrix of the input matrix that can be closely approximated by the outer product of one of its rows and columns up to a multiplicative scalar. 

% The \nearrankone problem asks for sub\-matrices such that the Frobenius, spectral and max norm of the matrix of errors $\outputerror$ are bounded. 

% \cnote[HM]{Does this say that we want all three norms to be simultaneously small? Or do we select one we like and then require it to be small?}
% \cnote[AG]{I think that this is a concise way to write down three different problems, one for each norm. We should definitely clarify what we mean.}
%A key observation is that, as discussed in Section~\ref{sec:analysis}, bounds on the 
\iffalse
the bound on the infinity norm is \emph{stricter} than the spectral and Frobenius norms, 
requiring that the magnitude of each entry of the submatrix cannot deviate from its approximation by more than $\tol$. 
A bound on the infinity norm implies a bound on the Frobenius norm, which, in turn, implies a bound on the spectral norm. 
\fi 
Unfortunately, due to the interaction between rows and columns,
the \nearrankone problem is computationally intractable.

\begin{proposition}
\label{proposition:np-hardness}
The \nearrankone problem is \np-hard. 
\end{proposition}

The $\mathbf{NP}$-hardness of \nearrankone follows from that of the largest rank-$1$ sub\-matrix problem~\cite{doan2013finding}
by setting $\errorbound=0$, and 
%proof follows from an easy reduction from the \nphard largest rank-$1$ sub\-matrix problem~\cite{doan2013finding} 
%for $\errorbound=0$.
%The hardness of \nearrankone 
highlights the connection with the \emph{maximum-edge biclique} problem~\cite{lyu2020maximum}, 
which is made evident in Section~\ref{sec:algorithms}.

\iffalse
For the proof % of Proposition~\ref{proposition:np-hardness}, 
we observe that setting $\delta=0$
%our problem generalizes the 
results in the problem of 
finding the largest rank-$1$ sub\-matrix, which is known to be \nphard~\cite{doan2013finding}. 
%~\cite{doan2013finding,gillis2010using}.
%  and our problem reduces to the problem of finding rank-$1$ submatrices of maximum size for $\tol=0$. 
%Without delving into details, 
The hardness %arises from 
can be explained by the connection between the \nearrankone problem 
and the \emph{maximum-edge biclique} problem~\cite{lyu2020maximum}. 
This connection is made evident in Section~\ref{sec:algorithms}.
%In Section~\ref{sec:algorithms}, we discuss this connection between the 
%maximum-edge biclique problem and Problem~\ref{prob:rank-%1}.
\fi 

%%%% DO WE NEED THE AFFINE PROBLEM FORMULATION? 


%As discussed in Section~\ref{sec:algorithms}, the methods we introduce to tackle Problem~\ref{prob:rank-1} can be adapted with minor modification to solve Problem~\ref{prob:rank-1-affine} too. 

\spara{Searching for a near-rank-$\mathbf{k}$ submatrix.}
We generalize the \nearrankone problem to the case of near-rank-$k$ sub\-matrices. 

\begin{problem}[Largest near-rank-$k$ submatrix (\nearrankk)]
\label{prob:rank-k}
    Given a matrix \inputmat $\in \real^{\nrows \times \ncols}$, and a threshold $\errorbound \in \real^+$, 
    find a sub\-matrix \outputmat $\in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ of maximum size 
    such that there exist a rank-$k$ matrix $\estimate{\outputmat}$ 
    %with column space spanned by columns $\xvec_1, \dots \xvec_k$ of \outputmat and 
    %row space spanned by rows $\yvec_1, \dots \yvec_k$ of \outputmat, 
    satisfying
    \begin{equation}
        \generalnormshort{\outputmat - \hat{\outputmat}} \leq \errorbound, ~
         \text{ where } * \text{ can be any of the norms } \{F, 2, \text{max} \}. 
    \end{equation}
\end{problem}

%\cnote[Aris]{
%Same question as before, why restricting to rows and columns of the input matrix? \\
%And again, when taking full rows and columns of \inputmat, how come the result is a submatrix, 
%and not a full matrix?
%}
%\cnote[MC]{
%%Fixed. 
%}

As \nearrankk is a generalization of \nearrankone, the \nearrankk problem is also \nphard. 

%While we omit the details, we can also introduce an \emph{affine} extension of Problem~\ref{prob:rank-k}. % just like have introduced the affine extension of Problem~\ref{prob:rank-1} in Problem~\ref{prob:rank-1-affine}. 

%\cnote[MC]{ Do we need the affine rank-$k$ problem formulation as well ? }
%\cnote[Aris]{No.}

% \cnote[MC]{I removed the formal problem statement for "general local low-rank approximation", i do not think we need it and i would keep this very short (if not omit). But we can also put it back as a formal problem statement if you want. }

\spara{Extensions.}
The problem formulations presented above focus on extracting a single sub\-matrix. 
In practice, one may wish to find a representation of the input matrix
as a sum of $N$ local low-rank patterns.
Such a problem is a generalization of both \nearrankone and \nearrankk, and hence, 
inherits their hardness. 

Additionally, it may be of interest to identify sub\-matrices that define affine subspaces. 
Extending our problem formulations and method to the case of affine subspaces (or  
near-low-rank sub\-matrices up to a particular translation) is straightforward. 
The details are deferred to an extended version of this work.

%call for a thorough explanation and are left for an extended version of this work.
%Due to space limitations, 
%The details are left for an extended version of this work.

\iffalse
\spara{Iterated local low-rank approximation.}
The problem formulations illustrated above in this section focus on the extraction of a single submatrix. 
%In practice, one may be interested in representing a matrix as the sum of multiple local low-rank patterns. 
%In other words, we may be interested in finding a representation of the input matrix \inputmat as: 
In practice, one may wish to find a representation of an input matrix \inputmat as a sum of $N$ local low-rank patterns, i.e., as:
\[
 \estimate{\inputmat} = \sum_{h=1}^{N} \estimate{\outputmat}^*_h,
\]
where $\estimate{\outputmat}^*_h \in \real^{\nrows \times \ncols}$  is
%a matrix 
obtained from the solution $\outputmat$ to 
\nearrankone~or~\nearrankk by setting to $\estimate{\outputmat}_{i,j}$ the entries $(i,j)$ that are part of 
%the output sub\-matrix
$\outputmat$ and to $0$ all others. 
This problem is a generalization of \nearrankone~or~\nearrankk, and hence inherits their hardness. 

\cnote[MC]{ Do you think we should make this definition of $\hat{X}^*_h$ more formal by introducing the notation for the set of rows and the set of columns of the sub\-matrix $\rowset'$ and $\colset'$ ? }

\spara{Searching for a near-rank-$\mathbf{\generalrank}$ submatrices up to a translation.}
As specified in Section~\ref{sec:introduction}, from a geometrical standpoint, near-rank-$1$ sub\-matrices correspond to subsets of points closely aligned to a line through the origin (i.e., a $1$-dimensional subspace). 
Similarly, near-rank-$\generalrank$ sub\-matrices correspond to subsets of points and dimensions that lie close to $\generalrank$-dimensional subspaces. 
Lines and other subspaces that do not pass through the origin are referred to as \emph{affine} subspaces. 

In general, it may also be of interest to identify affine subspaces. 
Unfortunately, affine subspaces do not necessarily correspond to low-rank sub\-matrices, but they do after a suitable translation. 
Extending our problem formulations and method to the case of affine subspaces, and thus of near-low-rank  sub\-matrices up to a translation, is straightforward. The details are given in~\ref{ap:affine}. 
\fi



%Similarly, a near-rank-$\generalrank$ sub\-matrix corresponds to subsets of points and dimensions that lie close to a $\generalrank$-dimensional subspaces. 


\iffalse 
In general, it may also be of interest to identify dense lines of points that do not pass through the origin (i.e., affine $1$-dimensional subspaces).  
Similarly, near-rank-$\generalrank$ sub\-matrices corresponds to subsets of points and dimensions that lie close to $\generalrank$-dimensional subspaces, but one may also be interested in 

Points along a line not through the origin in general do not appear as (near) rank-$1$ sub\.matrices. However, they can be easily translated to yield a near-rank-$1$ sub\-matrix. 
%The case of near-rank-$1$ submatrices up to a translation is discussed in 
%Problem formulations and algorithms for the case of near-rank-$1$ submatrices up to a translation are straightforward extensions of the 
Similarly, a near-rank-$\generalrank$ sub\-matrix corresponds to subsets of points and dimensions that lie close to a $\generalrank$-dimensional subspaces. 
%For example, as for the points shown in Figure~\ref{fig:line_three_d}, a near-rank-$2$ submatrix in three columns identifies points that lie close to a plane through the origin in the three-dimensional space. 
Again, points close to a plane, or in general, close to a $\generalrank$-dimensional subspace not including the origin (i.e., $\generalrank$-dimensional affine subspaces) results in rank-$\generalrank$ sub\-matrices after a suitable translation.

Extending problem formulations and algorithms to the case of  near-rank-$1$ sub\-matrices up to a translation is straightforward. The details are given in Appendix~\ref{ap:affine}.
\fi 

%Again, we can also consider affine rank-$\generalrank$ subspaces that can be reduced to rank-$\generalrank$ submatrices after suitable re-centering. 
 


\iffalse 
We thus have the following problem. 

\begin{problem}[Provably-accurate local low-rank approximation]\label{prob:local_low_rank}
    Given input matrix \inputmat, and threshold $\tol \in \real$, find 
    a representation of the input matrix \inputmat as
    $\estimate{\inputmat}_I = \sum_h \estimate{\outputmat}_h$, 
    where each $\estimate{\outputmat}_h$ is a zero-padded low-rank approximation 
    of a submatrix $\outputmat_h$, (i.e., $\estimate{\outputmat}_h \in \real^{\nrows \times \ncols}$ with zero entries 
 for all indices that are not in $\outputmat_i$) and $I$ is the set of indices that are at least in one of the $\outputmat_i$,
    such that $I$ is as large as possible and it holds that
    \[
    \generalnormshort{ \estimate{\inputmat}_{I} - \inputmat_{I}   } \leq \delta ,  ~\mbox{with } * \in \{ F,2,\infty \},
    \]
    where $\estimate{\inputmat}_{I}$ and $ \inputmat_{I} $ have zero entries for all the indices not in $I$. 
\end{problem}



\cnote[Aris]
{
Why this problem is characterized as ``provably-accurate'' while the previous problems are not?
}
\cnote[MC]
{
To distinguish from the more general term "local low-rank approximation" also found in the literature without the same constraints that we impose. However, i am not sure about the names. We could have provably-accurate in the other problem names or in none. 
}

\cnote[Aris]
{
 ``zero-padded'' should be defined.
}
\cnote[MC]
{
Added explanation.
}

The goal in Problem~\ref{prob:local_low_rank} is to approximate as many matrix as possible using a set of low-rank local submatrix approximations. 
A budget-constrained variant of the problem would ask for a representation using at most \budget parameters. 



\cnote[MC]{I think we can remove this last problem. }
\fi 










\iffalse 
We start by describing the problem of locally approximating a given matrix \inputmat by rank-$1$ matrices. 



\spara{Searching for provably-accurate near-rank-$1$ submatrix.}

First, we consider the problem of finding a single optimal rank-$1$ matrix. 

\begin{problem}
\label{prob:rank-1}
    Given input a matrix \inputmat $\in \mathbb{R}^{\nrows \times \ncols}$, and a threshold $\errorbound \in \real$, find a submatrix \outputmat $\in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ of maximum size such that there exist a rank-$1$ matrix $\hat{\outputmat}$ satisfying: 
    \begin{equation}
        |\outputmat_{i,j} - \hat{\outputmat}_{i,j}| \leq \delta, \quad \forall i=1,\dots \nrowssubmatrix,j=1, \dots \ncolssubmatrix. 
    \end{equation}
\end{problem}


Intuitively, we are looking for subsets of a matrix such that rows and columns are approximately proportional. In geometrical terms, Problem~\ref{prob:rank-1} asks to identify $1$ dimensional subspaces, i.e., subsets of points and dimensions that lie approximately along a line through the origin. 

Unfortunately, Problem~\ref{prob:rank-1} is computationally difficult, as formalized next. 

\begin{proposition}
Problem~\ref{prob:rank-1} is NP-hard. 
\end{proposition}

To see why the problem is \nphard, it is enough to observe that the problem of finding a rank-$1$ submatrix is known to be \nphard (see~\cite{doan2013finding,gillis2010using}) and our problem reduces to the problem of finding rank-$1$ submatrices of maximum size for $\errorbound=0$. 

We can also prove the hardness of the problem by a reduction from the \emph{maximum-edge biclique problem}~\cite{lyu2020maximum}.
In Section~\ref{sec:algorithms}, we will discuss more in detail the equivalence between the maximum-edge biclique problem and Problem~\ref{prob:rank-1}.

The hardness of the problem stems from the non-trivial interactions between the rows and the columns of the input matrix. If either the rows or columns of the matrix are fixed, the resulting problem can be solved in polynomial time through a simple algorithm (specifically, in time $\mathcal{O}(m^2n + m(n \log n))$), which is detailed in Section~\ref{sec:algo_special_case}. 
For instance, assume that the columns of \outputmat are given. 
Then, we consider the submatrix with only the selected columns, and for each row, we can efficiently compute the projection errors of all the other rows onto it. 
Then, we can select the rows with projection error lower than \errorbound. 
After repeating this simple process for every row, we select the row that maximizes the number of rows with projection error lower than \errorbound. 



%\spara{Searching for a provably-accurate near-rank-$1$ submatrix up to a translation.}

As already mentioned, near-rank-$1$ submatrices correspond to $1$ dimensional subspaces, i.e. subsets of points distributed along a line through the origin in certain dimensions.
Many datasets exhibits subsets of points in certain dimensions distributed along a line that however  does not pass through the origin. 
As we are looking for local patterns in the input matrix, centering the data globally is not helpful to identify such a line. 

A line not passing through the origin corresponds to a $1$-dimensional affine subspace. 
A $1$-dimensional affine subspaces does not preserve the symmetry between rows and columns of proper $1$-dimensional subspaces, where both rows and columns are proportional to each other. 
However, affine subspaces can be transformed in proper subspaces by translation. 

In this work, we also address the problem of identifying $1$-dimensional affine subspaces. 


\spara{Searching for provably-accurate near-rank-$k$ submatrix.}
We can generalize Problem~\ref{prob:rank-1} to the case of near-rank-$k$ submatrices. 

\begin{problem}
\label{prob:rank-k}
    Given  input a matrix \inputmat $\in \mathbb{R}^{\nrows \times \ncols}$, and a threshold $\errorbound \in \real$, find a submatrix \outputmat $\in \real^{\nrowssubmatrix \times \ncolssubmatrix}$ of maximum size such that there exist a rank-$k$ matrix $\hat{\outputmat}$ satisfying: 
    \begin{equation}
        |\outputmat_{i,j} - \hat{\outputmat}_{i,j}| \leq \delta, \quad \forall i=1,\dots \nrowssubmatrix,j=1, \dots \ncolssubmatrix. 
    \end{equation}
\end{problem}

A near-rank-$k$ submatrix corresponds to subsets of points and dimensions that lie close to a $k$-dimensional subspaces. 
For example, a near-rank-$2$ submatrix in three columns identifies points that lie close to a plane in the three-dimensional space. 
Again, we can also consider affine rank-$k$ subspaces that can be reduced to rank-$k$ subspaces by recentering. 

\spara{Local low-rank approximation}

The long-standing \svd decomposes a matrix as the sum of rank-$1$ (global) matrices. 
To impose a local structure on the decomposition, methods such as as \emph{sparse PCA}~\cite{mairal2009online} have been developed .
If we can solve Problem~\ref{prob:rank-1}, however, we can develop a model that is not only sparse, this relaxing the assumption that the entire matrix is well-approximated by a rank-$1$ matrix, but also provably-accurate and interpretable. 
The goal is to only approximate subsets of matrices that are well approximated by low-rank structures, and leave others matrix subsets that are not well-described by low-rank structures unaltered.


\begin{problem}[local low-rank approximation]
    Given a total space budget $\budget$ and an input matrix \inputmat, find vectors $\mathbf{u}_i$ and $\mathbf{v}_i$, of total space smaller than \budget and such that $ \outputmatestimated = \sum_i \mathbf{u}_i \mathbf{v}_i^T $ is as large as possible and satisfy: 
    \[
    | \outputmatestimate - \inputmat | \leq \delta. 
    \]
\end{problem}


\fi 


==> arXiv-2506.06456v1/proofs.tex <==
\subsection{Proof of Lemma~\ref{lemma:errortosine}}
Given two vectors \(\yvec \in \mathbb{R}^\ncols \) and \(\xvec \in \mathbb{R}^\ncols \), the orthogonal projection of \(\yvec\) onto \(\xvec\) captures the component of \(\yvec\) that lies in the direction of \(\xvec\). To prove Lemma~\ref{lemma:errortosine}, we need to show that the $L_2$ norm of the difference between $\yvec$ and its projection onto $\xvec$ is equal to the $L_2$ norm of \(\yvec\) multiplied by the sine of the angle \(\theta\) between \(\yvec\) and \(\xvec\).

Recall that the projection of the vector \(\yvec\) onto the vector \(\xvec\) is given by:
\[
\proj{\xvec}{\yvec} = \frac{\yvec^T \xvec}{\xvec^T \xvec} \xvec = \frac{\yvec^T \xvec}{\|\xvec\|_2^2} \xvec.  
\]
%where \(\yvec^T \xvec\) is the dot product of \(\yvec\) and \(\xvec\), and \(\xvec^T \xvec = \|\xvec\|_2^2\) is the squared $L_2$ norm of \(\xvec\).

The projection error \errorvec associated with  $\proj{\xvec}{\yvec}$ is the vector given by the difference between \(\yvec\) and its projection onto \(\xvec\), i.e., 
\[
\errorvec = \yvec - \proj{\xvec}{\yvec}  = \yvec - \frac{\yvec^T \xvec}{\xvec^T \xvec} \xvec.
\]
%Substituting the expression for the orthogonal projection:
%\[
%\errorvec 
%\]
The $L_2$ norm of the projection error $\|\errorvec \|_2$ is thus
\(
\|\errorvec\|_2 = \left\| \yvec - \frac{\yvec^T \xvec}{\xvec^T \xvec} \xvec \right\|_2. 
\)
By definition, the dot product \(\yvec^T \xvec\) can be expressed in terms of the $L_2$ norm of \(\yvec\), the $L_2$ norm of \(\xvec\), and the cosine of the angle \(\theta\) between \(\yvec\) and \(\xvec\) as follows: 
\[
\yvec^T \xvec = \|\yvec\|_2 \|\xvec\|_2 \cos(\theta). 
\]
Using this equality, we can rewrite the definition of the the projection error \errorvec as:
\[
\boldsymbol{\epsilon} = \yvec - \frac{\|\yvec\|_2 \|\xvec\|_2 \cos(\theta)}{\|\xvec\|_2^2} \xvec
= \yvec - \frac{\|\yvec\|_2 \cos(\theta)}{\|\xvec\|_2 } \xvec. 
\]
Further, the squared $L_2$ norm of \(\boldsymbol{\epsilon}\) becomes
\(
 \left\| \yvec - \frac{\|\yvec\|_2 \cos(\theta)}{\|\xvec\|_2} \xvec \right\|_2^2. 
\)
Since the projection error is orthogonal to the projection~\cite{strang2022introduction}, the Pythagorean theorem yields:
\begin{equation}\label{eq:orthogonality_projection_error_vector}
\|\yvec\|_2^2 = \|\proj{\xvec}{\yvec}\|_2^2 + \|\boldsymbol{\epsilon}\|_2^2. 
\end{equation}


Because the $L_2$ norm is equivariant under scalar multiplication,  the  $L_2$ norm of the projection \(\|\proj{\xvec}{\yvec}\|_2\) is:
\[
\|\proj{\xvec}{\yvec}\|_2 = \frac{\|\yvec\|_2 \|\xvec\|_2 \cos(\theta)}{\|\xvec\|_2}
= \|\yvec\|_2 \cos(\theta). 
\]
Therefore, using Equation~\ref{eq:orthogonality_projection_error_vector}, the squared $L_2$ norm of the projection error can be written as: 
\[
\|\boldsymbol{\epsilon}\|_2^2 = \|\yvec\|_2^2 - \|\yvec\|_2^2 \cos^2(\theta)
= \|\yvec\|_2^2 (1 - \cos^2(\theta))
= \|\yvec\|_2^2 \sin^2(\theta),  
\]
where we have employed the trigonometric identity $1 - \cos^2(\theta) = \sin^2(\theta)$. 
%
Finally, upon taking the square root of both sides, we get:
\[
\|\boldsymbol{\epsilon}\|_2 = \|\yvec\|_2 \sin(\theta). 
\]
Thus, we have shown that, as claimed, given the orthogonal projection of \yvec onto \xvec, the $L_2$ norm of the projection error is equal to the $L_2$ norm of \(\yvec\) multiplied by the sine of the angle \(\theta\) between \(\yvec\) and \(\xvec\). 
%\cnote[MC]{We have an alternative proof for this result, commented out below - currently keeping this.}

%\[
%\|\boldsymbol{\epsilon}\| = \|\yvec\|_2 \sin(\theta). 
%\]



%\spara{Proof of %Lemma~\ref{lemma:initialization}.}

\subsection{Proof of Theorem~\ref{th:expansion}}
Before proceeding with the proof of Theorem~\ref{th:expansion}, it is useful to prove the following lemma, which refers to the initialization phase only. 


%this section, given next, which refers to the entire (expanded) output submatrices $\outputmat$. 
%-based notion of closeness to rank-$1$ for a $2 \times 2$ submatrices that is much simpler than that given by the \svd. 
%The lemma is interesting because, although it only refers to the initialization stage of our algorithm, it is helpful 
%\cnote[MC]{This lemma now give results simular to the thorem but only for the initialization stage}
\begin{lemma}\label{lemma:initialization}
Consider a $2 \times 2$-sub\-matrix \initialmat and 
let $\initialerror = \initialmat - \estimate{\initialmat}$, where $\estimate{\initialmat}$ is a rank-$1$ approximation of \initialmat.
If, as for the sub\-matrices expanded by \ourmethod,  $|\det(\initialmat)| \leq \toleranceinit$, 
\initialmat admits rank-$1$ approximations $\estimate{\initialmat}$ 
such that: 
\begin{equation}\label{eq:initialization_guarantee_infinity_2by2}
       \infinitynorm{ \initialerror } \leq  
       \frac{\toleranceinit 
\max_{i,j} |\inputmat_{i,j}| } { 2 \min_{i,j} \inputmat_{i,j}^2 }
%\frac{\toleranceinit}{2 \min_{i,j} |\initialmat_{i,j}|},
\end{equation}

and


\begin{equation}\label{eq:initialization_guarantee_frobenius_2by2}
       % \| \initialerror \| \leq \min( \frac{\toleranceinit}{\| \yvec \|} , \frac{\toleranceinit}{\| \xvec \|}) = \toleranceinit \frac{1}{\max(\| \yvec \| \| \xvec \|)}. 
       \spectralnorm{ \initialerror } \leq \frobeniusnorm{ \initialerror } \ \leq  \frac{ \toleranceinit }{\maxnorm}, 
\end{equation} 
where $\maxnorm$ denotes the maximum $L_2$ norm of a row or column of \initialmat. 

\iffalse
and 
\begin{equation}\label{eq:initialization_guarantee_spectral_2by2}
       % \| \initialerror \| \leq \min( \frac{\toleranceinit}{\| \yvec \|} , \frac{\toleranceinit}{\| \xvec \|}) = \toleranceinit \frac{1}{\max(\| \yvec \| \| \xvec \|)}. 
     %  \spectralnorm{ \initialerror } \leq \frac{ \frobeniusnorm{\initialmat}^2 - \sqrt{ \frobeniusnorm{\initialmat}^2 - 4 \toleranceinit^2}  }{2}
\spectralnorm{ \initialerror } \leq \sqrt{\frac{\frobeniusnorm{\initialmat}^2 - \sqrt{\frobeniusnorm{\initialmat}^2  - 4 \toleranceinit^2}}{2}}
\end{equation}
\fi 

\end{lemma}

Lemma~\ref{lemma:initialization} is interesting  not only because it provides a useful criterion to set the value of \toleranceinit, but it also formalizes the determinant-based notion of closeness to rank $1$ for $2 \times 2$ sub\-matrices on which \ourmethod builds. 
This notion is particularly simple; it only requires few basic operations, two products, a difference and possibly a change of sign, while knowledge of the (two) singular values is not required. 
%and much simpler than the notion of closeness to rank $1$ given by the \svd. 
Moreover,  Lemma~\ref{lemma:initialization} is helpful for understanding the main result presented in Section~\ref{sec:analysis}, and its proof, given later in this section. 


%it supports the definition of closeness to rank-$1$ for $2 \times 2$ sub\-matrices based on the determinant adopted in this work, which is much simpler than the definition of closeness to rank-$1$ given by the \svd. 

\iffalse 
The intuition behind the lemma is that if a $2 \times 2$ sub\-matrix has near-zero determinant, then it can be approximated by a rank-$1$ sub\-matrix with little  error. 
Hence, we can identify near-rank-$1$ $2 \times 2$ sub\-matrices even without knowledge of the singular values. 
As we prove later, a similar claim also holds for general $\nrowssubmatrix \times \ncolssubmatrix$ submatrices. 
\fi 


\begin{proof}
Consider a $2 \times 2$ sub\-matrix: 
\[
\initialmat = \begin{pmatrix}
x_1 & x_2 \\
y_1 & y_2
\end{pmatrix}. 
\]
We will start by proving the bound on the max norm of the $2 \times 2$ matrix $\initialerror$, then we prove the bound on the Frobenius and spectral norms. % and finally we prove the bound on the spectral norm. 

\spara{Bound on the max norm.}
In what follows, we let $\xvec=(x_1,x_2)$ and $\yvec=(y_1, y_2)$.    
%In the noise-free scenario, 
If \initialmat has exactly rank $1$, we have $x_1 y_2 = x_2 y_1$ which is equivalent to $\xvec = \alpha \yvec$ for some $\alpha$. In simple words, $\xvec$ and $\yvec$ are proportional. 
In the realistic case of data corrupted by noise, we are interested in near-rank-$1$ $2 \times 2$ sub\-matrices, which are such that $|x_1 y_2 - x_2 y_1| \leq \toleranceinit$ for some small $\toleranceinit$. 
If we approximate the rows of the matrix \initialmat as \xvec and $\alpha \xvec$ to obtain a rank-$1$ submatrix $\estimate{\initialmat}$, the only source of error is the approximation of \yvec as $\alpha \xvec$. 
Thus, 
define $\epsilon_1 = y_1 - \alpha x_1$ and similarly $\epsilon_2 = y_2 - \alpha x_2$. 
The vector $\errorvec = (\epsilon_1, \epsilon_2) $ is referred to as error vector. 

We can take $\alpha$ to be the scalar that defines the orthogonal projection of \yvec onto \xvec. 
It is known that, for any orthogonal projection of a vector $\yvec$ onto another $\xvec$, the  vector \( \errorvec = (\epsilon_1, \epsilon_2),  \) which we henceforth simply refer to as error vector, 
is orthogonal to $\xvec$. 
Therefore: 
\[
\errorvec^T \xvec = \epsilon_1 x_1 + \epsilon_2 x_2 = 0,
\]
from which we derive: 
\[ 
\epsilon_2 = - \frac{x_1}{x_2} \epsilon_1. 
\]
%
Furthermore, the condition we impose on the determinant means that: 
\[
| x_1 y_2 - x_2 y_1 | 
\leq \toleranceinit.
\]
Substituting the expression of $\yvec$ as a linear function of $\xvec$, we obtain: 
\[
 |x_1 (\alpha x_2 + \epsilon_2)  - x_2 (\alpha x_1 + \epsilon_1) |
\leq \toleranceinit, 
\]
from which: 
\[
| x_1 \epsilon_2  -  x_2 \epsilon_1 |
\leq \toleranceinit.
\]
Substituting $\epsilon_2 = - \frac{x_1}{x_2} \epsilon_1$ and collecting $\epsilon_1$, one gets: 
\[
\left| - \epsilon_1 \left(  \frac{x_1^2}{x_2} + x_2  \right)\right| 
    = \left|\epsilon_1 \left( \frac{x_1^2 + x_2^2}{x_2}\right)\right| \leq \toleranceinit.  
\]
Therefore, we conclude: 
\[ 
\abs{\epsilon_1} \leq \frac{\toleranceinit  |x_2| }{ x_1^2 + x_2^2 }. 
\]
As $|\epsilon_1| = \frac{|x_2|}{|x_1|} |\epsilon_2|$, we also have: 
\[
\abs{\epsilon_2} \ \leq \frac{\toleranceinit  |x_1| }{ x_1^2 + x_2^2 }.
\] 
Equation~\ref{eq:initialization_guarantee_infinity_2by2} follows by observing that we have no made any assumptions on $x_1, x_2, y_1$ and $y_2$, and every entry must thus be bounded by \(  \frac{\toleranceinit 
\max_{i,j} |\inputmat_{i,j}| } { 2 \min_{i,j} \inputmat_{i,j}^2 }  \). 


%the same bound holds for any four entries as long as the condition on the row-wise and column-wise ratios imposed by our algorithm is satisfied. 
%To prove a bound on the infinity norm, we consider the rank-$1$ approximation of \inputmat given by the 
%The proof of the bound on the max norm follows by the upper bound on the absolute value of the determinant and the orthogonality between the vector of projection errors $\errorvec$ and $\xvec$
%is a direct consequence of the bound imposed on the ratio and the orthogonality of the residuals of the orthogonal projection of a vector $\yvec$ onto another vector $\xvec$.  
\iffalse
In particular, assume that $\xvec$ is the anchor row (or column) used in computing the ratios. 
For every pair of entries $(y_1, y_2)$ of another row (column) $\yvec$, we consider the approximations $y_1 = \alpha x_1$ and $y_2 = \alpha x_2$ where $\alpha$ is the orthogonal projection scalar for the projection of $\yvec$ onto $\xvec$. 


Therefore: 
\[
\epsilon_1 x_1 + \epsilon_2 x_2 = 0,
\]
i.e., 
\[ 
\epsilon_2 = - \frac{x_2}{x_1} \epsilon_1. 
\]
The condition we impose on the ratios of the rows and columns implies that: 
\[
| \frac{y_1}{x_1} - \frac{y_2}{x_2} | 
= 
| \frac{y_1x_2 -x_1 y_2}{x_1 x_2}| = 
 \frac{|y_1x_2 -x_1 y_2|}{|x_1| |x_2|} 
\leq \delta.
\]
Substituting the expression of $\yvec$ as a linear function of $\xvec$: 
\[
 \frac{|(\alpha x_1 + \epsilon_1) x_2 -x_1 (\alpha x_2 + \epsilon_2) |}{|x_1| |x_2|} 
\leq \delta.
\]
Simplifying: 
\[
 \frac{| \epsilon_1 x_2 - \epsilon_2 x_1 |}{|x_1| |x_2|} 
\leq \delta \iff | \epsilon_1 x_2 - \epsilon_2 x_1 |
\leq \delta |x_1| |x_2|.
\]
Substituting $\epsilon_2 = - \frac{x_2}{x_1} \epsilon_1$ and collecting $\epsilon_2$, one gets: 
\[
| \epsilon_2 (x_2 + x_2) | \leq \delta |x_1| |x_2|,
\]
from which we conclude: 
\[
\abs{\epsilon_2} \leq \frac{\delta}{2 |x_2|}. 
\]
As $\epsilon_1 = \frac{|x_2|}{|x_1|} |\epsilon_2|$, we also have: 
\[
\abs{\epsilon_1} \ \leq \frac{\delta}{2 |x_1|}.
\]
Equation~\ref{eq:initialization_guarantee_infinity} follows by observing that we have no made any assumptions on $x_1, x_2, y_1$ and $y_2$ and the same bound holds for any four entries as long as the condition on the row-wise and column-wise ratios imposed by our algorithm is satisfied. 
\fi 


\spara{Bounds on the Frobenius and spectral norms.}
To prove the bound on the Frobenius norm given in Equation~\ref{eq:initialization_guarantee_frobenius_2by2}, we again show that the bound holds for the rank-$1$  approximation $\estimate{\initialmat}$ obtained by stacking the rows $\xvec = (x_1, x_2)$ and $\yvec = \alpha \xvec$, where $\alpha$ is the orthogonal-projection scalar, i.e., $\alpha =\frac{\xvec^T \yvec}{\| \xvec \|^2_2}$.
Because \xvec can be approximated with \xvec itself, the $L_2$ norm of the projection error equals the Frobenius norm of the difference between $\initialmat$ and its rank-$1$ estimate $\estimate{\initialmat}$, i.e., $\| \boldsymbol{\epsilon} \|_2 = \| \initialmat - \estimate{\initialmat} \|_F = \| \initialerror \|_F $. 

Let $\theta$ be the angle between the two vectors $\xvec$ and $\yvec$. 
\iffalse 
Then, we have: $\| \mathbf{\epsilon} \|^2 = \epsilon_1^2 + \epsilon_2^2 = (c - \alpha a)^2 + (d - \alpha b)^2 = c^2 + \alpha^2 a^2 - c \alpha a + d^2 + \alpha^2 b^2 - \alpha d b = \| y \|^2 - \frac{\xvec^T \yvec}{\| \xvec \|_2^2} = \| y \|^2 sin^2(\theta)$.
\fi 
As stated in Lemma~\ref{lemma:errortosine}, we have that 
$\| \errorvec \|_2 =  \| \yvec \|_2 \sin(\theta)$.

Next, we show that we additionally have the identity: 
\begin{equation}
\label{eq:determinant_to_sine}
    |x_1 y_2 - x_2 y_1| = \| \xvec \|_2 \| \yvec \|_2 sin(\theta). 
\end{equation}
The $L_2$ norms of \( \mathbf{x} \) and \( \mathbf{y} \) are:
\begin{equation*}
\| \mathbf{x} \|_2 = \sqrt{x_1^2 + x_2^2} \text{ and } \| \mathbf{y} \|_2 = \sqrt{y_1^2 + y_2^2},
\end{equation*}
and the cosine of the angle \( \theta \) between the vectors $\xvec$ and $\yvec$ is given by:
\begin{equation*}
\cos(\theta) = \frac{x_1 y_1 + x_2 y_2}{\| \mathbf{x} \|_2 \| \mathbf{y} \|_2 }.
\end{equation*}
Using the identity \( \sin^2(\theta) + \cos^2(\theta) = 1 \), we get: 
\begin{equation*}
\sin^2(\theta) = 1 - \cos^2(\theta) =  1 - \left( \frac{x_1 y_1 + x_2 y_2}{\| \mathbf{x} \|_2 \| \mathbf{y} \|_2 } \right)^2,
\end{equation*}
%
that is: 
\begin{equation*}
\sin^2(\theta) = \frac{(x_1^2 + x_2^2)(y_1^2 + y_2^2) - (x_1 y_1 + x_2 y_2)^2}{(x_1^2 + x_2^2)(y_1^2 + y_2^2)}.
\end{equation*}
Expanding and simplifying, one obtains: 
\begin{equation*}
    \sin^2(\theta) = \frac{(x_1 y_2 - x_2 y_1)^2}{(x_1^2 + x_2^2)(y_1^2 + y_2^2)},
\end{equation*}
from which: 
\[
 \sin^2(\theta) \| \xvec \|_2^2 \| \yvec \|_2^2 = (x_1 y_2 - x_2 y_1)^2, 
\]
and thus Equation~\ref{eq:determinant_to_sine} follows by taking the square root of both sides. 
%Since
%\[
%|x_1 y_2 - x_2 y_1| = \| \mathbf{x} \| \| \mathbf{y} \| %|\sin(\theta)|. 
%\]
As $|x_1 y_2 - x_2 y_1| = \| \xvec \|_2 \| \yvec \|_2  \sin(\theta) $, the condition $|\det(\initialmat)| = |x_1 y_2 - x_2 y_1| \leq \toleranceinit$ implies: 
\[
\| \xvec \|_2 \| \yvec \|_2  \sin(\theta) \leq \toleranceinit,
\]
which holds if and only if:
\begin{equation*}
    \sin(\theta) \leq \frac{\toleranceinit}{\| \xvec \|_2 \|\yvec \|_2}. 
\end{equation*}
Further, since $\| \boldsymbol{\epsilon} \|_2 = \|\yvec\|_2 \sin(\theta)$, we conclude: 
\begin{equation*}\label{eq:forx}
    \| \boldsymbol{\epsilon} \|_2 =  \| \initialerror \|_F  \leq \frac{\toleranceinit}{\| \xvec \|_2}. 
\end{equation*}
We can swap the roles of \xvec and \yvec without changing the absolute value of the determinant, which leads to: 
\begin{equation}\label{eq:fory}
     \| \boldsymbol{\epsilon} \|_2  = \| \initialerror \|_F  \leq \frac{\toleranceinit}{\| \yvec \|_2}. 
\end{equation}
Similarly, %we can repeat the same argument given above considering the columns of \initialmat instead of the rows, and the lemma follows. 
swapping the columns does not change the absolute value of the determinant, which concludes the proof of the bound on the Frobenius norm. 
Finally, the spectral norm is always upper bounded by the Frobenius norm, and hence the lemma follows. 


%\cnote[MC]{Question to double check: does the fact that this inequality above holds for *all* choices of row / column \yvec mean that we should put the maximum in the denominator of the reported bound in the lemma?}


%\cnote[MC]{I did double check this proof for the spectral norm, but a further check on the last part of it would be useful. }


%\cnote[MC]{P.S. I think we can also move to the bounds on the spectral norm in the appendix. }





\iffalse 
Because $ \sqrt{(\|\xvec\|_2^ + \|\yvec\|_2^2)^2 - 4 (\|\xvec\|_2^ \|\yvec\|_2^2 - (\xvec \cdot \yvec)^2)} \geq 0$, it follows that: 
\[
\lambda_2 \leq \frac{\|\xvec\|_2^2 + \|\yvec\|_2^2}{2}.
\]
In order for this bound to hold for any choice of $\xvec$ and $\yvec$, we need: 
\[
\lambda_2 \leq \frac{2\gamma_{max}^2}{2} \leq \gamma_{max}^2.
\]
In view of the relationship between the eigenvalues of $\textbf{G}_{\initialmat}$ and the singular values of $\initialmat$, we conclude that: 
\[
\spectralnorm{\initialerror} \leq \gamma_{max}. 
\]
\fi 

%The numerator in this upper bound, $\|\xvec\|_2^2 + \|\yvec\|_2^2$ equals the square of the Frobenius norm of $\initialmat$. 
%i



\iffalse 
Let \( P \) be a \( 2 \times 2 \) matrix with row vectors:

\[
x = (x_1, x_2), \quad y = (y_1, y_2)
\]

so that:

\[
P = \begin{bmatrix} x_1 & x_2 \\ y_1 & y_2 \end{bmatrix}
\]

The **Gram matrix** is:

\[
P P^T = \begin{bmatrix} x_1 & x_2 \\ y_1 & y_2 \end{bmatrix}
\begin{bmatrix} x_1 & y_1 \\ x_2 & y_2 \end{bmatrix}
\]

Computing the product:

\[
P P^T = \begin{bmatrix}
\|x\|^2 & x \cdot y \\
x \cdot y & \|y\|^2
\end{bmatrix}
\]

where:
- \( \|x\|^2 = x_1^2 + x_2^2 \) (squared norm of the first row),
- \( \|y\|^2 = y_1^2 + y_2^2 \) (squared norm of the second row),
- \( x \cdot y = x_1 y_1 + x_2 y_2 \) (dot product of the two rows).

The **eigenvalues** \( \lambda_1, \lambda_2 \) satisfy:

\[
\det(P P^T - \lambda I) = 0
\]

Substituting \( P P^T \):

\[
\begin{vmatrix}
\|x\|^2 - \lambda & x \cdot y \\
x \cdot y & \|y\|^2 - \lambda
\end{vmatrix} = 0
\]

Expanding the determinant:

\[
(\|x\|^2 - \lambda)(\|y\|^2 - \lambda) - (x \cdot y)^2 = 0
\]

\[
\lambda^2 - (\|x\|^2 + \|y\|^2) \lambda + (\|x\|^2 \|y\|^2 - (x \cdot y)^2) = 0
\]

Thus, the **exact eigenvalues** are given by solving this quadratic equation:

\[
\lambda_{1,2} = \frac{(\|x\|^2 + \|y\|^2) \pm \sqrt{(\|x\|^2 + \|y\|^2)^2 - 4 (\|x\|^2 \|y\|^2 - (x \cdot y)^2)}}{2}
\]

Since \( P P^T \) is symmetric and positive semi-definite, we have:

\[
\lambda_1 \geq \lambda_2 \geq 0
\]
\fi 



%Finally, the lemma follows by merging Equations~\ref{eq:forx}~and~\ref{eq:fory}. 
\end{proof}

%\spara{Proof of %Theorem~\ref{theorem:expansion}.}
We are now in a position to prove Theorem~\ref{th:expansion}, which describes the approximation-error guarantees associated with Algorithm~\ref{alg:rankone} in terms of max, Frobenius and spectral norm. 
To prove the theorem, we extend the proof of Lemma~\ref{lemma:initialization} from the initialization to the expansion phase. 



\iffalse 
to extend the proof of Lemma~\ref{lemma:initialization} from the initialization to the expansion stage, and hence to prove 
\fi 
 

\begin{proof}
%We prove the bounds on the different norms separately, although some ideas are useful in deriving the bound for more than one norm. 
Like for the proof of Lemma~\ref{lemma:initialization}, we prove bounds separately for the max norm and Frobenius and spectral norms.  
For simplicity, we present the proof for the row-wise ratios, and we denote by \xvec the anchor row, while \yvec denotes any other row of \outputmat. 
The proofs for the column-wise ratios are always symmetric. 

\spara{Bound on the max norm.}
The proof of the bound on the max norm (Equation~\ref{eq:initialization_guarantee_infinity}) is straightforward, as it is a simple extension of the proof of the bound on the max norm given in Lemma~\ref{lemma:initialization} for the case of $2 \times 2$ sub\-matrices.    

%as it is a direct consequence of the bound imposed on the ratio and the orthogonality of the residuals of the orthogonal projection of a vector $\yvec$ onto another vector $\xvec$.  
%For convenience, throughout the proof of the theorem, we illustrate the arguments for the case of rows. 
%However, the argument for the columns is symmetric. 

%In particular, assume that $\anchorrow$ is the anchor row (or column) used in computing the ratios. 
Given the anchor row \anchorrow, 
for every pair of entries $(y_1, y_2)$ of another row  $\yvec$, we consider the approximations $y_1 = \alpha x^r_1$ and $y_2 = \alpha x^r_2$ where $\alpha$ is the orthogonal-projection scalar for the projection of $\yvec$ onto $\anchorrow$. 

%It is known that the vector of orthogonal projection residuals
The well-developed theory of orthogonal projections guarantees that the error vector 
\( \errorvec = (\epsilon_1, \epsilon_2) \)
is orthogonal to $\anchorrow$~\cite{strang2022introduction}. 
Therefore, we have: 
\[
\epsilon_1 x^r_1 + \epsilon_2 x^r_2 = 0,
\]
i.e., 
\[ 
\epsilon_2 = - \frac{x^r_1}{x^r_2} \epsilon_1. 
\]
The condition \ourmethod imposes on the ratio matrices 
%s of the rows and columns 
implies that: 
\[
| \frac{y_1}{x^r_1} - \frac{y_2}{x^r_2} | 
= 
| \frac{y_1x^r_2 -x^r_1 y_2}{x^r_1 x^r_2}| = 
 \frac{|y_1 x^r_2 - x^r_1 y_2|}{|x^r_1| |x^r_2|} 
\leq \delta.
\]
Substituting the expression of $\yvec$ as a linear function of $\xvec$: 
\[
 \frac{|(\alpha x^r_1 + \epsilon_1) x^r_2 -x^r_1 (\alpha x^r_2 + \epsilon_2) |}{|x^r_1| |x^r_2|} 
\leq \delta.
\]
Simplifying: 
\[
 \frac{| \epsilon_1 x^r_2 - \epsilon_2 x^r_1 |}{|x^r_1| |x^r_2|} 
\leq \delta \iff | \epsilon_1 x^r_2 - \epsilon_2 x^r_1 |
\leq \tol |x^r_1| |x^r_2|.
\]
Substituting $\epsilon_2 = - \frac{x^r_1}{x^r_2} \epsilon_1$ and collecting $\epsilon_1$, one gets: 
\[
\left| \epsilon_1 \left( \frac{ {x_2^r}^2 + {x_1^r}^2 }{ x_2^r } \right) \right| \leq  \tol |x^r_1| |x^r_2|,
\]
%\[
%| \epsilon_2 (x^r_2 + x^r_2) | %\leq \delta |x^r_1| |x^r_2|,
%\]
from which we conclude: 
\[
\abs{\epsilon_1} \leq \frac{\tol |x^r_1| {x^r_2}^2 }{ {x_1^r}^2 + {x_2^r}^2  }. 
\]
As $ |\epsilon_1| = \frac{|x^r_2|}{|x^r_1|} |\epsilon_2|$, we also have: 
\[
\abs{\epsilon_2} \ \leq \frac{\tol {x^r_1}^2 |x^r_2| }{{x_1^r}^2 + {x_2^r}^2 }. 
\]
%Equation~\ref{eq:initialization_guarantee_infinity} follows by observing that 
We have no made any assumptions on $x^r_1, x^r_2, y_1$ and $y_2$. Therefore, the bound:
\[
\frac{\tol \max_{i} |x_i^r|^3 }{2 \min_{i} {x^r_i}^2 }
\]
necessarily hold for any entry in \inputmat. 
Furthermore, a symmetric bound can be obtained by considering the column-wise ratios instead of the row-wise ones, and then
Equation~\ref{eq:initialization_guarantee_infinity} follows. 


%the same bound holds for any four entries as long as the condition on the row-wise and column-wise ratios imposed by our algorithm is satisfied. 

\spara{Bounds on the Frobenius and spectral norms.}
To prove the theorem, we extend the proof of Equation~\ref{eq:initialization_guarantee_frobenius_2by2} in Lemma~\ref{lemma:initialization} to the general case of $\nrowssubmatrix \times \ncolssubmatrix$ sub\-matrices.  
First notice that, given the orthogonal projection of a row \yvec onto \anchorrow, as in the case of Lemma~\ref{lemma:errortosine}, which does not make any assumption on the dimensions of the vectors under consideration, for the norm of the (now $\ncolssubmatrix$-dimensional) error vector, it holds that $\|\boldsymbol{\epsilon}\|_2^2 = \| \yvec \|_2^2 \sin^2 (\theta)$.
\iffalse 
as shown next. 
In this case, we are given two \( k \)-dimensional vectors:
\[
\xvec = (x_1, x_2, \dots, x_k), \quad \yvec = (y_1, y_2, \dots, y_k).
\]
We further define the projection scalar of \( \yvec \) onto \( \xvec \) as:
\begin{equation*}
    \alpha = \frac{ \mathbf{x}^T \yvec }{\| \xvec \|_2^2}.
\end{equation*}
Then, we define the components of the error vector \( \boldsymbol{\epsilon} \) as:
\[
\epsilon_i = y_i - \alpha x_i, \quad \text{for } i = 1,2,\dots,k.
\]
Expanding the squares,  we get: 
\[
\|\boldsymbol{\epsilon}\|_2^2 = \sum_{i=1}^{k} (y_i - \alpha x_i)^2 = \sum_{i=1}^{k} y_i^2 - 2\alpha \sum_{i=1}^{k} y_i x_i + \alpha^2 \sum_{i=1}^{k} x_i^2,
\]
which can be re-written more concisely as: 
\[
\|\boldsymbol{\epsilon}\|_2^2 = \| \yvec \|_2^2 - 2\alpha \xvec^T \yvec + \alpha^2 \|\xvec\|_2^2.
\]
Substituting for \( \alpha \), one obtains:
\[
\|\boldsymbol{\epsilon}\|_2^2 = \|\yvec\|_2^2 - 2 \frac{(\xvec^T \yvec)^2}{\| \xvec \|_2^2} + \frac{( \xvec^T \yvec )^2}{\| \xvec \|_2^2} = \| \yvec \|_2^2 - \frac{(\xvec^T \yvec)^2}{\| \xvec \|_2^2}.
\]
By definition of the cosine of the angle $\theta$ between \( \xvec \) and \( \yvec \):
\[
\cos^2(\theta) = \frac{(\xvec^T \yvec )^2}{\| \xvec \|^2 \|\yvec \|^2}.
\]
Combining the previous two equations:
\[
\|\boldsymbol{\epsilon}\|_2^2 = \| \yvec \|_2^2  (1 - \cos^2(\theta)).
\]
Since \( 1 - \cos^2(\theta) = \sin^2(\theta) \), we conclude:
\begin{equation*}
\|\boldsymbol{\epsilon}\|^2 = \|\mathbf{y}\|^2 \sin^2(\theta), 
\end{equation*}
which proves that also in the case of $k$-dimensional vectors, we have the same equality for the norm of the error vector as in the simple two-dimensional case. 
\fi 

%In expanding $2$-dimensional vectors to $k$-dimensional vectors, we could have simply computed determinant of $2 \times 2$ contiguous submatrices. 
%However, 
In the expansion stage, we seek submatrices such that the $2 \times 2$-determinants within it are near zero. Instead of computing determinants, however, we compute ratios, which is more convenient. 
%As already seen in the proof of Equation~\ref{eq:initialization_guarantee_infinity}, the ratios that are computed in the expansion stage of our method are directly related to the determinants of the $2\times2$-submatrices contained in the $2 \times \ncolssubmatrix$ expanded sub\-matrix. 
As already pointed out, 
the ratios that are computed in the expansion phase of our method are directly related to the determinants of the $2\times2$-sub\-matrices.
In particular, considering again row \anchorrow as the anchor row we divide by and another row $\yvec$, we require the following inequality on the ratios: 
\[
\left| \frac{y_i}{x^r_i} - \frac{y_j}{x^r_j} \right| \leq \tol \quad \text{for all } i \text{ and } j, 
\]
which implies: 
\[
| y_i x^r_j  - y_j x^r_i | \leq | x^r_i | | x^r_j | \tol \quad \text{for all } i \text{ and } j. 
\]
Thus, the bound on the absolute difference of ratios guarantees that the associated $2 \times 2$-sub\-matrix determinant is bounded by \tol, rescaled by the absolute values of the entries $x^r_i$ and $x^r_j$ of the anchor row. 

Keeping in mind the relationship between ratios and $2\times2$ determinants, we continue the proof by finding a bound on the
the norm of the error vector $\| \boldsymbol{\epsilon} \|_2^2 = \|\mathbf{y}\|_2^2 \sin^2(\theta)$ obtained by projecting \yvec onto \anchorrow.
%as before, we need to bound  $\sin^2\theta$. 
In particular, to find a bound for  $\| \boldsymbol{\epsilon} \|_2^2$, we need to bound $\sin^2(\theta)$. 
First, notice that: 
\[
\sin^2(\theta) = 1 - \cos^2(\theta )= 1 - \frac{({\anchorrow}^T \yvec)^2}{ \| \anchorrow \|_2^2 \| \yvec \|_2^2 } = \frac{\| \xvec \|_2^2 \| \yvec \|_2^2  - ({\anchorrow}^T \yvec)^2}{ \| \anchorrow \|_2^2 \| \yvec \|_2^2 }. 
\]
%
Let us focus on the numerator, $\| \anchorrow \|_2^2 \| \yvec \|_2^2  - ({\anchorrow}^T \yvec)^2$. 
For simplicity, in what follows, we use the notation $\sum_{i \neq j}$ to denote the sum over pairs $(i,j)$ from $1$ to $\ncolssubmatrix$ such that $i\neq j$, and, similarly, the notation $\sum_{i < j}$ to indicate the sum over pairs $(i,j)$ from $1$ to $\ncolssubmatrix$  such that $i$ is lower than $j$. 
Expanding the product of the squared $L_2$ norms, one obtains: 
%
\[
\|\anchorrow\|_2^2 \|\yvec\|_2^2 = \left( \sum_{i=1}^{\ncolssubmatrix} {x^r_i}^2 \right) \left( \sum_{j=1}^{\ncolssubmatrix} y_j^2 \right) = \sum_{i=1}^{\ncolssubmatrix} {x^r_i}^2 y_i^2 + \sum_{i \neq j} {x^r_i}^2 y_j^2.
\]
%
Similarly, expanding the squared dot product, we get:
%
\[
({\anchorrow}^T \yvec)^2 = \sum_{i=1}^{\ncolssubmatrix} {x^r_i}^2 y_i^2 + 2 \sum_{i < j} x^r_i y_i x^r_j y_j.
\]
Thus:
\[
\|\anchorrow\|_2^2 \|\yvec\|_2^2 - ({\anchorrow}^T \yvec)^2 = \sum_{i=1}^{\ncolssubmatrix} \anchorrowentryis^2 y_i^2 + \sum_{i \neq j} \anchorrowentryis^2 y_j^2 - \left( \sum_{i=1}^{\ncolssubmatrix} \anchorrowentryis^2 y_i^2 + 2 \sum_{i < j} \anchorrowentryi y_i \anchorrowentryj y_j \right).
\]
%
Canceling out the  terms \( \sum_{i=1}^{\ncolssubmatrix} {x^r_i}^2 y_i^2 \), we are left with:
\[
\sum_{i \neq j} \anchorrowentryis^2 y_j^2 - 2 \sum_{i < j} \anchorrowentryi y_i \anchorrowentryj y_j,
\]
%
%and re-writing the first summation exploiting symmetry:
By symmetry, the term $\sum_{i \neq j} \anchorrowentryis^2 y_j^2 $ can be re\-written as $\sum_{i < j} (\anchorrowentryis^2 y_j^2 + \anchorrowentryjs^2 y_i^2)$, and hence: 
\begin{align*}
    \sum_{i \neq j} \anchorrowentryis^2 y_j^2 - 2 \sum_{i < j} \anchorrowentryi y_i \anchorrowentryj y_j =&\\ \sum_{i < j} (\anchorrowentryis^2 y_j^2 + \anchorrowentryjs^2 y_i^2) - 2 \sum_{i < j} \anchorrowentryi y_i \anchorrowentryj y_j = \sum_{i < j} ( \anchorrowentryis^2 y_j^2 + \anchorrowentryjs^2 y_i^2 - 2 \anchorrowentryi y_i \anchorrowentryj y_j).
\end{align*}
%
%
The expression above corresponds to a sum of squared differences. Specifically, it is equivalent to: 
%
\[
\sum_{i < j} (y_i \anchorrowentryj - y_j \anchorrowentryi)^2.
\]
%
Thus, we have shown that:
%
\[
\|\anchorrow\|_2^2 \|\yvec\|_2^2 - ({\anchorrow}^T \yvec)^2 = \sum_{i < j} (y_i \anchorrowentryj - y_j \anchorrowentryi )^2.
\]
%
As explained above, the condition we impose on the ratios leads to $ | y_i \anchorrowentryj - y_j \anchorrowentryi   | \leq |\anchorrowentryi| |\anchorrowentryj| \tol $, or, equivalently $  (y_i \anchorrowentryj - y_j \anchorrowentryi  )^2 \leq {\anchorrowentryi}^2 {\anchorrowentryj}^2 \tol^2 $. 
%
Therefore: 
%
\[
\sin^2 (\theta) = \frac{\|\anchorrow\|_2^2 \|\yvec\|_2^2 - ( {\anchorrow}^T \yvec)^2}{\|\anchorrow\|_2^2 \|\yvec\|_2^2} = \frac{ \sum_{i < j} (\anchorrowentryi y_j - \anchorrowentryj y_i)^2 } {\|\anchorrow\|_2^2 \|\yvec\|_2^2} \leq  \frac{ \tol^2 \sum_{i < j} {\anchorrowentryi}^2 {\anchorrowentryj}^2 }{\|\anchorrow\|_2^2 \|\yvec\|_2^2}.
\]
Finally, recalling that $\| \boldsymbol{\epsilon} \|_2^2 = \| \yvec \|_2^2 \sin^2 (\theta)$, we have: 
\begin{equation}\label{eq:guarantee_k}
\| \boldsymbol{\epsilon} \|_2^2 \leq \frac{ \tol^2 \sum_{i < j} {\anchorrowentryi}^2 {\anchorrowentryj}^2 }{\|\anchorrow\|_2^2}. 
\end{equation}

Equation~\ref{eq:guarantee_k} applies to every non-anchor row $\yvec$ of \outputmat.  
As usual, 
the same derivations also hold for the columns of \outputmat. 
Hence, the bound on the Frobenius stated in the theorem follows, and the spectral norm is always bounded by the Frobenius norm. 
This concludes the proof of the theorem. 
\end{proof}


%\cnote[MC]{Perhaps the notation with double superscript r and 2 or r and T is a bit ugly? Should we change the notations \anchorrow and \anchorcolumn to something else ? Or we say that \xvec denotes the anchor row in the proof, which is what we initially had. }





























\subsection{Proof of Theorem~\ref{th:expansion_appendix}}
To conclude this section, we present the proof of Theorem~\ref{th:expansion_appendix} which bounds the low-rank-approximation error incurred by the rank-$1$ \svd for the sub\-matrices detected by \ourmethod. 

%To conclude the proof of the lemma, we prove the bound on the spectral norm specified in Equation~\ref{eq:initialization_guarantee_spectral_2by2}. 
%In this case, as the spectral norm is numerically equal to the largest singular value, it is convenient to prove the result based on the approximation given by the rank-$1$ \svd. 

\begin{proof}
To prove the bound on the spectral norm of the matrix of differences \outputerror obtained by approximating a near-rank-$1$ sub\-matrix discovered by \ourmethod through its rank-$1$ \svd,
%it is left to prove the bound on the spectral norm of the error matrix. 
we again consider the rows of \outputmat and we re\-use the bound on the sine of the angle $\theta$ between a row \yvec and the anchor row \anchorrow obtained in the proof of Theorem~\ref{th:expansion}. 
Specifically, while proving the bound on the Frobenius and spectral norms in Equation~\ref{eq:expansion_guarantee}, we have shown that: 
\[
\sin^2(\theta) \leq \frac{\|\anchorrow\|_2^2 \|\yvec\|_2^2 - ({\anchorrow}^T \yvec)^2}{\|\anchorrow\|_2^2 \|\yvec\|_2^2} = \frac{ \sum_{i < j} ( {x^r_i} y_j - {x^r_j} y_i)^2 } {\|\anchorrow\|_2^2 \|\yvec\|_2^2} \leq  \frac{ \tol^2 \sum_{i < j} {x^r_i}^2 {x^r_j}^2 }{\|\anchorrow\|_2^2 \|\yvec\|_2^2}.
\]
%
For ease of notation, we let $\yvec_{min}$ denote the non-anchor row \yvec of minimum squared $L_2$ norm in \inputmat and \( \tau = \frac{ \tol^2 \sum_{i < j} {\anchorrowentryi}^2 {\anchorrowentryj}^2 }{\|\anchorrow\|_2^2 \| \yvec_{min} \|_2^2 } \), which corresponds to the largest possible bound on $\sin^2(\theta)$ across all rows of \outputmat, and will be useful later in the proof. 
%\( \frac{\|\xvec\|^2 \|\yvec\|^2 - (\xvec \cdot \yvec)^2}{\|\xvec\|^2 \|\yvec\|^2} = \frac{ \sum_{i < j} (x_i y_j - x_j y_i)^2 } {\|\xvec\|^2 \|\yvec\|^2} \leq  \frac{ \tol^2 \sum_{i < j} |y_i|^2 |y_j|^2 }{\|\xvec\|^2 \|\yvec\|^2} = \omega \). 
%

A widely-known result in linear algebra guarantees that the square of a singular value of $\outputmat$ is equal to the corresponding eigenvalue of the symmetric and positive semi-definite Gram matrix $\gram = \outputmat \outputmat^T \in \real^{\nrowssubmatrix \times \nrowssubmatrix}$~\cite{strang2022introduction}. 
Consider the rank-$1$ approximation $\estimate{\outputmat}$ of $\outputmat$ given by the \svd.  
Subtracting $\estimate{\outputmat}$ from $\outputmat$ cancels out the leading (i.e., largest) singular value of \outputmat. 
Thus, to prove an upper bound on the spectral norm of \outputerror, we prove an upper bound on the second largest singular value of \outputmat, which is equivalent to the square root of the largest eigenvalue $\lambda_{max}(\gram)$ of \gram. 
%
To find an upper bound on the the second largest eigenvalue of \gram, we start by deriving a lower bound on the largest eigenvalue. 
Such lower bound follows from the inequality \( \sin^2(\theta) \leq \tau \) which holds for all angles $\theta$ between the anchor row \anchorrow and any other row $\yvec$. 
%For the purpose of exposition, let $\sqrt{1 - \delta^2 \sum_{i < j} |x_i|^2 |x_j|^2} = \omega'$. 
Intuitively, this inequality suggests that all the row vectors are aligned to the same vector \xvec. 
Thus, the angle between any two non-anchor rows cannot be arbitrarily large. 
%, and, equivalently, the cosine between any two rows cannot be arbitrarily small. 
%More precisely, the angle $\theta_{i,j}$ between two rows $\yvec_i$ and $\yvec_j$ is maximum when such two vectors lie on the opposite sides of \anchorrow and they deviate as much as possible from it. 
%When the two vectors $\yvec_i$ and $\yvec_j$ lie on the opposite sides of \anchorrow, $\theta_{i,j}$
%is equal to the sum of the two angles between \anchorrow and $\yvec_i$ and between \anchorrow and $\yvec_j$. 
More precisely, the angle between  $\yvec_i$ and $\yvec_j$ can be at most equal to the sum of the angles between $\yvec_i$ and $\anchorrow$ and between $\yvec_j$ and $\anchorrow$. 
In this case,  we have: 
\[ 
\cos (\theta_{i,j}) = \cos (\theta_i) \cos (\theta_j) - \sin (\theta_i) \sin (\theta_j), 
\]

%\cnote[MC]{Could you also double-check this statement above (starting from "more precisely..."?)}
%\cnote[AG]{What does ``their possible deviation'' mean?}
%\cnote[mc]{rephrased}

where $\theta_i$ and $\theta_j$ denote the angle between $\yvec_i$ and $\anchorrow$ and the angle between $\yvec_j$ and $\anchorrow$, respectively, whose squared sines are bounded by $\tau$. 
Recalling that the squared cosine equals the complement to $1$ of the squared sine, we obtain: 
\[
\cos(\theta_{i,j}) \geq ( \sqrt{1 - \tau} \sqrt{1 - \tau} ) - ( \sqrt{\tau}  \sqrt{\tau}),
\]
i.e., $\cos(\theta_{i,j}) \geq 1 - 2 \tau$, which is equivalent to: 
\[
\sin^2(\theta_{i,j}) \leq 4 \tau ( 1 - \tau). 
\]
%
We have obtained an upper bound on the squared sine of the angle between any pair of non-anchor rows in \outputmat, which translates into a lower bound on the inner product. 
In particular, we have that: 
\begin{align*}
    \sin^2(\theta_{i,j})  = 1 - \cos^2 (\theta_{i,j})   = 1 - \frac{ (\yvec_i^T \yvec_j)^2}{ \| \yvec_i \|^2_2 \| \yvec_j \|^2_2 } \leq 4 \tau (1 - \tau),  
\end{align*}
implying: 
\begin{align*}
 - (\yvec_i^T \yvec_j)^2 \leq 4 \tau (1 - \tau)  \| \yvec_i \|^2_2 \| \yvec_j \|^2_2 - 1,
\end{align*}
%\iff \xvec^T \yvec \geq 1 - \omega \| \xvec \|^2_2 \| \yvec \|^2_2, 
and from which: 
\[
\yvec_i^T \yvec_j \geq \sqrt{1 - 4 \tau ( 1 - \tau) \| \yvec_i \|^2_2 \| \yvec_j \|^2_2 }. 
\]
A bound that holds for all possible pairs of rows $\yvec_i$ and $\yvec_j$ is thus: 
\[
\sqrt{1 - 8 \tau (1 - \tau)  \| \yvec_{max} \|^2},  
\]
where 
$\yvec_{max}$ denotes the non-anchor row of maximum $L_2$ norm. 

%\[
%\yvec_i^T \yvec_j \geq \sqrt{1 - \delta^2 \sum_{i < j} %|x_i|^2 |x_j|^2}. 
%\]

Now that we have obtained a lower bound on the inner products between any pair  of rows of \outputmat, note that the inner products correspond precisely to the off-diagonal entries of \gram, while the diagonal entries of \gram are all of the form $\yvec_i^T \yvec_i = \| \yvec_i \|_2^2$. 
%
It is known that the largest eigenvalue of a matrix can be found by maximizing Rayleigh quotient~\cite{strang2022introduction}, i.e., it satisfies:
\begin{equation*}
    \lambda_{\max}(\gram) = \max_{\mathbf{v} \neq \mathbf{0}} \frac{\mathbf{v}^{T} \gram \mathbf{v}}{\mathbf{v}^{T} \mathbf{v}}.
\end{equation*}
%
Choosing $\mathbf{v} = (1,1,\dots,1)^T \in \real^{1 \times \nrowssubmatrix}$, we get:
%\begin{equation*}
%    \mathbf{v}^{T} \gram \mathbf{v} = %\sum_{i,j} \gram_{ij} \geq %\nrowssubmatrix + (\nrowssubmatrix %-1)\nrowssubmatrix  \tau', 
%\end{equation*}
\begin{equation*}
    \mathbf{v}^{T} \gram \mathbf{v} = \sum_{i,j} \gram_{ij} \geq \frobeniusnorm{\outputmat}^2 + (\nrowssubmatrix -1)\nrowssubmatrix  \tau', 
\end{equation*}
%
%where $\omega' = 1 - \omega \| \xvec \|_2 \| \yvec \|_2$. 
where $\tau' = \sqrt{1 - 8 \tau ( 1 - \tau) \| \yvec_{max} \|^2}$. 
%
Since the denominator of Rayleigh quotient $\mathbf{v}^{T} \mathbf{v}$ takes value $\nrowssubmatrix$, we obtain:
\begin{equation*}
    \lambda_{\max}(\gram) \geq \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} + (\nrowssubmatrix-1)\tau'.  
\end{equation*} 
%
%While we omit the details, one can alternatively arrive to the same inequality using Gershgorin circle theorem~\cite{weisstein2003gershgorin}.
%
Thus, for the largest singular value $\sigma_1(\outputmat)$ of \outputmat, we have that 
\(  \sigma_1(\outputmat) \geq  \sqrt{ \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} + (\nrowssubmatrix -1)\tau'} \). 
%
We also have the equality~\cite{strang2022introduction}:
\begin{equation*}
    \sum_{i=1}^{n} \lambda_i(\gram) = \text{Tr}(\gram) = \frobeniusnorm{\outputmat}^2.
\end{equation*}
%
Therefore, since $\lambda_{\max}(\gram) \geq \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} + (\nrowssubmatrix-1)\tau'$, and the eigenvalues after the first one cannot be larger than the first one, the remaining eigenvalues satisfy:
\begin{equation*}
    \sum_{i=2}^{\nrowssubmatrix} \lambda_i(\gram) \leq \frobeniusnorm{\outputmat}^2 - \left(\frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} + (\nrowssubmatrix-1)\tau'\right) = \frobeniusnorm{\outputmat}^2 - \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} - (\nrowssubmatrix-1)\tau'.
\end{equation*}
%
Hence, we get:
\begin{equation*}
    \lambda_2(\gram) \leq \frobeniusnorm{\outputmat}^2 - \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} - (\nrowssubmatrix-1)\tau'.
\end{equation*}
%
As a consequence, recalling the definition of $\tau'$, %and observing that $  \| \xvec \|_2 \| \yvec \|_2 \leq 2 \max_{\xvec} \| \xvec \|_2 $ ,  
we can conclude: 
\begin{align*}
\spectralnorm{\outputerror} \leq  \sigma_2( \outputmat )  \leq 
\\
\sqrt{
\frobeniusnorm{\outputmat}^2 - \frac{\frobeniusnorm{\outputmat}^2}{\nrowssubmatrix} - (\nrowssubmatrix-1) \sqrt{1 -  8 \max \| \outputmat_{i,:} \|^2_2  \frac{ \delta^2  \sum_{i < j}  { x^r_i }^2 {x^r_j}^2   }{ \| \xvec \|_2^2 \min_i \|\outputmat_{i,:}\|_2^2 } (1 - \frac{ \delta^2  \sum_{i < j}  { x^r_i }^2 {x^r_j}^2 }{ \| \xvec \|_2^2 \min_i \|\outputmat_{i,:}\|_2^2 } )   }
}.
\end{align*}


\iffalse
\begin{align*}
& \spectralnorm{\outputerror} \leq  \sigma_2( \outputmat )  \leq  \\
& \sqrt{(\nrowssubmatrix -1) (1 - \sqrt{1 -  8 \max \| \outputmat_{i,:} \|^2_2  \frac{ \delta^2  \sum_{i < j} | x_i |^2 | x_j |^2 }{ \| \xvec \|_2^2 \min_i \|\outputmat_{i,:}\|_2^2 } (1 - \frac{ \delta^2  \sum_{i < j} | x_i |^2 | x_j |^2 }{ \| \xvec \|_2^2 \min_i \|\outputmat_{i,:}\|_2^2 } )   }    )   }. 
\end{align*}
\fi 
%\[
%spectralnorm{\outputerror} \leq  \sigma_2( \outputmat ) %\leq \sqrt{(\nrowssubmatrix-1)(\omega \| \xvec \|_2 \| %\yvec \|_2 )} \leq \sqrt{(\nrowssubmatrix-1)( 2 \omega %%\max_{\xvec} \| \xvec \|_2 )}. 
%\] 

As usual, the same derivations also apply to the columns of \outputmat, which concludes the proof. 
%Therefore, the bound on the spectral norm and hence the theorem follows. 
\end{proof}


\iffalse 
\begin{align*}
\spectralnorm{\outputerror} \leq  \sigma_2( \outputmat )  \leq 
\\
\sqrt{
\gamma ( \frac{n-1}{n} )  - (\nrows-1) \sqrt{1 -  8 \max \| \outputmat_{i,:} \|^2_2 \tol^2 \omega_r  (1 - \tol^2 \omega_r )}
}.
\end{align*}
\fi 



























































\iffalse 
Given \initialmat, we compute the Gram matrix 
\[
\mathbf{G}_{\initialmat} = \initialmat \initialmat^T = \begin{bmatrix}
\|\xvec\|^2 &  \xvec^T \yvec \\
 \xvec^T y & \|\yvec\|^2
\end{bmatrix}. 
\]

The singular values of \initialmat are correspond to the square root of the eigenvalues of $\initialmat \initialmat^T $. 
Furthermore, the matrix $\initialerror$ has largest singular value given by the second (or smallest) singular value of \initialmat since the first singular value is completely captured by the rank-$1$ \svd. 
%
Therefore, an upper bound on the smallest eigenvalue of $\mathbf{G}_{\initialmat}$ results in an upper bound on the largest singular value of $\initialerror$, and thus on its spectral norm. 

By definition~\cite{strang2022introduction}, the eigenvalues \( \lambda_1(\mathbf{G}_{\initialmat}) \text{ and } \lambda_2(\mathbf{G}_{\initialmat}) \) of $\mathbf{G}_{\initialmat}$ are the roots of the following equation in the variable $\lambda$:
\[
\det(\mathbf{G}_{\initialmat} - \lambda \identitymat) = 0, 
\]
where \identitymat is the $2 \times 2$ identity matrix and hence \(
\mathbf{G}_{\initialmat} - \lambda \identitymat\) is 
\(
\begin{bmatrix}
\|\xvec\|_2^2 - \lambda & \xvec^T \yvec \\
\xvec^T \yvec & \|\yvec\|_2^2 - \lambda 
\end{bmatrix}.
\)
Expanding the determinant of $\mathbf{G}_{\initialmat} - \lambda \identitymat$ and equating it to $0$, we obtain:

\[
(\|\xvec\|_2^2 - \lambda)(\|\yvec\|_2^2 - \lambda) - (\xvec^T \yvec)^2 = 0, 
\]
i.e.,
\[
\lambda^2 - (\|\xvec\|_2^2 + \|\yvec\|_2^2) \lambda + (\|\xvec\|_2^2  \|\yvec\|_2^2 - (\xvec^T  \yvec)^2) = 0. 
\]

Thus, the two eigenvalues, which are by definition given by the two solutions of this quadratic equation, are: 

\[
\lambda_{1,2} = \frac{(\|\xvec\|_2^2 + \|\yvec\|_2^2) \pm \sqrt{(\|\xvec\|_2^2 + \|\yvec\|_2^2)^2 - 4 (\|\xvec\|_2^2 \|\yvec\|_2^2 - (\xvec^T  \yvec)^2)}}{2}. 
\]

Since \( \mathbf{G}_{\initialmat} \) is symmetric and positive semi-definite, both eigenvalues are nonnegative. 
Furthermore, as $\lambda_2 \leq \lambda_1$, it must be that: 
\[
\lambda_2 =  \frac{(\|\xvec\|_2^2 + \|\yvec\|_2^2) - \sqrt{(\|\xvec\|_2^ + \|\yvec\|_2^2)^2 - 4 (\|\xvec\|_2^ \|\yvec\|_2^2 - (\xvec \cdot \yvec)^2)}}{2} . 
\]
Simple algebra shows that the term \(  \|\xvec\|_2^2 \|\yvec\|_2^2 - (\xvec \cdot \yvec)^2 \) in the denominators equals \(  \|\xvec\|_2^2 \|\yvec\|_2^2 \sin^2(\theta) \), where, as usual, $\theta$ denotes the angle between $\xvec$ and $\yvec$. 
We have previously shown that \(  \|\xvec\|_2 \|\yvec\|_2 \sin(\theta) = | x_1 y_2 - x_2 y_1| \leq \toleranceinit \), so that \(\|\xvec\|_2^2 \|\yvec\|_2^2 \sin^2(\theta) \leq \toleranceinit^2 \). 
Therefore, we have: 
\[
\sqrt{(\|\xvec\|_2^2 + \|\yvec\|_2^2)^2 - 4 (\|\xvec\|_2^2 \|\yvec\|_2^2 - (\xvec^T \yvec)^2)}
\geq \sqrt{(\|\xvec\|_2^2 + \|\yvec\|_2^2)^2 - 4 \toleranceinit^2},
\]
which means: 
\[
\lambda_2 \leq \frac{(\|\xvec\|_2^2 + \|\yvec\|_2^2) - \sqrt{(\|\xvec\|_2^2 + \|\yvec\|_2^2)^2 - 4 \toleranceinit^2}}{2}.
\]
In view of the relationship between the eigenvalues of  \( \mathbf{G}_{\initialmat} \) and the singular values of \initialmat, we conclude that: 
\[
\sigma_2 \leq \sqrt{\frac{\|\xvec\|_2^2 + \|\yvec\|_2^2) - \sqrt{(\|\xvec\|_2^2 + \|\yvec\|_2^2)^2 - 4 \toleranceinit^2}}{2}}. 
\]



Finally, observe that \(  \|\xvec\|_2^2 + \|\yvec\|_2^2 = \frobeniusnorm{\initialmat}^2 \),  
so that: 
\( \sigma_2 \leq  \sqrt{\frac{\frobeniusnorm{\initialmat}^2 - \sqrt{\frobeniusnorm{\initialmat}^2  - 4 \toleranceinit^2}}{2}}, \) 
which concludes the proof of the bound on the spectral norm and thus the lemma. 
\fi 






\iffalse

\spara{Proof of Proposition~\ref{prop:necessary}.}
\begin{proof}
To see why this proposition holds, consider the following argument. 
Let $x_1$ and $x_2$ be two entries of the anchor row or columns and $(\epsilon_1 , \epsilon_2)$ the errors obtained when approximating two entries of another row $y_i$ and $y_2$ as $\alpha x_1$ and $\alpha x_2$, respectively. 

Assume $| \alpha + \frac{\epsilon_1}{x_1} - \alpha - \frac{\epsilon_2}{x_2}| =  | \frac{\epsilon_1}{x_1} - \frac{\epsilon_2}{x_2}| \geq \tol$.
How small can both $\epsilon_1$ and $\epsilon_2$ be? 
It is easy to see that at least one of them can be arbitrarily large. In particular, $\epsilon_1$ can become arbitrary large and $\epsilon_2$ can become arbitrary small, or vice versa. 
However, they cannot be arbitrary small at the same time. At least one of them will be lower bounded. 
Notice that by triangle inequality: 
\begin{equation}
    \frac{|\epsilon_1|}{|x_1|} - \frac{|\epsilon_2|}{|x_2|} \geq | \frac{\epsilon_1}{x_1} - \frac{\epsilon_2}{x_2}|. 
\end{equation}
We have: 
\begin{itemize}
    \item $|\epsilon_1| \geq \tol |x_1| + \frac{|\epsilon_2|}{|x_2|}$. 
    \item $|\epsilon_2| \geq \tol |x_2| + \frac{|\epsilon_1|}{|x_1|} $. 
\end{itemize}
Therefore, either $\epsilon_1 \geq \tol |x_1|$ or $\epsilon_2 \geq \tol |x_2|$. 
The above observation means that if we want the element-wise error magnitude to be at most  $\Delta$, we need $\tol  min(|x_1|, |x_2|) < \Delta$, i.e., $\tol < \frac{\Delta}{min(|x_1|, |x_2|}$.  
%For simplicity, we have considered vectors \xvec and \yvec corresponding to rows of the matrix. Analogous analysis also holds for the columns of the matrix. 
The analysis holds for any pair of row or column elements. 
\end{proof}
\fi 

==> arXiv-2506.06456v1/pseudocodes/general.tex <==
\makeatletter
% Modify comment style: // in dark gray color and italicized
\renewcommand{\algorithmiccomment}[1]{\hfill {\color{black!80} \textit{// #1}}}
\makeatother


\begin{algorithm}[t]
%\caption{General Procedure}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Matrix \inputmat, target rank $\generalrank$, number of initializations $\nrep$, initial tolerance $\toleranceinit$, tolerance $\tol$. 
\STATE \textbf{Output:} Near-rank-$\generalrank$ sub\-matrix $\outputmat^*$. 
\STATE $\outputmat^* \gets \mathbf{0}$
\FOR{$i = 1$ to $\nrep$}
    \STATE $\initialmat \gets $ \textbf{Initialization}(\inputmat, \generalrank, \toleranceinit)\COMMENT{first phase: initialization  (sampling)} 
    \STATE $\outputmat \gets $ \textbf{Expansion}(\initialmat, \generalrank, \tol)\COMMENT{second phase: expansion} 
 %\textbf{Expansion:} Expand the identified subset while ensuring the desired entry-wise error guarantees
    \IF{$\f{\outputmat} \geq \f{\outputmat^*}$}
    \STATE $\outputmat^* \gets \outputmat$\COMMENT{select the best sub\-matrix across different initializations}   
\ENDIF
\ENDFOR
\STATE \textbf{Return} $\outputmat^*$
\end{algorithmic}
\caption{Overview of \ourmethod.} % for near-rank-$\generalrank$ sub\-matrix discovery.}
\label{alg:general} 
\end{algorithm}



==> arXiv-2506.06456v1/pseudocodes/iterated.tex <==
\begin{algorithm}[t]
%\caption{Iterative Local Low-rank Approximation}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Matrix \inputmat, vector of target ranks $\mathbf{\generalrank} \in \real^{\nrows \times \ncols}$, number of initializations $\nrep$, number of near-low-rank sub\-matrices $N_{patterns}$, initial tolerance $\toleranceinit$, tolerance $\tol$. 
\STATE \textbf{Output:} Estimate $\estimate{\inputmat}$ of \inputmat. 

\STATE $\estimate{\inputmat} \gets \mathbf{0}$
\FOR{$h = 1$ to $N_{patterns}$}

    \STATE $\estimate{\outputmat}_h \gets \mathbf{0}, \rowset_h \gets \emptyset, \colset_h \gets \emptyset$ \COMMENT{initialize best sub\-matrix across target ranks}
    
    \FOR{$k \in \mathbf{\generalrank}$}

    \STATE $\outputmat, \estimate{\outputmat}, \rowset , \colset \gets  
    \textsc{FindNearLowRankSubmatrix}(\inputmat, \generalrank,  \nrep, \toleranceinit, \tol)$ \COMMENT{return a near-rank-$k$ sub\-matrix with its rank-$k$ estimate, row and column indices} 

    \IF{$f(\estimate{\outputmat}) > f(\estimate{\outputmat}_h)$}
    \STATE $\estimate{\outputmat}_h \gets \estimate{\outputmat},\rowset_h \gets \rowset, \colset_h \gets \colset$\COMMENT{update best sub\-matrix across target ranks}
%$\estimate{\outputmat}_h \gets \estimate{\outputmat}$
    \ENDIF
    \ENDFOR
    \STATE $\estimate{\inputmat}_{\rowset_h , \colset_h} = \estimate{\inputmat}_{\rowset_h , \colset_h}  + \estimate{\outputmat}_h $\COMMENT{update current estimate}

    \STATE $ \inputmat_{\rowset_h , \colset_h} \gets \inputmat_{\rowset_h , \colset_h} - \estimate{\outputmat}_h $\COMMENT{update input for the next iteration}
    \ENDFOR
    %\STATE $\initialmat \gets $ \textbf{Initialization}(\inputmat) 
    %\STATE $\outputmat \gets $ \textbf{Expansion}(\initialmat) 
 %\textbf{Expansion:} Expand the identified subset while ensuring the desired entry-wise error guarantees
   % \IF{$f(\outputmat) > f(\outputmat^*)$}
  %  \STATE $\outputmat^* \gets \outputmat$    
\STATE \textbf{Return} $\estimate{\inputmat}$
\end{algorithmic}
\caption{\label{alg:iterated} Iterative algorithm to find multiple near-rank-$k$ sub\-matrices.}
\end{algorithm}

==> arXiv-2506.06456v1/pseudocodes/rankk.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\STATE \textbf{Input:} Matrix $\inputmat \in \real^{\nrows \times \ncols}$, target rank \generalrank, number of initializations $\nrep$, initial tolerance $\toleranceinit$, tolerance $\tol$.
\STATE \textbf{Output:} Near-rank-$\generalrank$ sub\-matrix $\outputmat^*$.
\STATE $\outputmat^* \gets \textbf{0}$\COMMENT{start initialization phase} 
\STATE $\Omega \gets \{ (i,j) \}, \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols\}$
\FOR{$t = 1$ to $\nrep$}
    %\STATE $\initialmat' \gets  (i_1, j_1), (i_2, j_2), (i_3, j_3), (i_4, j_4)$  
    \STATE \( \Gamma \gets \{(i_h, j_h) \sim Uniform(\Omega) \mid h = 1, \dots,  \generalrank + 1 \} \)
    \STATE \( \initialmat'_{i_h, j_h} \gets \inputmat_{i_h, j_h}, \quad \forall (i_h , j_h) \in \Gamma \) 
    \WHILE{$ | \det(\initialmat') | > \toleranceinit$}
    \STATE \( \Gamma \gets \{(i_h, j_h) \sim Uniform(\Omega) \mid h = 1, \dots, \generalrank + 1 \} \)
    \STATE \( \initialmat'_{i_h, j_h} \gets \inputmat_{i_h, j_h}, \quad \forall (i_h , j_h) \in \Gamma \)\COMMENT{repeat until $\initialmat'$ is rank-deficient} 
    \ENDWHILE
    %
    \STATE $\initialmat \gets \initialmat'$\COMMENT{start expansion phase}
    %
    \STATE \( \indrows \gets \textsc{ExtractIndicatorMatrix}( \inputmat, \nrows,  \initialmat, \Gamma, \generalrank, \tol) \) %\COMMENT{compute indicator matrix for the rows}
    \STATE \(  \Gamma_{\mathcal{C}} \gets \{ (j,i)  \}, \quad \forall (i,j) \in \Gamma \) 
    \STATE      \( \indcols \gets \textsc{ExtractIndicatorMatrix}( \inputmat^T,  \ncols,   \initialmat^T, \Gamma_{\mathcal{C}} , \generalrank, \tol) \) %\COMMENT{compute indicator matrix} 
    %\COMMENT{compute indicator matrix for the columns}
    \STATE \( \ind \gets \indrows \cap {\indcols}^T \) \COMMENT{compute indicator matrix} 
    %
    \STATE \( \outputmat \gets \textsc{ExtractMaximumEdgeBiclique}(\ind) \) %\COMMENT{Extract maximum-edge biclique} 
    \IF{$f(\outputmat) > f(\outputmat^*)$}
    \STATE $\outputmat^* \gets \outputmat$  
    \ENDIF
    \ENDFOR
\STATE \textbf{Return} $\outputmat^*$
\STATE \textbf{Procedure }{\textsc{ExtractIndicatorMatrix}}
    \STATE \textbf{Input:} Input matrix \( \inputmat^{\Lambda}  \), number of rows \( 
    \nrows^{\Lambda} \),  initial submatrix $\initialmat^{\Lambda} $, set of indices $\Gamma^{\Lambda}$, target rank 
    $\generalrank$, tolerance $\tol$.  
    \STATE \textbf{Output:} indicator matrix \( {\ind}^{\Lambda} \). 
    %\STATE \( \Phi \gets \Gamma \{(i_k, j_k) \sim Uniform(\Omega) \mid k = 1, \dots,  \generalrank + 1 \}    \)
    \STATE \( \Phi \gets \{ i_h \sim Uniform(\{1, \dots, \nrows^{\Lambda} \}) \mid h = 1, \dots, \generalrank \} \)\COMMENT{sample \generalrank indices}
    %\STATE \( \initialmats \gets \initialmat_{\Phi, :} \) 
   % \STATE \( \bfA \gets \initialmats^T \)
    \STATE \( \mathbf{C} \gets \inputmat_{:, j; j \in \Gamma_{\Lambda}} \initialmat_{\Phi, :}^+ \) \COMMENT{compute orthogonal-projection coefficients}
    \STATE \( \estimate{\inputmat}^\perp \gets \mathbf{C} \inputmat_{\Phi,:}  \) \COMMENT{compute orthogonal projections}
    \STATE \( \errors \gets | \estimate{\inputmat}^\perp - \inputmat |  \)  \COMMENT{compute matrix of absolute errors}
    %\STATE \( \ind_{\Lambda} \gets \mathbf{0} \)
    \STATE \( {\ind^{\Lambda}}_{i,j} \gets  \mathbf{1}( \errors_{i,j} \leq \tol )  \) %\COMMENT{compute indicator matrix}
    \STATE \textbf{Return} \( \ind^{\Lambda} \)
\end{algorithmic}
\caption{\label{alg:rankk} Algorithm to find a near-rank-$k$ sub\-matrix.}
\end{algorithm}

==> arXiv-2506.06456v1/pseudocodes/rankone.tex <==
\begin{algorithm}[t!]
\begin{algorithmic}[1]
\STATE \textbf{Input:} Matrix $\inputmat \in \real^{\nrows \times \ncols}$, number of initializations $\nrep$, initial tolerance $\toleranceinit$, tolerance $\tol$. 
\STATE \textbf{Output:} Near-rank-$1$ sub\-matrix $\outputmat^*$. 
\STATE $\outputmat^* \gets \mathbf{0}$\COMMENT{start initialization phase}
\STATE $\Omega \gets \{ (i,j) \}, \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols\}$
\FOR{$t = 1$ to $\nrep$}
    %\STATE $\initialmat' \gets  (i_1, j_1), (i_2, j_2), (i_3, j_3), (i_4, j_4)$  
    \STATE \( \Gamma' \gets \{ (i_1, j_1), (i_2, j_2)  \sim Uniform(\Omega) \} \)\COMMENT{sample two entries at random}
    \STATE \( \Gamma \gets \ \Gamma' \cup \{ (i_2, j_1), (i_1, j_2) \} \)\COMMENT{complete $2 \times 2$ sub\-matrix} 
    \STATE \( \initialmat'_{i_h, j_h} \gets \inputmat_{i_h, j_h}, \quad \forall (i_h , j_h) \in \Gamma \) 
    \WHILE{$ |\det(\initialmat')| > \toleranceinit$}
    \STATE  \( \Gamma' \gets \{ (i_1, j_1), (i_2, j_2)  \sim Uniform(\Omega) \} \)\COMMENT{repeat until $\initialmat'$ is close to rank $1$} %\COMMENT{sample until the $2 \times 2$ sub\-matrix is close to rank $1$} 
    \STATE \( \Gamma \gets \ \Gamma' \cup \{ (i_2, j_1), (i_1, j_2) \} \) 
    \STATE \( \initialmat'_{i_h, j_h} \gets \inputmat_{i_h, j_h}, \quad \forall (i_h , j_h) \in \Gamma \) 
    \ENDWHILE
    %
    \STATE $\initialmat \gets \initialmat'$\COMMENT{start expansion phase}  
    %
    \STATE  $(i_a, j_a) \sim Uniform(\Gamma)$ \COMMENT{select anchor} 
    \STATE $(\anchorrow, \anchorcolumn) \gets (\inputmat_{i_a,:}, \inputmat_{:,j_a})$
    %
    \STATE \( \rowratiosij \gets \frac{\inputmat_{i,j}}{\anchorrow_j}, \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols \} \)\COMMENT{compute row-wise ratios} 
    %
    \STATE \( \columnratiosij \gets \frac{\inputmat_{i,j}}{\anchorcolumn_i}, \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols \} \)\COMMENT{compute column-wise ratios}
    % 
    %\STATE \( S_i \gets \{ j \mid | \rowratios_{i,j} - \rowratios_{i,j_{\mathcal{A}}} | < \tol \}, \quad \forall i \in \{1, \dots,  \nrows \} \)
    %\STATE \( \indrows \gets \mathbf{0} \)
    %\STATE \( {\indrows}_{i,j} \gets \mathbf{1} \left( | {\rowratios}_{i,j} - {\rowratios}_{i,j_{a}}| < \tol \right), \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols \} \) 
    \STATE \( \indrows \gets \mathbf{0}\)\COMMENT{compute indicator matrix for the rows}
    \FOR{$i=1$ to $\nrows$}
    %\STATE $\Psi_i \gets {S \subseteq \{ 1, \dots , \ncols \}, \, \anchorindexrow \in S, |\inputmat_{i,j_1} - \inputmat_{i,j_2}| \leq \tol} $
    %\STATE $\mathcal{S} \gets \{ \Psi \subseteq \{ 1, \dots , \ncols \} \mid \anchorindexcol \in \Psi, \,  | \rowratios_{i,j_1}- \rowratios_{i,j_2} | \leq \tol \,  \forall j_1, j_2 \in \Psi  \}  $
    %\STATE $\Psi_i \gets \argmax_{\Psi \in \mathcal{S}} |\Psi|$
    \STATE $\Psi_i \gets \argmax_{\{ \Psi \subseteq \{ 1, \dots , \ncols \} \mid \anchorindexcol \in \Psi, \,  | \rowratios_{i,j_1}- \rowratios_{i,j_2} | \leq \tol \,  \forall j_1, j_2 \in \Psi  \}} |\Psi|$ 
    %\STATE \text{subject to } $| \vec[i] - \vec[j] | \leq \delta, \quad \forall i, j \in S$ 
    \STATE \( \indrows_{i, \Psi_i} \gets 1 \)
    \ENDFOR
    \STATE \( \indcols \gets \mathbf{0} \)\COMMENT{compute indicator matrix for the columns}
    \FOR{$j=1$ to $\ncols$}
    %\STATE $\Psi_i \gets {S \subseteq \{ 1, \dots , \ncols \}, \, \anchorindexrow \in S, |\inputmat_{i,j_1} - \inputmat_{i,j_2}| \leq \tol}$
    %\STATE $\Psi_j \gets \{ \Psi \subseteq \{ 1, \dots , \nrows \} \mid \anchorindexrow \in \Psi, \,  | \inputmat_{i_1,j} - \inputmat_{i_2, j} | \leq \tol \,  \forall i_1, i_2 \in \Psi, \ \Psi  \in \argmax_{\Psi} |\Psi|  \} $
    \STATE $\Psi_j \gets \argmax_{\{ \Psi \subseteq \{ 1, \dots , \nrows \} \mid \anchorindexrow \in \Psi, \,  | \columnratios_{i_{1},j}- \columnratios_{i_{2},j} | \leq \tol \,  \forall i_1, i_2 \in \Psi  \}} |\Psi|$ 
    %\STATE \text{subject to } $| \vec[i] - \vec[j] | \leq \delta, \quad \forall i, j \in S$ 
    \STATE \( \indcols_{  \Psi_j  , j  } \gets 1 \)
    \ENDFOR 
    %\COMMENT{compute indicator matrix for the rows} 
    %\STATE \( {\indcols} \gets \mathbf{0} \)
    %\STATE \( {\indcols}_{i,j} \gets \mathbf{1} ( | {\columnratios}_{i,j} - {\columnratios}_{i_{a},j}
    %  < \tol) , \quad \forall i \in \{1, \dots, \nrows \}, \forall j \in \{1, \dots, \ncols\} \) %\COMMENT{compute indicator matrix for the columns} 
    \STATE \( \ind \gets \indrows \cap \indcols \) \COMMENT{compute indicator matrix} 
    %
    \STATE \( \outputmat \gets \textsc{ExtractMaximumEdgeBiclique}(\ind) \) %\COMMENT{Extract or approximate maximum-edge biclique} 
    \IF{$f(\outputmat) > f(\outputmat^*)$}
    \STATE $\outputmat^* \gets \outputmat$  
    \ENDIF
    \ENDFOR
\STATE \textbf{Return} $\outputmat^*$
\end{algorithmic}
\caption{\label{alg:rankone} Algorithm to find a near rank-$1$ sub\-matrix.}
\end{algorithm}

==> arXiv-2506.06456v1/related_arxiv.tex <==
\section{Related Work}
\label{sec:related}

\para{Low-rank matrix approximation.}
Low-rank approximation techniques are widely used 
to decompose a matrix into simpler components, 
capturing essential patterns while reducing noise and dimensionality. 
The \svd and the related \pca are among the most popular 
techniques~\cite{golub2013matrix}. 
%Nevertheless, several other methods for low-rank approximation and, more generally, for matrix decomposition, exist.
%Popular matrix decomposition techniques include the QR, Cholesky, and LU decompositions~\cite{bernstein2009matrix}. 
%All such techniques, however, assume a \emph{global} model for a matrix, approximating all its entries using a simpler structure. 
%\spara{Low-rank approximation beyond the \svd.}
% While the \svd has been widely successful across numerous applications, 
% it also has certain limitations in specific cases. 
% Over the years, research has been carried out to address the limitations of the \svd that may arise.  
%Thus, 
%over the years, research has been carried out to explore different approaches to low-rank approximation and address the limitations of the \svd that may arise. 
Nonnegative matrix factorization techniques~\cite{gillis2010using} 
%098aim to overcome certain limitations of \svd and 
have become popular in applications where the goal is to decompose data in nonnegative components. 
%In some applications where the data only have nonnegative values, it may be desirable to obtain a simpler matrix representation that also has only nonnegative values. 
%As the \svd does not guarantee nonnegativity in any case, . 
% Similarly, 
Boolean matrix decomposition relies on boolean algebra instead of linear algebra~\cite{miettinen2020recent}.
Column subset selection~\cite{boutsidis2009improved} and the CUR decomposition~\cite{mahoney2009cur}   
have emerged as more interpretable alternatives to the \svd. 
In 2019, Gillis and Shitov~\cite{gillis2019low}  studied the problem of low-rank approximation 
to minimize the maximum entry-wise deviation. 
%Further, in some applications, e.g. in consequential domains, it may be important to obtain inherently-interpretable simple representations of matrices. 
%To meet such needs, researchers have studied low-rank-approximation techniques that are more interpretable than the \svd, such 
More recently, an approach to low-rank approximation that accounts for multiplicative effects was introduced~\cite{ciaperoni2024hadamard}. % was introduced 
% to relax the implicit assumption of the \svd that the data follow a purely
%as a non-additive model. 
%As the \svd only provides guarantees on the total approximation error and not on the individual entries, 
%All such techniques, however, assume a \emph{global} model for a matrix; the \svd provides guarantees on the total approximation error, but not for its individual entries. 
%In this direction, 
%previous work however has studied the problem of global low-rank approximation to minimize the maximum entry-wise deviation~\cite{gillis2019low}. 
%In this work, we adopt a different point of view and we postulate that not all entries need to be approximated, but only those that admit a close approximation. 
\iffalse 
While the \svd provides optimality guarantees, the guarantees hold \emph{globally}, i.e. for the entire matrix approximation. 
On the other hand, individual entries may be far from their low-rank approximation. 
No low-rank-approximation technique can provide guarantees at the level of the individual matrix entries. 
Previous work however has also studied the problem of global low-rank approximation to minimize the maximum entry-wise deviation~\cite{gillis2019low}. 
Also recently work has been done to challenge the role of the \svd as a gold standard for low rank approximation. 
For instance, in 2024, Ciaperoni et al.~\cite{ciaperoni2024hadamard} 
% cant use citet with this template it seems 
introduce the Hadamard decomposition, an extension of the \svd that accounts for multiplicative effects and retrieves more concise yet equally accurate representations of matrices. 
Friedenberg et al.~\cite{friedenberg2017minkowski} also study the theoretical underpinning of such matrix-decomposition method from the point of view of algebraic geometry. 
The Hadamard decomposition relaxes the assumption made by the \svd that the data are generated as a sum of a number of rank-$1$ matrices.  
Meanwhile, Gleich~\cite{gleich2024better} shows that one can achieve a better low-rank approximation by computing the \svd after suitably reshaping the original matrix. 
\fi 
%All the work discussed so far in this section aims at finding simple representations for a given matrix that are as accurate as possible, where the accuracy is measured by aggregating the reconstruction error over all matrix entries. 
%Techniques like the \svd assume that the entire input matrix can be well-approximated by a low-rank structure. 
%As discussed in Section~\ref{sec:intro}, there are examples where a global assumption of low-rankness may be restrictive. 
%In real-world matrices across different domains, there can be submatrices that are 

\spara{Local low-rank matrix approximation.} 
Relatively less research has been conducted for finding decompositions
that do not assume a \emph{global} low-rank structure, 
which is the focus of our paper.
%  which can be restrictive in real-world matrices, 
The goal here is to find sub\-matrices that are \emph{locally} well-approximated by a low-rank structure.
%  and other that are full-rank. 
%Local low-rank approximation relaxes the global DA of low-rankness of the \svd  and related methods to deal with the scenario where there are 
% Despite the relevance of local low-rank approximations in the real world, % most research efforts have been devoted to global low-rank approximation, and local low-rank approximation 
% it still represents a largely unexplored area of research to which this work contributes. 
%
A simple heuristic to local low-rank approximation 
is obtained by imposing a sparsity constraint on matrix decomposition, 
%to the vectors that constitute a matrix decomposition the \svd.
and sparse PCA~\cite{mairal2009online} is a prominent example of such~methods.
% sparse-matrix-decomposition techniques. 


Doan and Vavasis proposed the problem of recovering near-rank-$1$ sub\-matrices 
by framing it as a convex-optimization problem  % and studying its properties~
\cite{doan2013finding}. 
Lee et al.~\cite{lee2016llorma} introduced the LLORMA method to address matrix-completion tasks while relaxing the assumption that the entire matrix has low rank. 
%given a partially observed matrix, 
%LLORMA predicts the missing observations 
%without assuming that the input matrix is %globally low rank. 
%Instead, LLORMA considers a model where each neighborhood is local well-approximated by a low-rank matrix. 
% LLORMA samples a number of anchor points from the observed entries (uniformly at random, by default), estimate a separate low-rank model around each anchor point, and uses a kernel smoother to blend the predictions of the local models.
LLORMA approximates the entire input matrix, 
and thus, it is fundamentally different from our work, 
which focuses on detecting local low-rank patterns. 
On the other hand, the problem we study finds application in matrix completion, 
as shown by the work of Ruchansky et al.~\cite{ruchansky2017targeted}, which introduces the \svp method to quickly detect low-rank sub\-matrices with the ultimate goal of improving the accuracy in matrix completion.  
% which has been designed to detect low-rank sub\-matrices to improve accuracy in matrix-completion tasks.  
% \svp first projects the rows and columns of the input matrix onto the first right singular vector, and then it extracts a sub\-matrix by selecting rows and columns that correspond to clusters with large row and column projections, respectively.
%t finds clusters of large row and column projections to obtain the output submatrix. 
% \svp and the other existing methods described so far for detecting low-rank sub\-matrices  are not expected to identify arbitrary sub\-matrices. 
% To tackle this lack of generality, in 2023, 
While \svp cannot discover arbitrary low-rank sub\-matrices, Dang et al.~\cite{dang2023generalized} introduced the \rpsp method, which addresses this lack of generality. 
%to detect arbitrary low-rank sub\-matrices. 
%(Random Probing-based Submatrix Propagation), 
%a novel approach for detecting local low-rank sub\-matrices. 
The core idea behind \rpsp is to sample sub\-matrices and count
the number of times that each entry belongs to a low-rank sub\-matrix. 
%
% approximates singular values from the \svd of progressively larger sampled sub\-matrices and estimates a matrix that counts the number of times that each entry belongs to a sampled low-rank sub\-matrix. The output low-rank sub\-matrices then correspond to co-clusters within this matrix of counts. 
Like \rpsp, our method targets arbitrary near-low-rank sub\-matrices. Unlike previous methods, our method can in principle identify  sub\-matrices that are close to a specific target rank. 


%, and thus it serves as our primary baseline.
%is the closest existing work to ours and serves as our primary baseline. 
%More details on \svp and \rpsp, which serve as our primary baselines, are given in~\ref{ap:technical_details}. 

 
% by sampling submatrices of increasingly large size and efficiently estimate their closeness to a low-rank structure by approximating singular values through a random projection approach. 

\iffalse 
which 
More specifically, this model assumes that there is a mapping that associates combinations of rows and columns to low-rank approximations which are slowly-varying. 
The mapping is estimated using non-parametric regression techniques. 
While this work addresses the  low-rank approximation problem while relaxing the globality assumption, it is fundamentally different from our work, since it still attempts to approximate the entire input matrix by combining different local low-rank structures. 
Instead, in our work, we are solely interested in identifying and approximating the submatrices that admit a faithful representation in terms of a low-rank matrix. 
\fi 

\iffalse 
In 2023, Dang et al.~\cite{dang2023generalized} develop a novel matrix computational framework called \rpsp (Random Probing based submatrix Propagation) 
that detects local low rank submatrices. 
\rpsp starts by sampling submatrices of increasingly large size and efficiently estimate their closeness to a low-rank structure by approximating singular values through a random projection approach. 
Thereby, \rpsp is able to estimate the likelihood that each matrix entry is contained into a low-rank submatrix, and finally yields low-rank submatrices by applying spectral co-clustering to the matrix of likelihoods~\cite{dhillon2001co}.
This work is the closest in nature to our work and serves as the main baseline for our methods. 
Nevertheless, in this work we  we adopt a different perspective on local low-rank submatrix detection. We only want to approximate those entries that provably admit a faithful low-rank representation.  
Furthermore, unlike \rpsp and other previous works, our approach does not rely on the \svd, leading to potential gains in efficiency and interpretability.  
\fi 


%Thus, our approach provides approximation guarantees for the retrieved low-rank submatrices. 
\spara{Co-clustering, projective clustering, and subspace clustering.}
%\cnote[MC]{this last paragraph can be removed}
%Another approach that can be used to find submatrices exhibiting particular properties is which
Co-cluster\-ing  algorithms~\cite{dhillon2001co}
%which are also used by \rpsp, 
simultaneously cluster the rows and columns of a matrix. 
Although co-clustering algorithms can be used %  useful building-blocks in the design of methods 
for detecting low-rank submatrices,  
% by themselves, co-clustering algorithms 
they cannot generally discover such structures, 
except in specific cases where the values of the low-rank submatrices deviate significantly from the background. 
%However, such algorithms, by themselves, are not designed to identify low-rank submatrices, except in the particular case where the values of the low-rank submatrices deviate significantly from the rest of the matrix. 
Projective clustering and subspace clustering are also related problems. % to the problem studied in this work. 
In projective clustering~\cite{agarwal2003approximation}, 
the goal is to partition the data into subsets such that the points in each subset are 
close to each other in some subspace. 
In subspace clustering~\cite{vidal2011subspace} the goal is to find a representation of the input data as 
a union of different subspaces. 
In general, clustering problems are fundamentally different from the problem we study, 
as they seek a partitioning of the entire data matrix. 


\iffalse 
\journal{
\spara{Affine sub\-spaces.}



}
\fi 








\iffalse 
%, which is not always the case (e.g. a low-rank submatrix may have the same mean as the entire matrix). 
%The methods we introduce to identify submatrices exhibiting the local low-rank property are inspired from the analogy between low-rank submatrices and vectors in a low-dimensional subspaces of a vector space. 
The problems studied in this work are also connected with projective clustering~\cite{agarwal2003approximation}. 
In projective clustering, 
For example, Agarwal and Procopiuc~\cite{agarwal2003approximation} investigate the maximum-cover-like problem of covering the space $\mathbb{R}^n$ by hyper-strips so that the maximum width of a hyperstrip (resp., the maximum diameter of a hyper-cylinder)
is minimized. % and
%Procopiuc et al.~\cite{procopiuc2002monte} use a Monte Carlo approach to approximate optimal projective clusters. 
A related problem is sometimes referred to in the literature as
subspace clustering. The goal of subspace clustering lies in 
%the 
%Subspace clustering is closely related to . 
%In subspace clustering 
Many different approaches have been proposed to address this problem~\cite{vidal2011subspace}.%Some methods rely on the assumption that similar points that are in a neighborhood of a given points lie in the same subspace. 
For example, some methods rely on the eigendecomposition of a Laplacian matrix obtained from a certain definition of affinity matrix reflecting the similarity of the points with respect to a common subspace. 
%The affinity matrix should not reflect the distances of the points. Instead, it should reflect 
%A possible approach to compute the affinity matrix is generalized principal component analysis~\cite{vidal2005generalized}. 
%Approaches to subspace clustering share the same fundamental differences with our method as approaches to projective clustering. 
The problems we introduce 
%can also be seen as a generalization of subspace clustering, 
%There are however importance differences. 
generalize subspace clustering, relaxing the assumption that the particular structure imposed on the data holds for the entire data matrix, and instead focusing only on identifying particularly natural subspaces. 
\fi 



%that grow from small submatrices of low rank property 
%determined by 

%The work that is closer to our









\iffalse 
There
exist mainly three types of methods that could be used to address the local low-rank-approximation problem, namely
co-clustering, sparse matrix decomposition, and anchor-based approaches. The main goal of co-clustering is to find a matrix partition
such that the intra-co-cluster distance could be minimized. For matrix decomposition-based methods, they identify
local low rank matrices by imposing sparsity constraints to the factor or singular matrices.
\fi 

\iffalse 
Among anchor-based methods,~\citet{lee2016llorma} consider a model where each neighborhood is well-approximated by a low-rank matrix. 
More specifically, this model assumes that there is a mapping that associates combinations of rows and columns to low-rank approximations which are slowly-varying. 
The mapping is estimated using non-parametric regression techniques. 
\fi 








%and the \svd plays a central role in low-rank approximation. 












%he singular value decomposition (\svd) and the closely related principal component analysis (\pca) are widely used method for matrix factorization and low-rank approximation. 
%Nevertheless, several other matrix-decomposition and low-rank-approximation methods exist. 


\iffalse 
While the optimality guarantees~\cite{chipman2020proofs} of the SVD make it a particularly appealing tool for a wide variety of applications, it has significant drawbacks in some cases. 
For instance, given a non-negative
input matrix, the SVD may yield negative values, which can be hard to interpret and hence not desirable.
To address this drawback,  non-negative matrix factorization has been introduced~\cite{gillis2019low}. 

Recently, a matrix-decomposition methods overcoming the additivity assumption of the SVD has been proposed~\cite{ciaperoni2024hadamard}. 
This decomposition can provide a more accurate and equally concise approximation of an input matrix. 
Meanwhile,~\citet{gleich2024better} demonstrates how a more accurate and equally concise approximations of matrix can be obtained by considering a different representation of the input matrix prior to applying the SVD. 


\spara{Local low-rank approximation}
In addition to methods that challenge the optimality of the SVD in providing an optimal approximation of an input matrix, work has also been carried out to relax the assumption of global low-rankness of the input matrix. 
In practice, the assumption of global low-rankness appears rather myopic; in practice there can be local subsets of data that are well-approximated by a low-rank matrix, and other that are closer to full-rank. % (e.g. due to the higher noise corruption). 
Local low-rank approximation is still a largely unexplored topic. 
\fi 


==> arXiv-2506.06456v1/special_case_algorithm.tex <==

In this section, we give a simple algorithm that can be used to solve Problem~\ref{prob:simplified} in polynomial time. 
The algorithm follows easily from the following result. 

\begin{lemma}\label{lemma:errortosine}
Consider two vectors $\xvec \in \real^\ncols$ and $\yvec \in \real^\ncols$ and let $\errorvec = \yvec - \proj{\xvec}{\yvec}$. 
We have: 
\[
\| \errorvec \|_2 = \| \yvec \|_2 \sin(\theta). 
\]
\end{lemma}

%the simplified problem where either the rows or the columns are given. 
To solve Problem~\ref{prob:simplified} optimally in polynomial time, i.e., to find a low-rank subset of rows for a fixed set of columns \colset, we simply normalize the rows 
of \inputmat to unit norm, and then compute the matrix $\sinematrix$ of pairwise sines, defined by: 
\[
\sinematrix = \sqrt{1 - (\inputmat \inputmat^T)^2}. 
\]
%Now, if we normalize the vectors to be unit norm (rows of $\inputmat$) we can 
The entry of indices $i$ and $j$ of \sinematrix indicates the $L_2$ norm of the error vector associated with the orthogonal projection of $\inputmat_{j,:}$ onto  $\inputmat_{i,:}$. 
Therefore, to find the largest possible set of rows,   we perform a linear scan over the rows of $\sinematrix$ and for each row we pick the largest possible subset such that all elements satisfy the input error requirements. 
The solution to Problem~\ref{prob:simplified} %for a fixed set of columns \colset 
is given by the largest subset found while scanning the rows. 

The solution to the symmetric problem asking for the largest subset of columns for a fixed set of rows \rowset can be found by simply inverting the role of the rows and columns in the algorithm. 
%In other words, we can easily find a solution to the rank-$1$ problem but for a fixed set of columns only, $I$.  
%This subset is exactly the solution to Problem~\ref{prob:simplified} for a fixed set of columns \colset. 

%Unfortunately, the simple deterministic algorithm presented in this section cannot be easily extend to tackle Problem~\ref{prob:rank-1}. 
%Instead, to address the general problem of discovering near-rank-$1$ sub\-matrices where both rows and columns are unknown, it is convenient to introduce sampling-based techniques.  
